Eigenvectors of Orthogonally Decomposable Functions

The Eigendecomposition of quadratic forms (symmetric matrices) guaranteed by the spectral theorem is a foundational result in applied mathematics. Motivated by a shared structure found in inferential problems of recent interest---namely orthogonal tensor decompositions, Independent Component Analysis (ICA), topic models, spectral clustering, and Gaussian mixture learning---we generalize the eigendecomposition from quadratic forms to a broad class of "orthogonally decomposable" functions. We identify a key role of convexity in our extension, and we generalize two traditional characterizations of eigenvectors: First, the eigenvectors of a quadratic form arise from the optima structure of the quadratic form on the sphere. Second, the eigenvectors are the fixed points of the power iteration. In our setting, we consider a simple first order generalization of the power method which we call gradient iteration. It leads to efficient and easily implementable methods for basis recovery. It includes influential Machine Learning methods such as cumulant-based FastICA and the tensor power iteration for orthogonally decomposable tensors as special cases. We provide a complete theoretical analysis of gradient iteration using the structure theory of discrete dynamical systems to show almost sure convergence and fast (super-linear) convergence rates. The analysis also extends to the case when the observed function is only approximately orthogonally decomposable, with bounds that are polynomial in dimension and other relevant parameters, such as perturbation size. Our perturbation results can be considered as a non-linear version of the classical Davis-Kahan theorem for perturbations of eigenvectors of symmetric matrices.

==> simplexframework - Copy/function-bounds.tex <==
\section{{\Sef} growth and perturbation bounds}
In this appendix, we provide some useful bounds for $(\alpha, \beta, \gamma, \delta)$-robust {\sef}s that are used throughout the error analysis proofs.
In particular, \cref{lem:F-robust-implications} provides useful bounds on each $g_k$, $h_k$ and their derivatives.
\cref{lem:fg-upper-bounds} provides bounds on the magnitude of $\nabla F$ and its projections.
Then, the remaining lemmas provide bounds on estimation and location perturbation errors for $\nabla F$ and $\GG$.

\begin{lem}\label{lem:F-robust-implications}
    The following bounds hold for every $k \in [\dm]$:
    \begin{compactenum}
        \item \label{lem:F-rb-impl:item:monomials}
        For every $x \in [-1, 1]$, $\frac{\beta}{(\delta + 1)\delta} \abs x^{2+2\delta} \leq \abs{g_k(x)} \leq \frac{\alpha}{(\gamma + 1)\gamma} \abs x^{2+2\gamma}$.
        \item \label{lem:F-rb-impl:item:1}
        For every $x \in [-1, 1]$, $2\frac{\beta}{\delta} \abs x^{1+2\delta} \leq \abs{g'_k(x)} \leq 2\frac \alpha \gamma \abs{x}^{1+2\gamma}$.
        \item \label{lem:F-rb-impl:item:1-5}
        For every $x \in [-1, 1]$, $2(2+1/\delta)\beta \abs x^{2\delta} \leq \abs{g_k''(x)} \leq 2(2+1/\gamma)\alpha \abs x^{2\gamma}$.
        \item \label{lem:F-rb-impl:item:2}
        For every $x \in [-1, 1]$,
        $\frac \beta \delta \abs x^{2\delta} \leq \abs{h_k'(\sign(x)x^2)} \leq \frac \alpha \gamma \abs x^{2\gamma}$.
        \item \label{lem:F-rb-impl:item:defn-equiv}
        For every $x \in [-1, 0) \cup (0, 1]$, $\beta \abs x^{2\delta-2} \leq \abs{h_k''(\sign(x)x^2)} \leq \alpha \abs x^{2\gamma-2}$
    \end{compactenum}
\end{lem}
\begin{proof}
    Using the symmetries from \cref{assumpt:gsymmetries}, it suffices to consider $x \geq 0$.

    To see part~\ref{lem:F-rb-impl:item:defn-equiv}, we apply \cref{defn:BEF-robust} to $h_k''(x^2)$ to obtain $\beta x^{2(\delta - 1)} \leq \abs{h_k''(x^2)} \leq \alpha x^{2(\gamma - 1)}$ on $x > 0$.

    For part~\ref{lem:F-rb-impl:item:2}, we use that $h_k'(0) = 0$ by \cref{assumpt:deriv0} to obtain that $h_k'(x) = \int_0^{x} h_k''(t) dt$.
    Further, since $h_k$ is either strictly convex or strictly concave on $[0, 1]$, it follows that the sign of $h_k''$ unchanging on $(0, 1]$.
    Thus, $\abs{h_k'(x)} = \int_0^{x} \abs{h_k''(t)} dt$.
    The upper bound is obtained as
    \begin{displaymath}
    \abs{h_k'(x^2)}
    \leq \int_0^{x^2} \alpha t^{\gamma - 1} dt
    = \frac \alpha \gamma t^{\gamma}\Big|_{t=0}^{t=x^2}
    = \frac \alpha \gamma x^{2\gamma} \ .
    \end{displaymath}
    By similar reasoning (replacing $\leq$ with $\geq$, $\gamma$ with $\delta$, and $\alpha$ with $\beta$) we obtain that $\abs{h_k'(x^2)} \geq \frac \beta \delta x^{2\delta}$.

    To obtain parts~\ref{lem:F-rb-impl:item:1} and \ref{lem:F-rb-impl:item:1-5}, we use the formulas from \cref{lem:h-g-relations} to express the derivatives of $g_k$ as $g_k'(x) = 2h_k'(x^2)x$ and $g_k''(x) = \indicator{x \neq 0}[4h_i''(x^2)x^2 + 2h_i'(x^2)]$.
    By part~\ref{lem:F-rb-impl:item:2}, we obtain the desired bounds on $g_k'(x)$.
    We note that
    \begin{displaymath}
    \abs{g_k''(x)}
    \leq 4 \alpha x^{2\gamma} + 2 \frac \alpha \gamma x^{2\gamma}
    \leq 2\alpha (2 + 1 / \gamma) x^{2\gamma} \ .
    \end{displaymath}
    Note that $h_i''(x)$ and $h_i'(x)$ share the same sign on $(0, x]$ (see \cref{lem:h-props} and recall that $h_i$ is convex if $h_i'' \geq 0$ on its domain and concave if $h_i'' \leq 0$ on its domain).
    As such,
    \begin{displaymath}
    \abs{g_k''(x)}
    = \indicator{x \neq 0} \abs{4h_k''(x^2)x^2 + 2h_k'(x^2)}
    \geq 4 \beta x^{2\delta} + 2 \frac \beta \delta x^{2\delta}
    \geq 2 \beta (2+1/\delta) x^{2\delta} \ .
    \end{displaymath}

    To obtain part~\ref{lem:F-rb-impl:item:monomials}, we first find bounds for $h_k$.
    Since $h_k'$ is strictly monotonic and $h_k'(0) = 0$, it follows that $\abs{h_k(x)} = \int_0^x \abs{h_k'(t)} dt$.
    We obtain the upper bound as:
    \begin{align*}
    \abs{g_k(x)}
    &= \abs{h_k(x^2)}
    = \int_0^{x^2} \abs{ h_k'(t) } dt \\
    &\leq \frac \alpha \gamma \int_0^{x^2} t^{\gamma} dt
    = \frac{\alpha}{(\gamma + 1)\gamma} t^{\gamma+1} \bigr|_{t = 0}^{t = x^2}
    = \frac{ \alpha}{(\gamma + 1)\gamma} x^{2\gamma + 2} \ .
    \end{align*}
    The lower bound is obtained in a similar manner.
\end{proof}

\begin{lem}\label{lem:fg-upper-bounds}
    If $F$ is $(\alpha, \beta, \gamma, \delta)$-robust, then its gradient is bounded as follows for any $\vec u \in S^{\dn - 1}$.
    \begin{compactenum}
        \item\label{bound:gradf-upper2}
        Let $\SS \subset [\dn]$.
        Then, $\norm{\Pmap_\SS \nabla F(\vec u)} \leq \frac{2\alpha} \gamma \norm{\Pmap_{\SS \cap [\dm]} \vec u}^{1+2\gamma}$.
        \item\label{bound:gradf-lower}
        Let $S \subset [\dn]$.
        Then, $\norm{\Pmap_\SS \nabla F(\vec u)} \geq \frac {2\beta} \delta \norm{\Pmap_{\SS \cap [\dm]} \vec u}^{1+2\delta} / \abs {\SS \cap [\dm]}^{\delta}$.
    \end{compactenum}
\end{lem}
\begin{proof}
    We first prove part~\ref{bound:gradf-upper2}.  We let $A = \SS \cap [\dm]$.
    \begin{align*}
    \norm{\Pmap_{\SS} \nabla F(\vec u)}^2
    &= \sum_{i \in A} g_i'(u_i)^2
    \leq \sum_{i \in A} \left(2\frac{\alpha}{\gamma} \abs{u_i}^{1+2\gamma}\right)^2 \\
    &= 4\frac{\alpha^2}{\gamma^2} \norm{\Pmap_A \vec u}^{2+4\gamma}\sum_{i \in A} \biggr(\frac{u_i^2}{\norm{\Pmap_A \vec u}^2}\biggr)^{1+2\gamma} \ .
    \end{align*}
    In the above, the inequality uses \cref{lem:F-robust-implications} part~\ref{lem:F-rb-impl:item:1}.
    For each $i \in A$, $u_i^2/\norm{\Pmap_A\vec u}^2 \leq 1$ holds.
    Since $\gamma > 0$, it follows that $(u_i^{2} / \norm{\Pmap_A \vec u}^2)^{1+2\gamma} \leq u_i^{2} / \norm{\Pmap_A \vec u}^2$.
    Thus,
    \begin{displaymath}
    \norm{\Pmap_{\SS} \nabla F(\vec u)}^2
    \leq 4\frac{\alpha^2}{\gamma^2} \norm{\Pmap_A \vec u}^{2+4\gamma} \sum_{i \in A} \frac{u_i^2}{\norm{\Pmap_A \vec u}^2}
    = 4\frac{\alpha^2}{\gamma^2} \norm{\Pmap_A \vec u}^{2+4\gamma}  \ .
    \end{displaymath}

    We now prove part~\ref{bound:gradf-lower}.
    We let $A = \SS \cap [\dm]$, and we note:
    \begin{displaymath}
    \norm{\Pmap_{\SS} \nabla F(\vec u)}^2
    = \sum_{i \in A} g_i'(u_i)^2
    \geq \sum_{i \in A} \left(\frac{2\beta}{\delta} \abs{u_i}^{1+2\delta}\right)^2
    = \frac{4 \beta^2}{\delta^2} \abs{A}\sum_{i \in A} \frac{1}{\abs A}\bigr(u_i^2\bigr)^{1+2\delta} \ .
    \end{displaymath}
    In the above, the inequality uses \cref{lem:F-robust-implications}.
    But by Jensen's inequality, we see that
    \begin{displaymath}
    \sum_{i \in A} \frac{1}{\abs A}\bigr(u_i^2\bigr)^{1+2\delta}
    \geq \biggr(\sum_{i \in A} \frac{1}{\abs A}u_i^2\biggr)^{1+2\delta}
    = \biggr(\frac{\norm{\Pmap_A \vec u}^2}{\abs A}\biggr)^{1+2\delta}
    \end{displaymath}
    Thus, $\norm{\Pmap_{\SS} \nabla F(\vec u)}^2 \geq 4(\beta/\delta)^2 (\norm{\Pmap_A \vec u}^{2+4\delta})/\abs A^{\delta}$.
    Taking square roots gives the desired bound.
\end{proof}

\begin{lem}\label{lem:nablaF-pert-error}
    Suppose that $\vec u, \vec w \in \overline{B(0, 1))}$.
    Then, $\norm{\nabla F(\vec  u) - \nabla F(\vec w)} \leq 2(1+\frac 1 \gamma) \alpha \norm{\vec u - \vec w}$.
\end{lem}
\begin{proof}
    The proof is by the fundamental theorem of calculus and Minkowski's inequality for integrals:
    \begin{align*}
    \norm{\nabla F(\vec u) - \nabla F(\vec w)}
    &= \Norm{ \int_0^1 \HH F(t \vec u + (1-t) \vec w)(\vec u - \vec w) dt  } \\
    & \leq \int_0^1 \norm{\HH F(t \vec u + (1-t) \vec w)} \norm{\vec u - \vec w} dt \\
    & \leq 2\left(2 + \frac 1 \gamma\right)\norm{\vec u - \vec w} \ .
    \end{align*}
    In the last inequality, we note that for any $\vec p \in \overline{\vec u \vec w}$, $\HH F(\vec p)$ is a diagonal matrix, that as such $\norm {\HH F(\vec p)} \leq \max_{i \in \dn}\abs{[\HH F(\vec p)]_{ii}} = \max_{i \in [\dn]}\abs{g_{i}''(p_i)} \leq 2(2 + \frac 1 \gamma) \alpha$ by \cref{lem:F-robust-implications}.
\end{proof}

\begin{lem}\label{lem:G-est-error}
    Let $\SS \subset [\dm]$.
    If $\norm {\Pmap_{\compl \SS} \vec u} \leq \frac 1 {\sqrt{2(1+2\delta)}}$ and $\epsilon \leq \frac \beta {2\delta \abs \SS^\delta}$ , then $\norm{ \hat \GG(\vec u) - \GG(\vec u)} \leq 4 \delta \abs \SS^\delta \epsilon / \beta$.
\end{lem}
\begin{proof}
    \begin{align*}
    \norm{\hat \GG(\vec u) - \GG(\vec u)}
    &= \Norm{\frac{ \pertgF(\vec u)}{\norm{\pertgF(\vec u)}}
        - \frac{\nabla F(\vec u)}{\norm{\nabla F(\vec u)}}} \\
    &\leq \Norm{\frac{\pertgF(\vec u) - \nabla F(\vec u)}{\norm{\pertgF(\vec u)}}
        + \frac{(\norm{\nabla F(\vec u)}-\norm{\pertgF(\vec u)})\nabla F(\vec u)}{\norm{\nabla F(\vec u)}\norm{\pertgF(\vec u)}}} \\
    &\leq \frac{2\epsilon}{\norm{\pertgF(\vec u)}}
    \leq \frac{2\epsilon}{\norm{\nabla F(\vec u)} - \epsilon}
    \end{align*}
    We apply \cref{lem:P0small-gradf-lower-bound} to see that $\norm{\nabla F(\vec u)} \geq \frac{\beta}{\delta \abs{\SS}^{\delta}}$.
    Using the bound on $\epsilon$, we obtain that $\norm{\nabla F(\vec u)} - \epsilon \geq \frac{\beta}{2\delta \abs{\SS}^{\delta}}$.
    Thus, $\norm{\hat \GG(\vec u) - \GG(\vec u)} \leq 4 \delta \abs{\SS}^\delta \epsilon / \beta$ as desired.
\end{proof}

Note that perhaps the most interesting case of \cref{lem:G-est-error} is the case in which $\SS = [\dm]$.
In this case, the result simplifies to:
\emph{If $\norm{\Pmap_0 \vec u} \leq \frac{1}{\sqrt{2(1+2\delta)}}$ and $\epsilon \leq \frac{\beta}{2 \delta \dm^\delta}$, then $\norm{\hat \GG(\vec u) - \GG(\vec u)} \leq 4 \delta \dm^\delta \epsilon / \beta$}.

\begin{lem}\label{lem:G-lpert-error}
    Let $\vec u, \vec w \in S^{\dn - 1}$.
    Let $\SS \subset [\dm]$, and suppose that $\norm{\Pmap_{\compl \SS} \vec u} \leq \frac 1 {\sqrt {2(1+2\delta)} }$, and further suppose that $w_i \neq 0$ for some $i \in [\dm]$.
    Then, $\norm{\GG(\vec u) - \GG(\vec w)} \leq 2\frac \alpha
    \beta\delta(2+\frac 1 \gamma) \abs \SS^\delta \norm{\vec u - \vec w}$.
\end{lem}
\begin{proof}
    Since there exists $i \in [\dm]$ such that $w_i \neq 0$, it follows that  $\nabla F(\vec w) \neq \vec 0$.
    \begin{align*}
    \norm{\GG(\vec u) - \GG(\vec w)}
    &=\Norm{ \frac{\nabla F(\vec u)}{\norm{\nabla F(\vec u)}} - \frac{\nabla F(\vec w)}{\norm{\nabla F(\vec w)}} } \\
    &= \Norm{
        \frac{\norm{\nabla F(\vec w)}[\nabla F(\vec u) - \nabla F(\vec w)] + [\norm{\nabla F(\vec w)} - \norm{\nabla F(\vec u)}] \nabla F(\vec w) }{\norm{\nabla F(\vec u)} \norm{\nabla F(\vec w)}}
    } \\
    &\leq 2 \frac{\norm{\nabla F(\vec u) - \nabla F(\vec w)}}{\norm{\nabla F(\vec u)}} \ .
    \end{align*}
    By \cref{lem:P0small-gradf-lower-bound}, we have that $\norm{\nabla
        F(\vec u)} \geq \frac \beta \delta \abs \SS^{-\delta}$.
    Further, by \cref{lem:nablaF-pert-error}, we see that $\norm{\nabla
        F(\vec u) - \nabla F(\vec w)} \leq 2(2+\frac 1 \gamma) \alpha \norm{\vec u
        - \vec w}$.
    As such, we obtain that $\norm{\GG(\vec u) - \GG(\vec w)}
    \leq 2\frac \alpha \beta\delta(2+\frac 1 \gamma) \abs \SS^\delta
    \norm{\vec u - \vec w}$.
\end{proof}

In addition, the following is a useful Corollary to the \cref{lem:small-coord-decrease-step,lem:P0small-gradf-lower-bound}.
\begin{cor}\label{cor:tcompress}
    Let $\SS \subset [\dm]$ and let $A \subset [\dm]$ be non-empty.
    Suppose that $\vec u \in S^{\dn - 1}$ satisfies $\norm{\Pmap_{\compl A} \vec u} \leq \frac{1}{\sqrt{2(1+2\delta)}}$, and that $\epsilon \leq \frac \beta {2\delta}\dm^{-\delta}$.
    If for all $i \in \compl \SS \cap [\dm]$ that $\abs {u_i} \leq \tcompress$.
    Then, the following hold:
    \begin{compactenum}
        \item For all $i \in \compl \SS$, $\abs{\hat \GG_i(\vec u)} \leq \max( \frac 1 2 \abs{u_i}, 4 \delta\abs A^{\delta}\epsilon/\beta )$.
        \item $\norm{\Pmap_{\compl \SS} \hat \GG(\vec u)} \leq \max( \frac 1 2 \norm{\Pmap_{\compl \SS}\vec u}, 4 \delta\abs A^{\delta}\epsilon/\beta )$.
    \end{compactenum}
\end{cor}
\begin{proof}
    We note by \cref{lem:P0small-gradf-lower-bound}, $\norm{\nabla F(\vec u)} \geq \frac \beta \delta \abs A^{-\delta}$.
    Parts 1 and 2 follow by applying \cref{lem:small-coord-decrease-step} with the choice of $C = 1/2$ and with this lower bound for $\norm {\nabla F(\vec u)}$.
    For part 1, we apply \cref{lem:small-coord-decrease-step} to the set $\{i\}$, and for part 2 we apply \cref{lem:small-coord-decrease-step} to the set $\compl \SS$.
\end{proof}
Note that the most interesting cases of this corollary are when $A = \SS$ and when $A = [\dm]$.



\section{Miscellany}

In this section, we collect a number useful results and statements which are used in the proofs of the theorems of this paper.

% \begin{thm}[Inverse Function Theorem, based on Wikipedia article]
%   % Suppose that $M$ and $N$ are manifolds, that $f : M \rightarrow N$, and that $\Jacob F_p : T_pM \rightarrow T_{F(p)} M$ is a bijection.
%   Suppose that $f : \R^n \rightarrow \R^n$ is continuously differentiable on
%   an open set $\mathcal X \subset \R^n$.
%   If $\Jacob f_{\vec p}$ is non-singular (invertible) for some $\vec p \in \mathcal X$, the there exists a
%   neighborhood $U$ of $f(\vec p)$ on which the inverse function $f^{-1}$
%   exists and is continuously differentiable.
% \end{thm}

The following is a special case of Lemma 7.25 of~\mycitet{Rudin}{rudin1986real}.
\begin{thm}\label{thm:continuous-f-measure0}
  Let $U \subset \R^k$ be an open set.
  Suppose $f : V \rightarrow \R^k$ is differentiable on its entire domain.
  If $E \subset V$ has Lebesgue measure 0, then $f(E)$ has Lebesgue measure 0.
\end{thm}

\subsection{Rates of Convergence}
\label{sec:rates-convergence}

For reference, we recall here the definitions of various orders of convergence.

Let $\{\vec x_n\}_{n=0}^\infty$ be a sequence in a normed vector space that
converges to $L$.
If there exists $q \geq 1$ and $\mu \in (0, 1)$ such that
\begin{equation*}
  \lim_{n \rightarrow \infty} \frac{\norm{\vec x_{n+1} - L}}{\norm{\vec x_n - L}^q} = \mu,
\end{equation*}
then the sequence $\{\vec x_n\}_{n=0}^\infty$ is said to converge to $L$ with \text{order} $q$.
In the case where $q = 1$, convergence is said to be \textit{linear}.
If
\begin{equation*}
  \lim_{n \rightarrow \infty} \frac{\norm{\vec x_{n+1} - L}}{\norm{\vec x_n - L}} = 0,
\end{equation*}
then the rate of convergence is said to be \textit{superlinear}.

More generally, if there is a sequence $\{\epsilon_n\}_{n=0}^\infty$ in $\R$ such that $\epsilon_n$ converges to 0 with order $q$ (or superlinearly respectively) under the above definitions and if $\norm{\vec x_n - L} \leq \epsilon_n$ for all $n$, then we also say that $\vec x_n$ converges to $L$ with order at least $q$ (or superlinearly respectively).

\subsection{Error bounds on eigenvalues and eigenspaces}
\label{sec:error-bounds-eigenv}

We now recall some classic results about the perturbation of eigenvalues and eigenspaces.
The following inequality is a known version of Weyl's inequality for matrix eigenvalues.
\begin{thm}[Weyl's inequality]\label{thm:Weyls-inequality}
  Let $A$, $\tilde A$, and $H$ be symmetric (or more generally Hermitian) $n \times n$ matrices such that $\tilde A = A + H$.
  Let the eigenvalues of $A$, $\tilde A$, and $H$ be given by $\lambda_1, \dotsc, \lambda_n$, $\tilde \lambda_1, \dotsc, \tilde \lambda_n$, and $\rho_1, \dotsc, \rho_n$ respectively.
  Assume that the eigenvalues are indexed in decreasing order, i.e., $\lambda_1 \geq \cdots \geq \lambda_n$.
  Then, for each $i \in [n]$, $\lambda_i + \rho_i \leq \tilde \lambda_i \leq \lambda_i \rho_n$.
\end{thm}

The next Theorem (namely the  $\sin \Theta$ theorem of~\mycitet{Davis and Kahan}{davis1970rotation}) allows us to bound the error in eigenvector subspaces of a matrix under a perturbation.
This theorem requires a bit more explanation.
In particular, we will still assume that we have a Hermitian matrix $A$ which is the matrix we are interested in, and that $\tilde A = A + H$ is a perturbed version of $A$ (with $\tilde A$ and $H$ also both Hermitian).
Suppose that $A = \sum_{i=1}^n \lambda_i \vec v_i \vec v_i^T$ and $\tilde A \sum_{i=1}^n \tilde \lambda_i \tilde {\vec v_i} \tilde {\vec v_i}^T$ give eigendecompositions with the ordering of the eigenvalues $\lambda_i$ not yet determined.
We may split the indices at a point $k$ and define the matrices $A_0 = \sum_{i=1}^k \lambda_i \vec v_i \vec v_i^T$, $A_1 = \sum_{i=k+1}^n \lambda_i \vec v_i \vec v_i^T$, $\tilde A_0 = \sum_{i=1}^k \tilde \lambda_i \tilde {\vec v_i}\tilde{ \vec v_i}^T$, $\tilde A_0 = \sum_{i=k+1}^m \tilde \lambda_i \tilde {\vec v_i}\tilde{ \vec v_i}^T$.
\begin{thm}[Davis-Kahan $\sin \Theta$ theorem]\label{thm:sin-theta-thm}
  Suppose that there exists an interval $[\alpha, \beta]$ and a $\Delta > 0$ such that the eigenvalues of $A_0$ lie within $[\alpha, \beta]$ and the eigenvalues of $\tilde A_1$ all lie outside the interval $(\alpha - \Delta, \beta + \Delta)$ [or alternatively, the eigenvalues of $\tilde A_1$ lie within $[\alpha, \beta]$ and the eigenvalues of $A_0$ all lie outside the interval $(\alpha - \Delta, \beta + \Delta)$].
  Then, $\Delta \norm{\sin \Theta_0} \leq \norm H$.
  % \vnote{Technically, the statement is given in terms of a residual $R$ rather than $H$, but see discussion at the top of page 7 of \mycitet{Davis and Kahan}{davis1970rotation}, and note that $R = H E_0$ in their notation with the norm $\norm{\cdot}$ being unitary invariant.  $E_0$ is just an eigenspace corresponding to the eigenvalues of $A_0$.  As such, $\norm{R} \leq \norm{H}$.}
\end{thm}
The definition of $\sin \Theta_0$ is somewhat involved (see \citep{davis1970rotation} for details).
 In our setting it suffices to note that $\norm{\sin \Theta_0}$ bounds certain projection operators.
In particular, if $\Pi_0 = \sum_{i=1}^k \vec v_i \vec v_i^T$ and $\tilde \Pi_0 = \sum_{i=1}^k \tilde{\vec v_i} \tilde{\vec v_i}^T$, then $\norm{(\Id-\tilde \Pi_0) \Pi_0} \leq \norm{\sin \Theta_0} \leq \frac 1 \Delta \norm H$.

\subsection{Concentration and anti-concentration of the $\chi^2$ distribution}
The following bounds are a direct implication of~\citep[Lemma 1]{laurent2000adaptive}.
\begin{lem}\label{lem:chi2-concentration}
  Let $Z$ be distributed according to the $\chi^2$ distribution with $D$ degrees of freedom.
  Then, for all $x > 0$, the following hold:
  \begin{compactenum}
  \item $\Pr[Z - D \geq 2\sqrt{Dx} + 2x] \leq \exp(-x)$.
  \item $\Pr[D - Z \geq 2\sqrt{Dx}] \leq \exp(- x)$.
  \end{compactenum}
\end{lem}

We have the following Corollary, which is useful in our error analysis.
\begin{cor}\label{cor:chi2-concentration}
    There exists universal constant $C > 0$ such that the following holds:
    Let $Z$ be distributed according to the $\chi^2$ distribution with $D$ degrees of freedom.
    Then,
    \begin{compactenum}
      \item
       $\Pr[Z \geq 2D] \leq \exp(- \frac{2-\sqrt 3}{2} D)$.
      \item $\Pr[Z \leq \frac 1 2 D] \leq \exp(-\frac 1 {16} D)$.
    \end{compactenum}
     with probability at least $\exp(-C D)$,
\end{cor}
\begin{proof}
    We first prove part 1.
    We note that
    \begin{displaymath}
        \Pr[Z \geq 2D] = \Pr[Z - D \geq D]
    \end{displaymath}
    In order to apply \cref{lem:chi2-concentration}, we need to choose $x$ such that $2\sqrt{Dx} + 2x = D$.
    That is, $2\sqrt{Dx} + 2x - D = 0$.
    But by the quadratic formula, it follows that
    \begin{displaymath}
        \sqrt x
        = \frac{-2\sqrt D + \sqrt{4 D + 8 D}}{4}
        = \frac{\sqrt 3 - 1}{2}\sqrt D \ .
    \end{displaymath}
    Squaring both sides yields $x = \frac{2-\sqrt 3}{2}D$.

    In order to prove part 2, we note that $\Pr[Z \leq \frac 1 2 D] = \Pr[D - Z \geq \frac 1 2 D]$.
    We apply \cref{lem:chi2-concentration} with the choice of $x$ such that $2\sqrt{D x} = \frac 1 2 D$, which is to say $x = \frac{1}{16} D$.
\end{proof}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> simplexframework - Copy/gi-error-nohes.tex <==
\section{Gradient Iteration Under a Perturbation}
\label{sec:gi-error-analysis}

\begin{algorithm}[tb]
  \caption[GI-Loop]{\label{alg:GI-LOOP} Perform the gradient iteration for a predetermined number of iterations.
    The inputs are %$\hat \GG$ (the Gradient iteration function handle),
    $\vec u(0)$ (an initialization vector) and $N$ (the number of iterations).
    The output is $\vec u(N)$ (the $N$\textsuperscript{th} element of the resulting gradient iteration sequence).
  }
  \begin{algorithmic}
  \Function{GI-Loop}{$\vec u(0), N$}
  \For{$n\leftarrow 1$ to $N$}
  \State $\vec u(n) \leftarrow \hat \GG(\vec u(n-1))$
  \EndFor
  \State \Return $\vec u(N)$
  \EndFunction
  \end{algorithmic}
\end{algorithm}

\begin{algorithm}[tb]
  \caption[\textsc{FindBasisElement}]{\label{alg:SingleRecovery}
    A robust extension to the gradient iteration algorithm for guaranteed recovery of a single hidden basis element.}
    Inputs:\\
    \begin{tabularx}{\linewidth}{lX}
    $\{\gvec \mu_1, \dotsc, \gvec \mu_k\}$ & A (possibly empty) set of approximate hidden basis directions.  \\
    $\sigma$ & Positive parameter determining jump size to break stagnation of $\hat \GG$. \\
    $\pertgF$ & Function pointer to our estimate of $\nabla F$.  $\hat \GG$ is also being implicitly defined from this in our pseudo-code. \\
    $N_1$, $N_2$, $I$ & Parameters which determine total loop iterations.
    \end{tabularx}\\
    Outputs: An approximate basis element not estimated by any of $\gvec \mu_1, \dotsc, \gvec \mu_k$.
  %   \begin{tabular}{ll}
  %   $\gvec \nu \qquad\qquad\quad$ & An approximate basis element not estimated by any of $\gvec \mu_1, \dotsc, \gvec \mu_k$.
  % \end{tabular}
    \hrule
  \NumTabs{2}
  \begin{algorithmic}[1]
    \Function{FindBasisElement}{$\{\gvec \mu_1, \dotsc, \gvec \mu_k\}$, $\sigma$, $\pertgF$, $N_1$, $N_2$, $I$}
      \State // Find a starting vector sufficiently outside the subspace $\spn(\myZv_{\dm + 1}, \dotsc, \myZv_\dn)$.
      \State \label{alg:step-xi-spread} Let $\vec x_1, \dotsc, \vec x_{\dn - k}$ be orthonormal vectors in $\spn(\gvec \mu_1, \dotsc, \gvec \mu_k)^\perp$.
      \State\label{alg:step:best-xi} $j \leftarrow \argmax_{i \in [\dn-k]} \norm{\pertgF(\vec x_i)}$
      \State\label{alg:step:zero-nonbasis-coords}
        $\vec u \leftarrow \hat \GG(\vec x_j)$ \tab // ``Zero'' the values of $u_{m+1}, \dotsc, u_\dn$.
        % \State\label{alg:step:zero-nonbasis-coords2}
        % $\vec u \leftarrow \hat \GG(\vec u)$
        \State\label{alg:step:zero-nonbasis-coords2}
        $\vec u \leftarrow \Call{GI-Loop}{\vec u, N_1}$
        % \hfill // ``Zero'' coordinates corresponding to directions $\gvec \mu_1, \dotsc, \gvec \mu_k$.
      %\For{$i\leftarrow 1$ to $\hat \dm - k - 1$}
      \For{$i\leftarrow 1$ to $I$}
        \tab // Start of the main loop
        \State\label{alg:step:draw-jump}
        Draw $\vec x$ uniformly at random from $\sigma \sphere^{\dn - 1} \cap \vec u^\perp$ %$\mathcal N(\vec 0, \sigma^2 \Pmap_{\vec u^\perp})$
        \State\label{alg:step:jump1}
        $\vec w \leftarrow \vec u \cos(\norm{\vec x}) + \frac{\norm{\vec x}}{\vec x}\sin(\norm{\vec x})$
        \tab // A random jump from $\vec u$
        \State\label{alg:step:gi-in-main-loop}
            $\vec u \leftarrow \textsc{GI-Loop}(\vec w, N_2)$
            %$\vec u \leftarrow \textsc{GI-Loop}(\vec u \cos(\norm{\vec x}) + \frac{\norm{\vec x}}{\vec x}\sin(\norm{\vec x}), N_2)$
            \EndFor
      \State\label{alg:step:exit}
          \Return $\vec u$
    \EndFunction
  \end{algorithmic}
\end{algorithm}

\begin{algorithm}[tbh]
  \caption[\textsc{RobustGI-Recovery}]{\label{alg:FullRecovery}
    A robust algorithm to recover approximations to all of the hidden basis elements.
  }
    Inputs:\\
    \begin{tabularx}{\linewidth}{lX}
    $\hat \dm\qquad\qquad$
    & The desired number of basis elements to recover.  It is required that $\hat \dm \geq \dm$. \\
    $\sigma$ & Parameter determining perturbation noise added to escape near ``stationary points'' of $\hat \GG$. \\
    $\pertgF$ & Function pointer to our estimate of $\nabla F$.  $\hat \GG$ is also being implicitly defined from this in our pseudo-code. \\
    $N_1$, $N_2$, $I$ & Parameters which determine total loop iterations.
    \end{tabularx}\\
    Outputs:\\
    \begin{tabular}{ll}
    $\gvec \mu_1, \dotsc, \gvec \mu_{\hat \dm}$
    & The first $\dm$ of these are approximate hidden basis elements.
    \end{tabular}\hrule
  \begin{algorithmic}[1]
    \Function{RobustGI-Recovery}{$\hat \dm$, $\sigma$, $\pertgF$, $N_1$, $N_2$, $I$}
    \For{$i \leftarrow 1$ to $\hat \dm$}
      \State $\gvec \mu_i \leftarrow$ \Call{FindBasisElement}{$\{\gvec \mu_1, \dotsc, \gvec \mu_{i-1}\}$, $\sigma$, $\pertgF$, $N_1$, $N_2$ $I$}
    \EndFor
    \State \Return $\gvec \mu_1, \dotsc, \gvec \mu_{\hat \dm}$
    \EndFunction
  \end{algorithmic}
\end{algorithm}

In \cref{sec:gi-stability-structure}, we saw that the hidden basis
elements $\myZv_i$ are attractors, that convergence to this set of attractors
is guaranteed except on a set of measure 0, and that the rate of convergence is super-linear.
In this section, we provide a robust extension to the gradient iteration
algorithm for recovering all of the hidden basis elements.
We demonstrate that for a wide class of contrasts, the recovery process is
robust to a perturbation, and that the hidden basis elements $\myZv_1, \dotsc,
\myZv_\dm$ can be efficiently recovered given approximate access to $\nabla F$.

To provide quantifiable algorithmic bounds, we require quantifiable
assumptions upon the hidden convexity (or concavity) of the $h_i$ functions
associated with $F$.
For smooth functions, convexity is characterized by the second derivative of
the function.
%In order to place bounds upon the hidden convexity of our transformed
% contrasts $h_k$,
In particular, we use the following notion of robustness.
\begin{defn}\label{defn:BEF-robust}
  Let $\alpha$, $\beta$, $\gamma$, and $\delta$ be strictly positive constants, and let $D \subset \R$.
  A contrast function $g : D \rightarrow \R$ satisfying \crefrange{assumpt:first}{assumpt:last} is said to be \emph{$(\alpha, \beta, \gamma, \delta)$-robust}\index{contrast function!robust} if for all $x > 0$, $\beta \abs x^{\delta - 1} \leq \Abs{\frac {d^2}{dt^2}[g(\sqrt t)]\big|_{t = x}} \leq \alpha \abs x^{\gamma - 1}$.
  Further, \ansef\@ $F(\vec u) = \sum_{i = 1}^\ldim g_i(\ipCanonical{\vec u}{\hbev_i})$ is said to be \emph{$(\alpha, \beta, \gamma, \delta)$-robust}\index{Basis Encoding Function!robust orthogonal} if each of its contrast functions $g_i$ are $(\alpha, \beta, \gamma, \delta)$-robust on the domain $[-1, 1]$.
\end{defn}

This definition is designed to capture a broad class of functions of interest.
For instance, we capture monomials of the form $p_{a, r}(x) = \frac{a}{(r+1)r}x^{2r+2}$ on $[0, 1]$ where $r > 0$ and $a > 0$ are real (with either positive or negative reflections of this on $[-1, 0]$.
Indeed, the robustness criterion in \cref{defn:BEF-robust} may alternatively be stated as
$\frac{d^2}{dt^2}(p_{\beta, \delta}(\sqrt t))\bigr|_{t = x}
\leq \Abs{\frac {d^2}{dt^2}[g(\sqrt t)]\big|_{t = x}}
\leq \frac{d^2}{dt^2}(p_{\alpha, \gamma}(\sqrt t))\bigr|_{t = x}$ for all $x > 0$ in the domain of $g$.
In particular, the monomial functions $ax^r$ with $r \geq 3$ an integer which arise in the setting of orthogonal tensor decompositions are captured as a special case.

\Cref{defn:BEF-robust} provides several natural condition numbers which arise in our analysis.

\begin{rmk}\label{rmk:condition-nums-robust-BEF}
  If $F$ is $(\alpha, \beta, \gamma, \delta)$-robust, then $\alpha \geq \beta$ and $\gamma \leq \delta$.
\end{rmk}
\begin{proof}
  To see that $\alpha \geq \beta$, we note that $\alpha x^{\gamma-1} \geq \beta x^{\delta - 1}$ holds at $x = 1$.
  To see that $\gamma \leq \delta$, we note that asymptotically as $x \rightarrow 0$ from the right, $\beta x^{\delta - 1} = O(x^{\gamma - 1})$.
\end{proof}
Under \cref{rmk:condition-nums-robust-BEF}, we see that $\frac \alpha \beta$ and $\frac \delta \gamma$ are both lower bounded by $1$.
These ratios will act as condition numbers in our time and error bounds.

For the remainder of this section, we will assume that $F$ is $(\alpha, \beta, \gamma, \delta)$-robust unless otherwise specified.
Hatted objects such as $\pertgF$ and $\hat \GG$ will represent the natural estimates of un-hatted objects, and in particular $$\hat \GG(\vec u) := \begin{cases}
\pertgF(\vec u)/\norm{\pertgF(\vec u)} & \text{if } \pertgF(\vec u) \neq \vec 0 \\
\vec u & \text{otherwise}
\end{cases} \ .$$
For $\epsilon > 0$, we say that $\pertgF$ is an \emph{$\epsilon$-approximation} of $\nabla F$ if $\norm{\pertgF(\vec u) - \grad F(\vec u)} \leq \epsilon$ for all $\vec u \in \overline{B(0, 1)}$.
We assume (unless otherwise stated) throughout this section that $\pertgF$ is an $\epsilon$-approximation of $\nabla F$ with any bounds on $\epsilon$ being made clear by context.

We will see that under these assumptions, we are able to recover approximations of hidden basis elements using \textsc{FindBasisElement} (\cref{alg:SingleRecovery}).
We use the following notion of recovery since we do not care about the ordering or the sign associated with the original hidden basis.
\begin{defn}
  Consider the distance $d(\vec u, \vec v) := \min(\norm{\vec u - \vec v},
  \norm{-\vec u - \vec v})$.
  We say that $\tilde \myZv_1, \dotsc, \tilde \myZv_k$ is an
  \emph{$\epsilon$-recovery} of the basis $\myZv_1, \dotsc, \myZv_k$ if
  there exists a permutation $\pi$ of $[k]$ such that $d(\tilde \myZv_i,
  \myZv_{\pi(i)}) \leq \epsilon$ for all $i \in [k]$.
\end{defn}
If we have approximately recovered several hidden basis elements using \textsc{FindBasisElement}, then we may use \textsc{FindBasisElement} to approximately recover a new hidden basis element.
% The recovery takes into account previously found basis elements.
% In particular, if $\myZv_{i_1}, \dotsc, \myZv_{i_k}$ are approximated by $\gvec \mu_1, \dotsc, \gvec \mu_k$, then \textsc{FindBasisElement} approximately recovers a hidden basis element $\myZv_{i_{k+1}}$ such that $i_{k+1} \in [\dm] \setminus \{i_1, \dotsc, i_k\}$.
In particular, \textsc{FindBasisElement} may be run repeatedly to recover all hidden basis elements.
Formally, we have the following result.


For clarity, we will denote by $C_0, C_1, C_2, \dotsc$ positive universal constants in the main theorem statements.
These can represent different constant values in different theorem statements.
% If a $C_i$ appears in two different theorems or lemmas, it can represent distinct universal constants.
\begin{thm}\label{thm:single-recovery-main}
  Suppose that
  \begin{compactitem}
  \item $\epsilon \leq C_1 4^{-\frac{4+2\delta}{\gamma}}\frac{\sigma \beta}{\delta}\big[\frac {\beta\gamma}{\alpha \delta} \big]^{\frac{4\delta + 7}{2\gamma}}\dm^{-\frac \delta \gamma(2\delta - \gamma + \frac 7 2)}\dn^{-\frac 1 2 - \delta}$,
  \item $\sigma \leq \frac{C_0}{\sqrt{\dn(1+\delta)}} \big[ \frac {\beta\gamma}{16\alpha\delta}\big]^{\frac 1 \gamma}\dm^{-\frac \delta \gamma}$,
  \item $N_1 \geq C_2 \lceil \log_{1+2\gamma}(\log_2(\frac{\beta}{\delta \epsilon}))\rceil$, and
  \item $N_2 \geq C_3\bigr\lceil 4^{\frac 2 \gamma}\frac{\sqrt \dn}{\sigma} (\frac{\alpha\delta}{\beta\gamma})^{\frac {\delta+2} \gamma}\dm^{\frac \delta \gamma(\delta - \gamma + 2)}[\frac 1 \gamma \log(\frac{\alpha \delta}{\beta \gamma}) + \frac \delta \gamma \log(\dm)]\bigr\rceil \newline \phantom{.}\qquad \ + C_2 \lceil \log_{1+2\gamma}(\log_2(\frac{\beta}{\delta \epsilon}))\rceil$.
  \end{compactitem}
  Let $p \in (0, 1)$.
  Suppose that $I \geq C_3 \dm \lceil \log(\dm / p) \rceil$,
  that $\gvec \mu_1, \dotsc, \gvec \mu_k$ is a $C_4 \delta \epsilon / \beta$-recovery of $\myZv_1, \dotsc, \myZv_k$
  % $\norm{\gvec \mu_i - \myZv_i} \leq C_4 \delta \epsilon / \beta$ for all $i \in [k]$,
  and that $k < \dm$.
  After executing
  \begin{displaymath}
    \gvec \mu_{k+1} \leftarrow
    \textsc{FindBasisElement}(\{\gvec \mu_1, \dotsc, \gvec \mu_k\}, \sigma, \pertgF, N_1, N_2, I) \ ,
\end{displaymath}
  then with probability at least $1 - p$, there exists $j \in \{k+1, k+2, \dotsc, \dm\}$ such that $\gvec \mu_{k+1}$ is a $C_4 \delta \epsilon / \beta$-recovery of $\myZv_j$.
\end{thm}

\textsc{FindBasisElement} operates as follows.
We first find a warm start $\vec u$ which is approximately contained in $\spn(\gvec \mu_1, \dotsc, \gvec \mu_k)$ for which $\norm{\Pmap_0 \vec u}$ is small.
Then, we enter the main loop.
There are three main ideas underlying the main loop and its analysis:
\paragraph{Small Coordinates Decay Rapidly}
There exists a threshold $\tau > 0$ such that if $i \in [\dm]$ satisfies that $\abs{u_i} \leq \tau$, then when applying the gradient iteration $\abs{\hat \GG_i(\vec u)} \leq C \abs{u_i}$ (with $C < 1$) unless $u_i$ is already on the order of $\epsilon$.
We call coordinates of $\vec u$ small if they are below such a threshold and large if they are above it.
This constant $C$ actually gets smaller as the $u_i$ gets smaller, and we are able to see that the small coordinates of $\vec u$, and we see super-exponential decay in the small coordinates of $\vec u$.
This super-exponential decay is seen in the lower bound on $N_1$, which interestingly includes the only dependency on $\epsilon$ seen in the running time of \textsc{FindBasisElement}.
This phenomenon is analyzed in \cref{sec:small-coord-analysis}.

\paragraph{The Big Become Bigger}
During the execution of step~\ref{alg:step:gi-in-main-loop}, we may consider a fixed point $\vec v$ of $\GG / {\sim}$ such that $v_i \neq 0$ if and only if $i$ corresponds to a large coordinate of $\vec w$.
Similarly to what was seen before in \cref{prop:gi-expand-all} in the exact case, if there is an $i$ such that $w_i > v_i$ with a sufficient gap, then the gradient iteration drives one of the large coordinates to become small.
The remaining large coordinates become bigger to compensate.
When finally only one hidden coordinate of $\vec u$ remains big, we have recovered an approximate hidden basis element.
This phenomenon is analyzed in \cref{sec:large-coord-analysis-1}.

\paragraph{Jumping Out of Stagnation}
It is possible for the gradient iteration to stagnate.
In particular, this can occur as follows.
If $\SS \subset [\dm]$ is the set of large coordinates, $\vec v$ is the fixed point of $\GG / {\sim}$ such that $v_i \neq 0$ if and only if $i \in \SS$, and if $\abs{u_i} \leq \abs{v_i}$ (or under the perturbed setting, $\abs{u_i}$ is not sufficiently larger than $\abs{v_i}$ from the unperturbed setting), then the large coordinate progress from the preceding paragraph is not guaranteed.
However, by taking a small random jump from $\vec u$ as is done in steps~\ref{alg:step:draw-jump} and~\ref{alg:step:jump1} of \textsc{FindBasisElement}, then with at least constant probability, we can make one of the large coordinates of $\vec u$ sufficiently greater than the corresponding coordinate of $\vec v$.
Then, the large coordinate analysis from the preceding paragraph applies.
It is from this interplay between the big becoming bigger and the jumping out of stagnation that we are able guarantee with probability $1-\Delta$ that $O(\dm \log(\dm / \Delta))$ iterations of the main loop suffice to drive all but one of the hidden coordinates of $\vec u$ to 0, and hence producing an approximation to one of the hidden basis elements.
This jumping phenomenon is analyzed in \cref{sec:perturb-step-analysis}.

Finally, in \textsc{RobustGI-Recovery} (\cref{alg:FullRecovery}), we run \textsc{FindBasisElement} until all hidden basis elements are well approximated.
More formally, we have the following result.
\begin{thm}\label{thm:full-recovery-main}
  Suppose that
  \begin{compactitem}
  \item $\sigma \leq \frac{C_0}{\sqrt{\dn(1+\delta)}} \big[ \frac {\beta\gamma}{16\alpha\delta}\big]^{\frac 1 \gamma}\dm^{-\frac \delta \gamma}$,
  \item $\epsilon \leq C_1 4^{-\frac{4+2\delta}{\gamma}}\frac{\sigma \beta}{\delta}\big[\frac {\beta\gamma}{\alpha \delta} \big]^{\frac{4\delta + 7}{2\gamma}}\dm^{-\frac \delta \gamma(2\delta - \gamma + \frac 7 2)}\dn^{-\frac 1 2 - \delta}$,
  \item $N_1 \geq C_2 \lceil \log_{1+2\gamma}(\log_2(\frac{\beta}{\delta \epsilon}))\rceil$, and
  \item $N_2 \geq C_3\bigr\lceil 4^{\frac 2 \gamma}\frac{\sqrt \dn}{\sigma} (\frac{\alpha\delta}{\beta\gamma})^{\frac {\delta+2} \gamma}\dm^{\frac \delta \gamma(\delta - \gamma + 2)}[\frac 1 \gamma \log(\frac{\alpha \delta}{\beta \gamma}) + \frac \delta \gamma \log(\dm)]\bigr\rceil \newline \phantom{.}\qquad \ + C_2 \lceil \log_{1+2\gamma}(\log_2(\frac{\beta}{\delta \epsilon}))\rceil$.
  \end{compactitem}
  Let $p \in (0, 1)$,
  and suppose that $I \geq C_3 \dm \lceil \log(\dm / p) \rceil$.
  If $\hat \dm \geq \dm$ and we execute $\gvec \mu_1, \dotsc, \gvec \mu_{\hat \dm} \leftarrow \textsc{RobustGI-Recovery}(\hat \dm, \sigma, \pertgF, N_1, N_2, I)$, then with probability at least $1-p$, $\gvec \mu_1, \dotsc, \gvec \mu_\dm$ is a $C_4\delta \epsilon / \beta$-recovery of $\myZv_1, \dotsc, \myZv_\dm$.
\end{thm}

To simplify the exposition, the proofs of \cref{thm:single-recovery-main,thm:full-recovery-main} are deffered to \cref{sec:proof-details-pert}.

We now consider the running time of \textsc{RobustGI-Recovery}.
First, $I$, $N_1$, and $N_2$ can be viewed as parameters controlling the running time of the algorithm.
More formally, we have the following result.
\begin{thm}\label{thm:running-time}
  Suppose that we are working in a computation model supporting the following operations:
  Basic arithmetic operations, square roots, and trigonometric functions on scalars, branches on conditional; inner products in $\R^\dn$; and computations of $\pertgF(\vec u)$.
  Then,
  \textsc{RobustGI-Recovery} runs in $O(\hat \dm( N_1 + I N_2 ) + \hat \dm \dn^2)$ time.
\end{thm}

To see the $O(\hat \dm\dn^2)$ portion of the upper bound on scalar and vector operations in \cref{thm:running-time}, we note that step~\ref{alg:step-xi-spread} of \textsc{FindBasisElement} can be implemented using Gram-Schmidt orthogonalization involving the $\gvec \mu_i$s and the canonical vectors in the ambient space.
When the desired number of basis elements $\dm$ is known, then $\hat \dm$ can be chosen as $\dm$.
When the number of basis elements is unknown, then $\hat \dm$ may be chosen as $\dn$, and in a more practical setting the values of $\norm{\pertgF(\gvec \mu_\ell)}$ may be thresholded to determine which returned vectors correspond to hidden basis elements.
% Our general bound on the running time for \textsc{RobustGI-Recovery} is stated as follows:
% To obtain the time bound seen in \cref{thm:main-informal}, we choose $N_1 = N_2$, we note that the main loop runs at most $\hat \dm^2$ times, and we use a somewhat larger, simplified lower bound for $\hat \dm^2 N_2 + C\hat \dm \dn^2$ as our lower bound for $N$ (with $C$ a constant).
% The $C\hat \dm \dn^2$ portion of this bound comes from step~\ref{alg:step-xi-spread}, which can be implemented using Gram-Schmidt orthogonalization involving the $\gvec \mu_i$s and canonical vectors in the ambient space.



In addition, we note that $\nabla F$ is an $\epsilon$-approximation to itself for any $\epsilon > 0$.
As such, \cref{thm:full-recovery-main} also implies a polynomial time algorithm for recovering each hidden basis element within a preset but arbitrary precision $\eta$.
In the following Corollary of \cref{thm:full-recovery-main}, we characterize the running time of \textsc{RobustGI-Recovery} as a function of the precision of the hidden basis estimate.
\begin{cor}\label{cor:robust-all-recovery-error-version}
  Suppose that
  \begin{compactitem}
  \item $\sigma \leq \frac{C_0}{\sqrt{\dn(1+\delta)}} \big[ \frac {\beta\gamma}{16\alpha\delta}\big]^{\frac 1 \gamma}\dm^{-\frac \delta \gamma}$,
  \item $\eta \leq C_1 4^{-\frac{4+2\delta}{\gamma}}\sigma \big[\frac {\beta\gamma}{\alpha \delta} \big]^{\frac{4\delta + 7}{2\gamma}}\dm^{-\frac \delta \gamma(2\delta - \gamma + \frac 7 2)}\dn^{-\frac 1 2 - \delta}$,
  \item $N_1 \geq C_2 \lceil \log_{1+2\gamma}(\log_2(\frac{1}{\eta}))\rceil$, and
  \item $N_2 \geq C_3\bigr\lceil 4^{\frac 2 \gamma}\frac{\sqrt \dn}{\sigma} (\frac{\alpha\delta}{\beta\gamma})^{\frac {\delta+2} \gamma}\dm^{\frac \delta \gamma(\delta - \gamma + 2)}[\frac 1 \gamma \log(\frac{\alpha \delta}{\beta \gamma}) + \frac \delta \gamma \log(\dm)]\bigr\rceil \\phantom{.}\qquad\ + C_2 \lceil \log_{1+2\gamma}(\log_2(\frac{1}{\eta}))\rceil$.
  \end{compactitem}
  Let $p \in (0, 1)$,
  and suppose $I \geq C_4 \dm \lceil \log(\dm / p) \rceil$.
  Suppose further that $\pertgF$ is a $C_5 \frac \beta \delta \eta$-approximation to $\nabla F$.
  If $\hat \dm \geq \dm$ and we execute
  \begin{displaymath}
    \gvec \mu_1, \dotsc, \gvec \mu_{\hat \dm} \leftarrow \textsc{RobustGI-Recovery}(\hat \dm, \sigma, \pertgF, N_1, N_2, I) \ ,
  \end{displaymath}
  then with probability at least $1-p$, $\gvec \mu_1, \dotsc, \gvec \mu_\dm$ is an $\eta$-recovery of $\myZv_1, \dotsc, \myZv_\dm$.
\end{cor}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> simplexframework - Copy/gi-error-proof-details.tex <==
In this appendix, we prove the theorem statements made in section~\ref{sec:gi-error-analysis} about our robust algorithm for hidden basis recovery.
We continue with the notation introduced in that section.
In addition, we will make use of several new notations in our analysis.

Given a $\SS \subset [\dn]$, we define the projection matrix $\Pmap_\SS := \sum_{i \in \SS} \myZv_i\myZv_i^T$.
In particular, this implies $\Pmap_\SS \vec u := \sum_{i \in \SS} u_i \myZv_i$.
We will denote the set complement by $\bar \SS := [\dn] \setminus \SS$.
Two projections will be of particular interest:  the projection onto the distinguished basis elements $\Pmap_{[\dm]} \vec u := \sum_{i=1}^\dm u_i \myZv_i$ and its complement projection which we will denote by $\Pmap_0 \vec u := \sum_{i=\dm + 1}^\dn u_i \myZv_i$.
In addition, if $\mathcal X$ is a subspace of $\R^\dn$, we will denote by $\Pmap_{\mathcal X}$ the orthogonal projection operator onto the subspace $\mathcal X$.
In particular, if $\SS \subset [\dn]$, then the operators $\Pmap_\SS$ and $\Pmap_{\spn(\{\myZv_i \suchthat i \in \SS\})}$ are identical.


\subsection{Small Coordinates Decay Rapidly}
\label{sec:small-coord-analysis}
We will be particularly interested in sequences under the gradient iteration, that is sequences of the form: $\{\vec u(n)\}_{n=0}^\infty$ defined recursively by $\hat \GG(\vec u(n)) = \vec u(n-1)$ and $\vec u(0) \in \sphere^{\dn -1}$.
In this section, we demonstrate two main things about sequences of this form:
First, $\norm{\Pmap_0 \vec u(n)}$ should rapidly become very small.
Second, for any $i \in [\dm]$ such that $u_i(0)$ has sufficiently small magnitude, then the gradient iteration should make $u_i(n)$ decay rapidly until it is very small.
Using these two ideas, we will be able to guarantee that under applications of gradient iteration, the number of hidden coordinates of $\vec u(n)$ which are near zero out can only increase.

We quantify these effects in the following Lemmas.
\Cref{lem:small-coord-decrease-step} characterizes how a single step of the gradient iteration makes $\norm{\Pmap_0 \vec u}$ and the small coordinates of $\vec u$ contract.
Then, \cref{lem:small-coord-decrease-time} expands upon \cref{lem:small-coord-decrease-step} to provide a bound on the number of steps required to decay the small coordinates of $\vec u(n)$ down to a magnitude of order $\epsilon$.

\begin{lem}\label{lem:small-coord-decrease-step}
  Fix $\vec u \in \sphere^{\dn - 1}$ such that $\epsilon < \frac 1 2 \norm{\nabla F(\vec u)}$.
  The following hold:
  \begin{enumerate}
    \item\label{lem:small-coord-trivial} $\norm{\Pmap_0\hat \GG(\vec u)} \leq \frac{2 \epsilon}{\norm{\nabla F(\vec u)}}$.
    \item\label{lem:small-coord-projection}
      Fix any $C \geq 0$.
      Let $\SS \subset [\dn]$ be such that $\abs{u_i} \leq \bigr[\frac {C\gamma}{8 \alpha} \norm{ \nabla F(\vec u) }\bigr]^{\frac 1 {2\gamma}}$ for all $i \in \SS \cap [\dm]$.
      Then, $\norm{\Pmap_{\SS} \hat \GG(\vec u)} \leq \max( C \norm{\Pmap_{\SS \cap [\dm]} \vec u}, \frac{4 \epsilon}{\norm{\nabla F(\vec u)}} )$.
  \end{enumerate}
\end{lem}
\begin{proof}
  Let $A \subset [\dn]$.
  Expanding $\norm{\Pmap_A \hat \GG(\vec u)}$ we obtain for each $i \in [\dn]$:
  \begin{equation} \label{eq:Gi-upper-bound-noassumpt}
    \norm{\Pmap_A \hat \GG(\vec u)}
    = \frac{\norm{\Pmap_A \pertgF(\vec u)}}{\norm{\pertgF(\vec u)}}
    \leq \frac{\norm{\Pmap_A \nabla F(\vec u)} + \epsilon}{\norm{\nabla F(\vec u)} - \epsilon} \ .
  \end{equation}
  As we assumed $\epsilon \leq \frac 1 2 \norm{\nabla F(\vec u)}$,
  \begin{equation}\label{eq:Gi-upper-1}
    \norm{\Pmap_A \hat \GG(\vec u)}
    \leq \frac{\norm{\Pmap_A \nabla F(\vec u)} + \epsilon}{\norm{\nabla F(\vec u)} - \frac 1 2 \norm{\nabla F(\vec u)}}
    = 2 \cdot \frac{\norm{\Pmap_A \nabla F(\vec u)} + \epsilon}{\norm{\nabla F(\vec u)}} \ .
  \end{equation}
  If $A = [\dn] \setminus [\dm]$, then $\Pmap_A \nabla F(\vec u) = 0$, and \cref{eq:Gi-upper-1} implies that $\norm{\Pmap_0 \hat \GG(\vec u)} = \norm{\Pmap_A \hat \GG(\vec u)} \leq \frac{2 \epsilon}{\norm{\nabla F(\vec u)}}$.

  We now prove part~\ref{lem:small-coord-projection}.
  If $\norm{\Pmap_\SS\nabla F(\vec u)} \leq \epsilon$, then \cref{eq:Gi-upper-1} implies that $\norm{\Pmap_\SS \hat \GG(\vec u)} \leq \frac{4 \epsilon}{\norm{\nabla F(\vec u)}}$.
  If $\epsilon \leq \norm{\Pmap_\SS\nabla F(\vec u)}$, then we obtain from \cref{eq:Gi-upper-1} that
    $\norm{\Pmap_\SS \hat \GG(\vec u)}
    \leq \frac{4 \norm{\Pmap_\SS\nabla F(\vec u)}}{\norm{\nabla F(\vec u)}}$.
  We expand $\norm{\Pmap_\SS \nabla F(\vec u)}$ to obtain:
  \begin{align*}
    \norm{\Pmap_{\SS} \nabla F(\vec u)}^2
    &= \sum_{i \in \SS} \abs{g_i'(u_i)}^2
    \leq \sum_{i \in \SS\cap [\dm]} (2\frac \alpha \beta \abs{u_i}^{1+2\gamma})^2 \\
    &\leq \sum_{i \in \SS\cap [\dm]} (2 \frac \alpha \beta \abs {u_i} \cdot \frac{C \gamma}{8 \alpha} \norm{\nabla F(\vec u)})^2
    \leq [\frac{C}{4}\norm{\nabla F(\vec u)}\norm{\Pmap_{\SS \cap [\dm]}\vec u}]^2 \ ,
  \end{align*}
  by using \cref{lem:F-robust-implications} for the first inequality and we use the upper bound on each $\abs{u_i}$ for the second inequality.
  It follows that $\norm{\Pmap_{\SS} \hat \GG(\vec u)} \leq C \norm{\Pmap_{\SS \cap [\dm]} \vec u}^2$.
  Whether $\epsilon \leq \norm{\Pmap_\SS \nabla F(\vec u)}$ or $\epsilon \geq \norm{\Pmap_\SS \nabla F(\vec u)}$, % we obtain our desired result that
  $\norm{\Pmap_\SS \hat \GG(\vec u)} \leq \max(C \norm {\Pmap_{\SS \cap [\dm]}\vec u},\allowbreak \frac{4 \epsilon}{\norm{\nabla F(\vec u)}})$ holds.
\end{proof}

\begin{lem}\label{lem:small-coord-decrease-time}
  Let $\{ \vec u(n) \}_{n=0}^\infty$ be a sequence in $\SS^{\dn-1}$ defined recursively by $\vec u(n) = \hat \GG(\vec u(n\nobreak-\nobreak 1))$.
  Let $L > 0$ be such that $\norm{\nabla F(\vec u(n))} \geq L$ for all $n \in \N$.
  Fix $\SS \subset [\dn]$.
  Suppose $\epsilon < \min\Big(\frac 1 2 L, \allowbreak \bigr(\frac{\gamma L^{1+2\gamma}}{8 \cdot 4^{2\gamma}\alpha}\bigr)^{\frac 1 {2\gamma}} \Big)$ and suppose there exists $C \in (0, 1)$ such that $\norm{ \Pmap_{\SS \cap [\dm]} \vec u(0)} \leq [\frac {C\gamma}{8 \alpha} L]^{\frac 1 {2\gamma}}$.
  If
  \begin{displaymath}
    N \geq
    \log_{1+2\gamma}\left(
      \log_{ \frac 1 C } \left(\frac{L \gamma}{8\alpha}\right)
      + 2\gamma \log_{ \frac 1 C } \left(\frac L {4\epsilon}\right)
    \right) \ ,
  \end{displaymath}
  is a positive integer,
  then for each $n \geq N$, $\norm{\Pmap_\SS \vec u(n)} \leq \frac{4 \epsilon}{L}$.
\end{lem}
\begin{proof}
  Let $N_0$ denote the least integer such that $\norm{\Pmap_\SS \vec u(N_0)} \leq \frac{ 4 \epsilon }{\norm{ \nabla F(\vec u)} }$ (or $\infty$ if it does not exist).
  Also, for compactness of notation, we define $A := \SS \cap [\dm]$.
  \begin{claim}\label{claim:small-coord-exponentiation}
    For each $n < N_0$, $\norm{\Pmap_{A} \vec u(n)} \leq [\frac \gamma {8 \alpha} C^{(1+2\gamma)^n} L]^{\frac 1 {2\gamma}}$.
    % \vnote{xxx TODO: Make this contain a $\sqrt{\abs{\SS \cap
    % [\dm]}}$ by allowing coordinate-wise leq in the original
    % formulation.  This will make the time barely worse (though still
    % log log) but will allow for smaller $\epsilon$ later. xxx}
  \end{claim}
  \begin{subproof}
    We proceed by induction on $n$.
    The base case of $n=0$ is true from the givens of this Lemma.
    We now choose $k < N_0 - 1$ and suppose that the claim holds for $n = k$.
    We see
    \begin{align*}
      \norm{\Pmap_\SS \vec u(k+1)}
      &\leq C^{(1+2\gamma)^k}\norm{\Pmap_{A} \vec u(k)}
      \leq C^{(1+2\gamma)^k}[\frac \gamma {8\alpha} C^{(1+2\gamma)^k} L]^{\frac 1 {2\gamma}} \\
      & = [\frac \gamma {8\alpha} C^{2\gamma(1+2\gamma)^k+(1+2\gamma)^k} L]^{\frac 1 {2\gamma}}
      = [\frac \gamma {8\alpha} C^{(1+2\gamma)^{k+1}} L]^{\frac 1 {2\gamma}} \ ,
    \end{align*}
    using \cref{lem:small-coord-decrease-step} in the first inequality.
    Noting that $\norm{\Pmap_{A}\vec u(k+1)} \leq \norm{\Pmap_\SS \vec u(k+1)}$ since $A \subset \SS$ gives the desired result.
  \end{subproof}
  By our assumptions, we may write the lower bound on $N$ as
  $\log_{1+2\gamma}\bigr(\log_{\frac 1  C} (\frac{\gamma L^{1+2\gamma}}{8 \cdot 4^{2\gamma}\alpha\epsilon^{2\gamma}})\bigr)$. Thus,
  % Note that
  \begin{align*}
    [\frac \gamma {8 \alpha} C^{(1+2\gamma)^N} L]^{\frac 1 {2\gamma}}
    &\leq
    \Big[\frac \gamma {8 \alpha} C^{\log_{\frac 1  C} \bigr(\frac{\gamma L^{1+2\gamma}}{8\cdot 4^{2\gamma}\alpha\epsilon^{2\gamma}}\bigr)}L\Big]^{\frac 1 {2\gamma}}
    = \Big[\frac \gamma {8 \alpha}  \Big(\frac{8 \cdot 4^{2\gamma}\alpha\epsilon^{2\gamma}}{\gamma L^{1+2\gamma}}\Big) L\Big]^{\frac 1 {2\gamma}}
    \leq \frac {4 \epsilon} L \ .
  \end{align*}
  By \cref{claim:small-coord-exponentiation}, it follows that $N_0 \leq N$.

  We note that for some constant $C' \in [0, 1)$,
  \begin{displaymath}
    \frac{4\epsilon} L \leq
    4C' \Bigr(\frac{\gamma L^{1+2\gamma}}{8\cdot 4^{2\gamma}\alpha}\Bigr)^{\frac 1 {2\gamma}} / L
    = [\frac \gamma {8 \alpha} (C')^{2\gamma} L]^{\frac 1 {2\gamma}} \ .
  \end{displaymath}
  If $\norm{\Pmap_A \vec u(n)} \leq \frac {4\epsilon}{L}$, then \cref{lem:small-coord-decrease-step} implies that
  \begin{displaymath}
    \norm{\Pmap_A \vec u(n+1)} \leq \norm{\Pmap_\SS \vec u(n+1)} \leq \max\left((C')^{2\gamma}\norm{\Pmap_A \vec u(n)},\ \tfrac{4\epsilon} L\right) \leq \tfrac{4\epsilon} L \ .
  \end{displaymath}
  It follows by induction on $n$ that $\norm{\Pmap_\SS \vec u(n)} \leq \frac{4\epsilon} L$ for all $n \geq N_0$.
\end{proof}

In \cref{lem:small-coord-decrease-step,lem:small-coord-decrease-time}, one detail seems to be missing, namely the dependence on $\norm{\nabla F(\vec u)}$.
Since during most steps of \textsc{FindBasisElement} $\norm{\Pmap_0 \vec u}$ will be small, we will typically be able use of the following lemma to lower bound $\norm{\nabla F(\vec u)}$.
\begin{lem}\label{lem:P0small-gradf-lower-bound}
  Let $\vec u \in \sphere^{\dn - 1}$.
  Let $\SS \subset [\dm]$ be non-empty.
  If $\norm{\Pmap_{\compl \SS} \vec u} \leq \frac{1}{\sqrt{2(1+2\delta)}}$, then $\norm{\Pmap_{\SS} \vec u}^{1+2\delta} \geq \frac 1 2$ and $\norm{\nabla F(\vec u)} \geq \frac{\beta}{\delta} \abs{\SS}^{-\delta}$.
\end{lem}
Note that in the worst case where $\SS = [\dm]$, may apply \cref{lem:P0small-gradf-lower-bound} to obtain the lower bound that $\norm{\nabla F(\vec u)} \geq \frac \beta \delta \dm^{-\delta}$.
\begin{proof}[\proofword\@of \cref{lem:P0small-gradf-lower-bound}]
  Once we prove that $\norm{\Pmap_{\SS} \vec u}^{1+2\delta} \geq \frac 1 2$, then the lower bound on $\norm{\nabla F(\vec u)}$ follows from \cref{lem:fg-upper-bounds}.
  We now focus on the proof of the lower bound for $\norm{\Pmap_{\SS} \vec u}^{1+2\delta}$.

  We let $f : \R \rightarrow \R$ be defined by $f(x) = x^{2+4\delta}$.
  As such, $\sqrt{f(\norm{\Pmap_{\SS}\vec u})} = \norm{\Pmap_{\SS}\vec u}^{1+2\delta}$.
  The Taylor expansion of $f$ around 1 for any $x \in [0, 1]$ is
  \begin{displaymath}
    f(x) = f(1) + f'(1)(x-1) + \frac 1 2 f''(y)(x - 1)^2
  \end{displaymath}
  for some $y \in [x, 1]$.
  Notice that $\frac 1 2 f''(y)(x-1)^2 = \frac 1 2 (2+4\delta)(1+4\delta)y^{4\delta}(x-1)^2 \geq 0$.
  As such, $f(x) \geq f(1) + f'(1)(x-1) = 1-2(1+2\delta)(1-x)$.
  To obtain that $f(x)\geq \frac 1 4$, it suffices to show that $1-2(1+2\delta)(1-x) \geq \frac 1 4$.
  Rearranging terms, we see that this occurs if $x \geq 1 - \frac{3}{8(1+2\delta)}$.

  In order for $\norm{\Pmap_{\SS}\vec u}^{1+2\delta} = \sqrt{f(\norm{\Pmap_{\SS}\vec u})} \geq \frac 1 2$, it suffices that $\norm{\Pmap_{\SS}\vec u} \geq 1 - \frac{3}{8(1+2\delta)}$.
  Note that
  \begin{displaymath}
    \sqrt{\frac 3 {4(1+2\delta)} - \frac{9}{64(1+2\delta)^2}}
    % > \sqrt{\frac 3 {4(1+\delta)} - \frac{9}{64(1+\delta)}}
    > \sqrt{\frac 3 {4(1+2\delta)} - \frac{1}{4(1+2\delta)}}
    = \frac 1 {\sqrt {2(1+2\delta)} }
    \geq \norm{\Pmap_{\compl \SS} \vec u} \ .
  \end{displaymath}
  As such,
  \begin{displaymath}
    \norm{\Pmap_{\SS}\vec u}
    = \sqrt{1 - \norm{\Pmap_{\bar \SS} \vec u}^2}
    \geq \sqrt{ 1 - \frac 3 {4(1+2\delta)} + \frac 9 {64(1+2\delta)^2} }
    \geq 1 - \frac 3 {8(1+2\delta)} \ ,
  \end{displaymath}
  as desired.
\end{proof}

Importantly, since $\norm{\Pmap_0 \vec u(n)}$ rapidly goes to 0 under the gradient iteration, the precondition that $\norm{\Pmap_0 \vec u(n)} \leq \frac 1 {\sqrt {2(1+2\delta)} }$ used in \cref{lem:P0small-gradf-lower-bound} when $\SS = [\dm]$ is actually closed under applications of the gradient iteration when $\epsilon$ is sufficiently small.
In particular, we have the following result.
\begin{cor}\label{cor:P0small-closure}
  Suppose that the sequence $\{\vec u(n)\}_{n=0}^\infty$ is recursively defined by $\vec u(n+1) = \hat \GG(\vec u(n))$, and that $\norm{\Pmap_0 \vec u(0)} \leq \frac{1}{\sqrt{2(1+2\delta)}}$.
  If $\epsilon \leq \frac{\beta}{2 \dm^\delta \delta\sqrt{2(1+2\delta)}}$, then $\norm{\Pmap_0 \vec u(n)} \leq \frac 1 {\sqrt{2(1+2\delta)}}$ and $\norm{\nabla F(\vec u)} \geq \frac \beta \delta \dm^{-\delta}$ for all $n$.
\end{cor}
\begin{proof}
  We argue by induction on the hypothesis $\norm{\Pmap_0 \vec u(n)}
  \leq \frac 1 {\sqrt{2(1+2\delta)}}$.
  The base case is given.
  Further, if $\norm{\Pmap_0 \vec u(n)} \leq \frac{1}{\sqrt{2(1+2\delta)}}$,
  then $\norm{\nabla F(\vec u)} \geq \frac \beta \delta \dm^{-\delta}$ by
  \cref{lem:P0small-gradf-lower-bound}.
  Using \cref{lem:small-coord-decrease-step}, we obtain
  \begin{displaymath}
    \norm{\Pmap_0
      \vec u(n+1)} = \norm{\Pmap_0 \hat \GG(\vec u(n))} \leq
    \frac{2\epsilon}{\norm{\nabla F(\vec u(n))}} \leq 2 \epsilon \dm^\delta
    \delta / \beta \leq \frac 1 {\sqrt{2(1+2\delta)}} \ . \qedhere
  \end{displaymath}
\end{proof}

We now combine the \cref{lem:small-coord-decrease-step,lem:P0small-gradf-lower-bound} to provide a time bound for the rapid decay of the small coordinates of $\vec u(n)$.
Here and later in our analysis, we will introduce a number of useful constants and expressions for various lemmas and propositions that we prove, indexing these expressions by the lemma/proposition number of the result for which they were introduced.
We define $\tcompress := [\frac {\beta\gamma} {16 \alpha\delta }\dm^{- \delta}]^{\frac 1 {2\gamma}}$.
This magnitude is treated as a threshold for the cutoff between small and large coordinates of $\vec u$.
Those coordinates of $\vec u(0)$ for which $\abs{u_i(0)} \leq \tcompress$ shrink and then stay small under the gradient iteration unless $\norm{\Pmap_0 \vec u(0)}$ is unusually large.
More formally, we have the following result.

\begin{prop}\label{prop:GI-Loop-Small-Coords-Error}
  Let $\vec u \in \sphere^{\dn - 1}$.
  Suppose that $\epsilon < \frac \beta {8\delta \sqrt{1+2\delta} }\dm^{- \delta-\frac 1 2}\left[\frac{\beta \gamma}{16\alpha \delta}\dm^{- \delta}\right]^{\frac 1 {2\gamma}}$, that
  $\norm{\Pmap_0 \vec u} \leq \frac 1 {\sqrt{2(1+2\delta)}}$, and that
  \begin{displaymath}
  N \geq \log_{1+2\gamma} \biggr(
  \log_2 \biggr( \frac{\beta \gamma}{8\alpha \delta} \biggr)
  + 2\gamma \log_2 \biggr( \frac{\beta}{4\delta\epsilon} \biggr)
  %  \cdot \dm^{-\frac{\delta(1+\gamma)} 2}\bigg(\frac{\beta}{(1+\delta)\epsilon}\bigg)^\gamma
  \biggr) \ ,
\end{displaymath}
  is a positive integer.
  Let $\vec w \leftarrow \textsc{GI-Loop}(\vec u, 2N)$.
  The following hold:
  \begin{enumerate}
    \item \label{prop:GI-small-coord:it:trivial} $\norm{\Pmap_0 \vec w} \leq 2\delta \dm^{\delta} \epsilon / \beta$.
    \item \label{prop:GI-small-coord:it:nontrivial}
    Let $\SS \subset [\dm]$.
    If $\abs{u_j} \leq [\frac {\beta\gamma} {16 \alpha\delta }\dm^{- \delta}]^{\frac 1 {2\gamma}}$ for all $j \in \SS$,
    then $\norm{(\Pmap_0 + \Pmap_\SS) \vec w} \leq 4\delta (\dm-\abs \SS)^{\delta} \epsilon / \beta$.
  \end{enumerate}
\end{prop}
\def\Nsc{\ensuremath{N_{\ref{prop:GI-Loop-Small-Coords-Error}}}}%
Also for later reference, we define \Nsc\@ to be $\bigr\lceil\log_{1+2\gamma} \bigr(
  \log_2 \bigr( \frac{\beta \gamma}{8\alpha \delta} \bigr)
  + 2\gamma \log_2 \bigr( \frac{\beta}{4 \delta \epsilon} \bigr)\bigr)\bigr\rceil$.
  Note that since $\frac{\beta \gamma}{8 \alpha \delta} < 1$, we have that $\log_2(\frac{\beta \gamma}{8 \alpha \delta}) < 0$.
  In particular, it is actually sufficient in \cref{prop:GI-Loop-Small-Coords-Error} that $N \geq \log_{1+2\gamma}(2\gamma \log_2(\frac {\beta}{4\delta \epsilon}))$.
  Further, $\log_{1+2\gamma}(2\gamma) + \log_{1+2\gamma}( \log_2(\frac {\beta}{4\delta \epsilon})) \leq \log_{1+2\gamma}( \log_2(\frac {\beta}{4\delta \epsilon})) + 1$ implies that it is sufficient that $N \geq C \log_{1+2\gamma}( \log_2(\frac {\beta}{4\delta \epsilon}))$ for some universal constant $C$.
  In particular, this time bound represents a super-linear (order $1+2\gamma$) rate of convergence of the small coordinates to $\epsilon$-error which corresponds to the convergence rate guarantees that were seen in \cref{thm:gi-convergence} for the unperturbed setting.
  We also use this simplified version of the bound in the statements of \cref{thm:single-recovery-main,thm:full-recovery-main}.

\begin{proof}[\proofword\@of \cref{prop:GI-Loop-Small-Coords-Error}]
  We first define the sequence $\{\vec u(n)\}_{n=0}^\infty$ recursively by $\vec u(0) = \vec u$ and $\vec u(n+1) = \hat \GG(\vec u(n))$.
  By construction, $\vec w = \vec u(2N)$.
  As such, it suffices to prove the desired properties on this sequence.

  We first show (by induction on $n$) that for every $n \in \N \cup \{0\}$,
  $\norm{\nabla F(\vec u(n))} \geq \frac \beta \delta \dm^{- \delta}$.
  The base case when $n = 0$ follows by \cref{lem:P0small-gradf-lower-bound} (choosing $\SS$ in \cref{lem:P0small-gradf-lower-bound} as $[\dm]$).
  Letting $L = \frac \beta {\delta} \dm^{-\delta}$,
  it is easily verified that $\epsilon \leq \frac 1 2 L$, and in particular, we may apply \cref{lem:small-coord-decrease-step} whenever our inductive hypothesis holds.
  We suppose that our inductive hypothesis holds for $n = k$.
  Using \cref{lem:small-coord-decrease-step} part~\ref{lem:small-coord-trivial}, we see that
  \begin{align}\label{eq:null-proj-bound}
    \norm{\Pmap_0 \vec u(k+1)}
    &\leq \frac {2 \epsilon}{ \norm{\nabla F(\vec u(k))} }
    \leq \frac {2 \epsilon} L \nonumber \\
    &\leq \frac{\beta}{8\delta\sqrt{1+2\delta}} \dm^{-\delta-\frac 1 2}\left[\frac{\beta\gamma}{16\alpha\delta\dm^{\delta}}\right]^{\frac 1 {2\gamma}} / L
    < \frac 1 {2\sqrt{2(1+2\delta)}} \ .
  \end{align}
  As such, we may apply \cref{lem:P0small-gradf-lower-bound} to see that $\norm{ \nabla F(\vec u(k+1)) } \geq L$ as desired.
  By the principle of mathematical induction, $\norm{\nabla F(\vec u(n))} \geq L$ for all $n \in \N \cup \{0\}$.

  To obtain part~\ref{prop:GI-small-coord:it:trivial}, apply \cref{lem:small-coord-decrease-step} to see that
  \begin{displaymath}
  \norm{\Pmap_0 \vec w} = \norm{\Pmap_0 \vec u(2N)} \leq \frac{2 \epsilon}{\norm{\nabla F(\vec u(2N-1))}} \leq \frac{2\delta\dm^{\delta} \epsilon} \beta \ .
  \end{displaymath}

  We now prove part~\ref{prop:GI-small-coord:it:nontrivial}.
  With $L$ as before, we note that by construction,
  \begin{align*}
    \epsilon
    &< \frac{\beta}{8\delta\sqrt{1+2\delta}\dm^{\delta+\frac 1 2}}
    \left[\frac{\beta\gamma}{16\alpha\delta\dm^{\delta}}\right]^{\frac 1 {2\gamma}} \\
    &= \frac{L}{8\sqrt{1+2\delta}\dm^{\frac 1  2}}\left[\frac{L\gamma}{16\alpha}\right]^{\frac 1 {2\gamma}}
    \leq \min\biggr( \frac 1 2 L, \Big(\frac{\gamma L^{1+2\gamma}}{8\cdot 4^{2\gamma} \alpha} \Big)^{\frac 1 {2\gamma}} \biggr) \ .
  \end{align*}
  Notice that $L$ is a lower bound on $\norm{\nabla F(\vec u(n))}$ for all $n$.
  We apply \cref{lem:small-coord-decrease-time} with the choice $\SS_{\ref{lem:small-coord-decrease-time}} =\{j\}$ such that $j \in \SS$, the choice $C = \frac 1 2$, and our choice of $L$.
  We obtain $\abs{u_j(n)} \leq \frac {4\epsilon} L \leq 4\delta\dm^{\delta}\epsilon / \beta$ for all $n \geq N$.

  We fix $k \geq N$ an arbitrary integer.
  We note that
  \begin{align*}
    \norm{\Pmap_{\SS} \vec u(k)}
    &\leq \sqrt{\textstyle{\sum_{j \in \SS}} (4\delta \dm^{\delta} \epsilon / \beta)^2}
    \leq 4\delta \dm^{\delta+\frac 1 2} \epsilon / \beta \\
    &\leq \min\left( \frac 1 {2\sqrt{2(1+2\delta)}},\ [\frac{\beta \gamma}{16 \alpha \delta} \dm^{- \delta}]^{\frac 1 {2\gamma}}\right)
  \end{align*}
  by our choice of $\epsilon$.
  Combining with \cref{eq:null-proj-bound}, we see that $\norm{(\Pmap_0 + \Pmap_\SS)\vec u(k)} \leq \frac 1 {\sqrt{2(1+2\delta)}}$.
  Applying \cref{lem:P0small-gradf-lower-bound} with $\SS_{\ref{lem:P0small-gradf-lower-bound}} = \compl \SS \cap [\dm]$, we see that $\norm{\nabla F(\vec u(k))} \geq \frac \beta \delta \abs{\compl \SS \cap [\dm]}^{- \delta} = \frac \beta \delta (m - \abs{\SS})^{- \delta}$.
  We set a new choice of lower bound $L = \frac \beta \delta (m - \abs{\SS})^{- \delta}$, and we note that $\norm{\Pmap_\SS \vec u(k)} \leq [\frac{\beta \gamma}{16 \alpha \delta} \dm^{- \delta}]^{\frac 1 {2\gamma}} \leq [\frac{\beta \gamma}{16 \alpha \delta} (\dm-\abs \SS)^{- \delta}]^{\frac 1 {2\gamma}} \leq [\frac{\gamma L}{16 \alpha}]^{\frac 1 {2\gamma}}$.
  With our new choice of $L$, we may thus apply \cref{lem:small-coord-decrease-time} on the sequence $\{\vec u(n)\}_{n=N}^\infty$ to obtain that $\norm{\Pmap_\SS \vec w} = \norm{\Pmap_\SS \vec u(2N)} \leq \frac {4 \epsilon} L \leq 4 \delta (\dm-\abs \SS)^\delta \epsilon / \beta$.
\end{proof}

\Cref{prop:GI-Loop-Small-Coords-Error} foreshadows a bound for the final estimation error for the recovery of any hidden basis element using \textsc{FindBasisElement}.
We have not yet demonstrated that the main loop of \textsc{FindBasisElement} drives every coordinate of $\vec u$ (except 1) to become small in the sense of \cref{prop:GI-Loop-Small-Coords-Error}; however, we will eventually do so.
% With this goal in mind, we can predict what our basis recovery error will be.
Combining \cref{lem:hbe-error-bound} below with the error bound from \cref{prop:GI-Loop-Small-Coords-Error} (with $\SS$ chosen such that $\dm - \abs{\SS} = 1$), we will predict that for $\vec u$ returned by \textsc{FindBasisElement}, there exists a sign $s \in \{ \pm 1 \}$ and a hidden basis element $\myZv_i$ such that $i \in [\dm]$ and $\norm{s \myZv_k - \gvec \nu} \leq 4 \sqrt 2 \delta \epsilon / \beta$.
Later, when arguing about the accuracy of \textsc{FindBasisElement}, we will use this predicted bound when making assumptions on how accurately the previously recovered $\gvec \mu_k$s estimate hidden basis elements.

\begin{lem}\label{lem:hbe-error-bound}
  Fix $\vec u \in \sphere^{\dn - 1}$ and $j \in [\dm]$.
  Let $\SS = \{ j \}$.
  Then, there exists $s \in \{ \pm 1 \}$ such that $\norm{s \myZv_j - \vec u} \leq \norm{P_{\compl \SS} \vec u} \sqrt 2$. % 4 \sqrt 2 \epsilon / \beta$.
\end{lem}
\begin{proof}
  We choose $s$ such that $s u_j = \abs {u_j}$.
  We note that
  \begin{displaymath}
    \norm{s \myZv_j - \vec u}^2
    = \norm{P_{\compl \SS} \vec u}^2 + (s - u_j)^2
    \leq \norm{P_{\compl \SS} \vec u}^2 + \abs{(s - u_j)(s + u_j)} \ ,
  \end{displaymath}
  where the inequality uses that $s$ and $u_j$ are of the same sign and hence that $s+u_j$ has at least the same magnitude as $s - u_j$.
  But since $(s - u_j)(s + u_j) = 1 - u_j^2 \geq 0$, we obtain:
  \begin{displaymath}
    \norm{s \myZv_j - \vec u}^2
    \leq \norm{P_{\compl \SS} \vec u}^2 + 1 - u_j^2 \ .
  \end{displaymath}
  Since $\vec u \in \sphere^{\dn - 1}$ is a unit vector, $u_j^2 = 1 - \norm{P_{\compl \SS} \vec u}^2$.
  Thus, $\norm{s \myZv_j - \vec u}^2
    \leq 2\norm{P_{\compl \SS} \vec u}^2 $.
    % \leq 2[4\delta \epsilon / \beta]^2 \ .
  Taking square roots gives the desired result.
\end{proof}

\subsubsection{Setting Up the Main Loop of \textsc{FindBasisElement}}

We now demonstrate that the steps in \textsc{FindBasisElement} preceding the main loop create a warm start for the main loop.
That is, we wish to demonstrate that after line~\ref{alg:step:zero-nonbasis-coords2} of \textsc{FindBasisElement}, $\norm{\Pmap_0 \vec u}$ is small and so are the coordinates of $\vec u$ corresponding to the hidden basis directions approximately recovered in $\gvec \mu_1, \dotsc, \gvec \mu_k$.
This line of argument is carried out in \cref{lem:zeroing-nonbasis-coords,lem:main-loop-precondition} below.

\begin{lem}\label{lem:zeroing-nonbasis-coords}
    Consider an execution of \textsc{FindBasisElement}.
    Fix $\eta \in [0, \frac 1 {4 \dm \sqrt \dn}]$.
    Suppose that $k < \dm$; that there is a permutation $\pi$ on $[\dm]$; there are sign values $s_1, \dotsc, s_k \in \{+1, -1\}$ such that for each $i \in [k]$, $\norm{s_i \gvec \mu_i - \myZv_{\pi(i)}} \leq \eta$; and that $\epsilon \leq \frac \beta {4 \sqrt 2 \delta} \dm^{- \delta} \dn^{- \frac 1 2 - \delta}$.
    At the end of the execution of step~\ref{alg:step:zero-nonbasis-coords} of \textsc{FindBasisElement}, the following hold:
    \begin{enumerate}
        \item\label{item:step5:null-space} $\norm{\Pmap_0 \gvec u} \leq \dm^{\delta}\dn^{\frac 1 2 + \delta}\delta \epsilon / \beta$.
        \item\label{item:step5:controlled-space} If $\eta \leq 4\sqrt 2 \delta \epsilon/ \beta$, and $i \in \{\pi(j) \suchthat j \in [k]\}$, then $ \abs{u_i} \leq \frac{25 \alpha\delta}{2\beta\gamma} \dm^{\delta} \dn^{\frac 1 2 + \delta} \delta \epsilon/\beta$.
    \end{enumerate}
\end{lem}


% \begin{proof}[\proofword\@of Lemma~\ref{lem:zeroing-nonbasis-coords}]
\begin{proof}
    First, we demonstrate that one of the vectors $\vec x_i$ from step~\ref{alg:step-xi-spread} of \textsc{FindBasisElement} has $\norm{\Pmap_{[\dm]} \vec x_i}^2 \geq \frac{\dm-k}{\dn}$.
    We will later use this to demonstrate that $j$ in step~\ref{alg:step:best-xi} satisfies that $\norm{\nabla F(\vec x_j)}$ is sufficiently large for $\hat \GG(\vec x_j)$ to work as intended.

    \begin{claim}\label{claim:xi-in-non-negligeable-region}
        There exists $i \in [\dn - k]$ such that $\norm{\Pmap_{[\dm]} \vec x_i}^2 \geq \frac{\dm-k}\dn$.
    \end{claim}
    \begin{subproof}
        %We let $\SS$ be the set passed into \textsc{FindBasisElement}.
        We let $\SS = \{\pi(k+1), \pi(k+2), \dotsc, \pi(\dm) \}$.
        % Since $\SS \subset [\dm]$, it follows $\norm{\Pmap_{[\dm]} \vec v} \geq \norm{\Pmap_{\SS} \vec v}$ for any $\vec v\in \sphere^{\dn-1}$.
        We extend the list of vectors $\vec x_1, \dotsc, \vec x_{\dn-k}$ to be an orthonormal basis of the space: $\vec x_1, \dotsc, \vec x_\dn$.
        Since each $\myZv_i$ is a unit vector, it follows:
        \begin{equation}
        \label{eq:PtildeS-mean}
        \frac 1 \dn \sum_{i=1}^{\dn} \norm{\Pmap_\SS \vec x_i}^2
        = \frac 1 \dn \sum_{i=1}^{\dn} \sum_{j=k+1}^\dm \ipCanonicalp{\vec x_i}{\myZv_{\pi(j)}}^2
        = \frac 1 \dn \sum_{j={k+1}}^\dm \norm{\myZv_{\pi(j)}}^2
        = \frac{\dm-k}{\dn} \ .
        \end{equation}
        Treating \cref{eq:PtildeS-mean} as a sample average, there exists $i \in [\dn]$ such that $\norm{\Pmap_{\SS} \vec x_i}^2 \geq \frac{\dm - k}\dn$.

        To complete the proof, we need only demonstrate that for any $i > \dn - k$, $\norm{\Pmap_{S} \vec u} < \sqrt{\frac{\dm - k}\dn}$.
        To show this, we first demonstrate that $\gvec \mu_1, \dotsc, \gvec \mu_k$ span a $k$ dimensional space.
        Note that this implies that $\vec x_1, \dotsc, \vec x_{\dn - k}$ span the space $\spn(\gvec \mu_1, \dotsc, \gvec \mu_k)^\perp$.
        Therefore, for any $i > \dn - k$ we have $\vec x_i \in \spn(\gvec \mu_1, \dotsc, \gvec \mu_k)$.
        Then to complete the proof, we demonstrate that for any $\vec v \in \spn(\gvec \mu_1, \dotsc, \gvec \mu_k)$, we have $\norm{\Pmap_{S} \vec u} < \sqrt{\frac{\dm - k}\dn}$.

        Now consider the matrices $A = A_0 = \sum_{i=1}^k \gvec \mu_i \gvec \mu_i^T$ and $\tilde A = \tilde A_0 = \sum_{i=1}^k \myZv_{\pi(i)} \myZv_{\pi(i)}^T$.
        We note:
        \begin{align*}
        \norm{A_0 - \tilde A_0}
        &= \Big \lVert { \sum_{i=1}^k[(\gvec \mu_i - \myZv_{\pi(i)})\gvec \mu_i^T
            + \myZv_{\pi(i)}(\gvec \mu_i - \myZv_{\pi(i)})^T ]} \Big\lVert \\
        &\leq 2 \sum_{i=1}^k\norm{\gvec \mu_i - \myZv_{\pi(i)}}\norm{\gvec \mu_i}
        \leq 2k\eta \ .
        \end{align*}
        In particular, Weyl's inequality (reproduced in \cref{thm:Weyls-inequality}) implies that the $k$\textsuperscript{th} lowest eigenvalue $\lambda_k(A_0) \geq \lambda_k(\tilde A_0) - 2k\eta \geq 1 - 2k\eta > 0$.
        The vectors $\gvec \mu_1, \dotsc, \gvec \mu_k$ are linearly independent.
        As the $k$ eigenvalues of $A_0$ are contained in the interval $[1 - 2k\eta,\ 1 + 2k\eta]$ by Weyl's inequality,
        \cref{thm:sin-theta-thm} (the Davis-Kahan sin $\Theta$ theorem\index{sin $\Theta$ theorem}) with $\tilde A_1 = \sum_{i=k+1}^\dn 0 \myZv_{\pi(i)}\myZv_{\pi(i)}^T$, implies that
        \begin{displaymath}
        (1-2k\eta)\norm{\Pmap_{\spn(\myZv_{\pi(k+1)}, \dotsc, \myZv_{\pi(\dn)})} \Pmap_{\spn(\gvec \mu_1, \dotsc, \gvec \mu_k)}}
        \leq 2k\eta
        \end{displaymath}
        \begin{align*}
        \norm{\Pmap_{\spn(\myZv_{\pi(k+1)}, \dotsc, \myZv_{\pi(\dn)})} \Pmap_{\spn(\gvec \mu_1, \dotsc, \gvec \mu_k)}}
        &\leq \frac{2k\eta}{1-2k\eta}
        < \frac {1/(2\sqrt{\dn})}{1-1/(2\sqrt \dn)}
        \leq \frac {1/(2\sqrt{\dn})}{1/2} \\
        &\leq \frac 1 {\sqrt \dn}
        \leq \sqrt{\frac {\dm-k} \dn} \ .
        \end{align*}
        As such, if $\vec v \in \spn(\gvec \mu_1, \dotsc, \gvec \mu_k)$, then
        \begin{displaymath}
          \norm {\Pmap_\SS \vec v} \leq \norm{\Pmap_{\spn(\myZv_{\pi(k+1)}, \dotsc, \myZv_{\pi(\dn)})} \Pmap_{\spn(\gvec \mu_1, \dotsc, \gvec \mu_k)}} < \sqrt{\frac{\dm - k}{\dn}} \ .
      \end{displaymath}

    \end{subproof}
    We now fix $i\in [\dn - k]$ such that $\norm{\Pmap_{[\dm]} \vec x_i}^2 \geq \frac{\dm - k}{\dn}$ according to \cref{claim:xi-in-non-negligeable-region}, and we fix $j$ according to step~\ref{alg:step:best-xi} from \textsc{FindBasisElement}.
    Note that,
    \begin{displaymath}
    \norm{\grad F(\vec x_i)}
    \geq \frac {2\beta} {\delta} \norm{\Pmap_{[\dm]} \vec x_i}^{1+2\delta}\dm^{-\delta}
    \geq \frac {2 \beta} \delta \left(\frac{m-k}{\dn}\right)^{\frac {1+2\delta} 2} \dm^{- \delta}
    \geq \frac{\beta}{2\delta} \dm^{- \delta} \dn^{- \frac{1+2\delta} 2} \ ,
    \end{displaymath}
    using \cref{lem:fg-upper-bounds} (with projection on the set $[\dn]$) for the first inequality and that $k < m$ implies $m-k \geq 1$ for the final inequality.

    It follows that
    \begin{equation}\label{eq:1}
    \norm{\pertgF(\vec x_j)}
    \geq \norm{\pertgF(\vec x_i)}
    \geq \norm{\nabla F(\vec x_i)} - \epsilon
    \geq \frac{2\beta} \delta \dm^{-\delta} \dn^{-\frac {1+2\delta} 2} - \epsilon
    \end{equation}
    where the first inequality follows from by the choice of $j$ from step~\ref{alg:step:best-xi} of \textsc{FindBasisElement}, and the second inequality uses that $\pertgF$ is an $\epsilon$-approximation to $\nabla F$.

    We now show part~\ref{item:step5:null-space}.
    By the assumption that
    $\epsilon
    \leq \frac \beta {4 \sqrt 2 \delta} \dm^{- \delta} \dn^{- \frac {1+2\delta} 2 }
    \leq \frac \beta \delta \dm^{- \delta} \dn^{- \frac {1+2\delta} 2 }$,
    we have that $\norm{\pertgF(\vec x_j)} \geq \frac{\beta}{\delta}\dm^{-\delta} \dn^{-\frac {1+2\delta} 2}$.
    We see
    \begin{displaymath}
    \norm{\Pmap_0\hat \GG(\vec x_j)}
    \leq \frac{\epsilon}{\norm{\pertgF(\vec x_j)}}
    \leq \dm^{\delta}\dn^{\frac{1+2\delta} 2} \delta \epsilon / \beta \ .
    \end{displaymath}

    We now show part~\ref{item:step5:controlled-space}.
    We let $\vec w = \vec x_j$.
    We let $\ell \in [k]$, and noting that $\vec w \perp \gvec \mu_\ell$ by construction, we obtain the following bound for $\abs {w_{\pi(\ell)}}$:
    \begin{align}\label{eq:2}
    \abs{w_{\pi(\ell)}}
    &= \abs{\ipCanonical{\vec x_j}{(\myZv_{\pi(\ell)} - s_\ell \gvec \mu_\ell + s_\ell \gvec \mu_\ell)}}
    = \abs{\ipCanonical{\vec x_j}{(\myZv_{\pi(\ell)} - s_\ell \gvec \mu_\ell)}} \nonumber \\
    &\leq \norm{\vec x_j} \norm{\myZv_{\pi(\ell)} - s_\ell \gvec \mu_\ell}
    \leq 4 \sqrt 2 \delta \epsilon / \beta \ .
    \end{align}
    We now fix $i \in \{ \pi(\ell) \suchthat \ell \in [k]\}$
    and bound $\abs {u_i} = \abs {\hat \GG_i(\vec w)}$:
    \begin{align*}
    \abs {u_i} = \abs{\hat \GG_i(\vec w)}
    & = \frac{\abs{\pertgF_i(\vec w)}}{\norm{\pertgF(\vec w)}}
    \leq \frac{\abs{\partial_i F(\vec w)}+\epsilon}{\norm{\pertgF(\vec w)}}
    \leq \frac{\frac {2\alpha}{\gamma} \abs{w_i}^{1+2\gamma} + \epsilon }{ \frac{2 \beta} \delta \dm^{-\delta} \dn^{-\frac {1+2\delta} 2} - \epsilon} \\
    &\leq
    \frac{8\sqrt 2 \cdot \frac{\alpha\delta}{\beta\gamma} \left( 4\sqrt 2 \delta \epsilon / \beta \right)^{2\gamma} \epsilon + \epsilon }{ \frac{\beta}{\delta} \dm^{-\delta} \dn^{-\frac {1+2\delta} 2}}
    \end{align*}
    In the above, the second inequality uses \cref{lem:fg-upper-bounds} and \cref{eq:1}; the third inequality uses \cref{eq:2} and that $\epsilon \leq \frac{\beta}{4\sqrt 2 \delta}\dm^{- \delta}\dn^{- \frac {1+2\delta} 2} \leq \frac{\beta}{\delta}\dm^{- \delta}\dn^{- \frac {1+2\delta} 2}$.
    By our given bound on $\epsilon$, we note that $\left( 4\sqrt 2 \delta \epsilon / \beta \right)^{2\gamma} \leq 1$.
    As such, we obtain that
    \begin{align*}
    \abs {u_i} = \abs{\hat \GG_i(\vec w)}
    &\leq  \frac{[8\sqrt 2 \cdot \frac{\alpha\delta}{\beta\gamma} + 1] \epsilon }{ \frac{\beta}{\delta} \dm^{-\delta} \dn^{-\frac {1+2\delta} 2}}
    \leq \frac{(8\sqrt 2 + 1) \cdot \frac{\alpha\delta}{\beta\gamma}\dm^{\frac {1+2\delta} 2} \epsilon }{ \frac{\beta}{\delta} \dm^{-\delta} \dn^{-\frac {1+2\delta} 2}} \\
    &\leq  (8\sqrt 2 + 1) \cdot \frac{\alpha\delta^2}{\beta^2\gamma} \dm^{\delta} \dn^{\frac {1+2\delta} 2} \epsilon
    \leq \frac{25 \alpha \delta^2}{2 \beta^2\gamma} \dm^{\delta} \dn^{\frac {1+2\delta} 2} \epsilon
    \ . \qedhere
    \end{align*}
\end{proof}


\begin{lem}\label{lem:main-loop-precondition}
    Let $k$ be defined as in an execution of \textsc{FindBasisElement}.
    Suppose that $k < \dm$,
    that
    $\epsilon < \frac 1 {16 \sqrt 2} \frac{\beta^2\gamma}{\alpha \delta^2 \sqrt{1+2\delta}}\dm^{-\frac 1 2 -\delta}\dn^{- \frac 1 2 - \delta}\tcompress$,
    that $N_1 \geq 2 N_{\ref{prop:GI-Loop-Small-Coords-Error}}$,
    and that
    there exists a permutation $\pi$ of $[\dm]$ and sign values $s_1, \dotsc, s_k \in \{\pm 1\}$ such that $\norm{s_j \myZv_{\pi(j)} - \gvec \mu_j} \leq 4 \sqrt 2 \delta \epsilon / \beta$ for each $j \in [k]$.
    At the beginning of the execution of the main loop of \textsc{FindBasisElement}, the following hold for $\vec u$:
    \begin{enumerate}
        \item $\norm{\Pmap_0 \vec u} \leq 2 \dm^{\delta} \delta \epsilon / \beta$.
        \item Let $\SS = \{ \pi(j) \suchthat j \in [k] \}$.
        Then, $\norm{(\Pmap_0 + \Pmap_\SS) \vec u} \leq 4(\dm - \abs \SS)^{\delta} \delta \epsilon / \beta$.
    \end{enumerate}
\end{lem}
\begin{proof}
    We first notice that for each $j \in [k]$,
    \begin{displaymath}
    \norm{s_j \myZv_{\pi(j)} - \gvec \mu_j}
    \leq 4 \sqrt 2 \delta \epsilon / \beta
    < \frac{\beta\gamma}{4\alpha\delta\sqrt{1+2\delta}\dm^{\frac 1 2+\delta}}\dn^{-\frac{1+2\delta} 2}\left[\frac{\beta}{16\alpha}\dm^{-\delta}\right]^{\frac 1 {2\gamma}}
    < \frac 1 {4 \dm \sqrt \dn} \ ,
    \end{displaymath}
    where the final inequality uses that $\delta \geq \gamma$ to see that $\dm^{- \frac{\delta}{2\gamma}} \leq \dm^{-\frac 1 2}$.
    As such, we may apply \cref{lem:zeroing-nonbasis-coords} to see that at the end of step~\ref{alg:step:zero-nonbasis-coords} of \textsc{FindBasisElement} that $\norm{\Pmap_0 \vec u} \leq \dm^{\delta} \dn^{\frac {1+2\delta} 2}\delta \epsilon / \beta$ and for each $j \in [k]$ that $\abs{u_{\pi(j)}} \leq \frac{25 \alpha \delta^2}{2\beta^2\gamma} \dm^{\delta} \dn^{\frac{1+2\delta} 2} \epsilon$.
    By our choice of $\epsilon$, it may be verified that
    \begin{displaymath}
    \norm{\Pmap_0 \vec u} \leq \dm^{\delta} \dn^{\frac {1+2\delta} 2} \delta \epsilon / \beta
    < \frac 1 {\sqrt{2(1+2\delta)}}
    \end{displaymath}
    and that for each $j \in [k]$,
    \begin{displaymath}
    \abs{u_{\pi(j)}}
    \leq \frac{25 \alpha\delta^2}{2\beta^2\gamma} \dm^{\delta} \dn^{\frac{1+2\delta} 2} \epsilon
    < \Bigr[ \frac{\beta\gamma}{16 \alpha\delta}\dm^{-\delta}\Bigr]^{\frac 1 {2\gamma}} \ .
    \end{displaymath}
    As the step $\vec u \leftarrow \textsc{GI-Loop}(\vec u, N_1)$ in line~\ref{alg:step:zero-nonbasis-coords2} sets up the main loop of \textsc{FindBasisElement}, applying \cref{prop:GI-Loop-Small-Coords-Error} gives the desired result.
\end{proof}

\subsection{The Big Become Bigger}
\label{sec:large-coord-analysis}
\label{sec:large-coord-analysis-1}

We saw in \cref{sec:small-coord-analysis} that the small coordinates of $\vec u$ rapidly decay under the gradient iteration until they are on the order of $\epsilon$.
In this section, we demonstrate how the large coordinates of $\vec u$ diverge under the gradient iteration, causing some to become bigger and other large coordinates to become small.
In particular, we create a robust version of \cref{prop:gi-expand-all} from \cref{sec:gi-divergence-criteria}.
We recall that in \cref{prop:gi-expand-all}, it was seen that if $\vec v$ is a fixed point of $\GG / {\sim}$ and $\vec u$ satisfied that there exists $i \in [\dm]$ with $v_i \neq 0$ and $\abs{u_i} > v_i$, then for some $u_j$ with $j$ among the non-zero coordinates of $\vec v$ is driven towards 0 by the gradient iteration.
This proposition provided a very useful characterization of the instability of all fixed points of $\GG/{\sim}$ other than the hidden basis $\pm \myZv_1, \dotsc, \pm \myZv_\dm$.


Before proceeding, we will need the following technical result.
\begin{lem}\label{lem:vi-spread}
 % Suppose that $F$ is $(\alpha, \beta, \gamma, \delta)$-robust.
 Let $\SS \subset [\dm]$ be non-empty, and let $\vec v \in \porth^{\dn - 1}$ be a fixed point of $\GG/{\sim}$ such that $v_i \neq 0$ if and only if $i \in \SS$.
 If $k \in \SS$, then $\abs {v_k} \geq  \big(\frac{\beta \gamma }{\alpha \delta \abs \SS^{\delta}} \big)^{\frac 1 {2\gamma}}$.
\end{lem}
\begin{proof}
  Since $\sum_{i \in \SS} v_i^2 = 1$, there exists $j \in \SS$ with $v_j^2 \geq \frac 1 {\abs \SS}$.
  By \cref{lem:F-robust-implications}, $\abs{h_j'(v_j^2)} \geq \frac \beta \alpha \abs {v_j}^{2\delta} \geq \frac{\beta}{\alpha \abs \SS^{\delta}}$.

  Fix any $k \in \SS$.  Then, by \cref{lem:F-robust-implications}, $\abs{h_k'(v_k^2)} \leq \frac{\alpha}{\gamma} \abs {v_k}^{2\gamma}$.
  Since $h_k'(v_k^2) = h_j'(v_j^2)$ by \cref{obs:stationary-criterion}, it follows that $\frac{\alpha}{\gamma}\abs {v_k}^{2\gamma} \geq \frac{\beta}{\delta \abs \SS^{\delta}}$.
  In particular, $\abs {v_k} \geq \big(\frac{\beta\gamma}{\alpha\delta \abs{\SS}^{\delta} }\big)^{\frac 1 {2\gamma}}$.
  % = \big(\frac{\beta\gamma}{\alpha\delta}\big)^{\frac 1 {2\gamma}} \abs{\SS}^{-\frac{\delta}{2\gamma}}$.
\end{proof}

We now demonstrate that when there exists a large coordinate $k$ such that $\abs{u_k}$ is sufficiently greater than the corresponding coordinate $\abs{v_k}$ of a fixed point $\vec v$ of $\GG/{\sim}$, then the separation between large coordinates of $\vec u$ expands under the Gradient iteration.
This expansion was the main idea underlying the proof of \cref{prop:gi-expand-all} (see \cref{claim:expand}).
\begin{lem}\label{lem:robust-GI-progress}
  Let $\vec u \in \sphere^{\dn-1}$ be such that the set $\SS := \{ i \suchthat \abs{u_i} \geq \tcompress\}$ is a subset of $[\dm]$ containing at least 2 elements.
  Suppose $\norm{\Pmap_0 \vec u} \leq \frac 1 {2\sqrt{1+2\delta}}$.
  Let $\vec v \in \porth^{\dn - 1}$ be the fixed point of $\GG/{\sim}$ such that $v_i \neq 0$ if and only if $i \in \SS$.
  Let ${\ell} = \argmax_{i\in\SS} \frac{\abs{u_i}}{v_i}$, and ${k} = \argmin_{i \in \SS} \frac{\abs{u_i}} {v_i}$.
  Fix $\eta \in (0, 1]$, suppose that $\frac{\abs{u_{\ell}}/v_{\ell}}{\abs{u_{k}}/v_{k}} \geq (1 + \eta)^2$, and that $\abs {u_\ell} \geq v_\ell$.
  The following hold:
  \begin{enumerate}
  \item\label{lem:robust-GI-progress:it:1}
    If $\epsilon \leq \frac 1 8 \frac \beta \delta \big(\frac{\beta \gamma}{\alpha \delta}\big)^{\frac \delta \gamma}\abs{\SS}^{-\frac \delta \gamma(\delta - \gamma)} \tcompress^{1 + 2\delta}\eta$, then
    \begin{displaymath}
      \max_{i, j \in \SS} \frac{\abs{\hat \GG_i(\vec u)}/v_i}{\abs{\hat \GG_j(\vec u)}/v_j}
      \geq \left(1 + \frac 3 4 \fcondexpand^{\frac{\delta}{\gamma}}\abs{\SS}^{-\frac \delta \gamma (\delta - \gamma)}\eta \right)\frac{\abs{u_{\ell}}/v_{\ell}}{\abs{u_{k}}/v_{k}} \ .
    \end{displaymath}
  \item\label{lem:robust-GI-progress:it:3}
    If $\epsilon \leq \frac 9 {256} \frac \beta \delta \tcompress^2 \Big(\frac{\beta \gamma}{\alpha \delta}\Big)^{\frac {2\delta + 1}{2\gamma}}\abs{\SS}^{-\frac {\delta}{\gamma}(\frac 1 2 + \delta - \gamma) - \delta}\eta$, then there exists $i \in \SS$ such that $\abs{\GG_i(\vec u)} \geq v_i$.
  \end{enumerate}
\end{lem}

\newcommand{\epsdiverge}[1]{\ensuremath{E_{\ref{lem:robust-GI-progress}}\left(#1\right)}}
For later use, we define the expression
\begin{displaymath}
  \epsdiverge{\eta, \SS}
  := \frac 9 {256}\frac \beta {\delta} \big(\frac{\beta \gamma}{\alpha \delta}\big)^{\frac {2\delta+1}{2\gamma}}\abs{\SS}^{-\frac {\delta}{\gamma}(\frac 1 2 + \delta - \gamma) - \delta} \tcompress^{2 + 2\delta}\eta \ ,
\end{displaymath}
 which serves as a sufficient upper bound for $\epsilon$ in both parts~\ref{lem:robust-GI-progress:it:1} and~\ref{lem:robust-GI-progress:it:3} of \cref{lem:robust-GI-progress}.

\begin{proof}[\proofword\@of \cref{lem:robust-GI-progress}]
  We first prove part~\ref{lem:robust-GI-progress:it:1}.
  In doing so, we will make use of the following claims.
    \begin{claim}\label{claim:robust-GI-progress-single-step}
      Suppose there exists $\Delta > 0$ such that one of the following holds: (1) $h_{\ell}'(u_{\ell}^2) \geq (1+\Delta)h_{\ell}'(v_{\ell}^2)$ or (2) $h_{k}'(u_{k}^2) \leq (1+\Delta)^{-1}h_{k}'(v_{k}^2)$.
      Suppose there exists $\zeta \in (0, \min(\frac 1 {16}, \frac 1 8 \Delta)]$ such that $\epsilon \leq \zeta \min_{i \in \SS} \abs{\partial_i F(\vec u)}$.
      Then,
      $\max_{i, j \in \SS} \frac{\abs{\hat \GG_i(\vec u)}/v_i}{\abs{\hat \GG_j(\vec u)}/v_j} \geq (1+\frac 1 4 \Delta) \frac{\abs {u_{\ell}}/v_{\ell}}{\abs {u_{k}}/v_{k}}$.

  \end{claim}
  \begin{subproof}
  We first bound the error on calculating $\GG_i(\vec u)$.
  For each $i \in \SS$, we have:
  \begin{displaymath}
    %\label{eq:G-hat-Ubound}
    \abs{\hat \GG_i(\vec u)}
    = \frac{\abs{\pertgF_i(\vec u)}}{\norm{\pertgF(\vec u)}}
    \leq \frac{\abs{\partial_i F(\vec u)} + \epsilon}{\norm{\grad F(\vec u)}-\epsilon}
    \leq \frac{1+\zeta}{1-\zeta} \cdot \frac{\abs{\partial_i F(\vec u)}}{\norm{\grad F(\vec u)}}
    = \frac{1+\zeta}{1-\zeta} \cdot \abs{\GG_i(\vec u)}
  \end{displaymath}
  \begin{displaymath}
    % \label{eq:G-hat-Lbound}
    \abs{\hat \GG_i(\vec u)}
    = \frac{\abs{\pertgF_i (\vec u)}}{\norm{\pertgF(\vec u)}}
    \geq \frac{\abs{\partial_i F(\vec u)} - \epsilon}{\norm{\grad F(\vec u)}+\epsilon}
    \geq \frac{1-\zeta}{1+\zeta} \cdot \frac{\abs{\partial_i F(\vec u)}}{\norm{\grad F(\vec u)}}
    = \frac{1-\zeta}{1+\zeta} \cdot \abs{\GG_i(\vec u)} \ .
  \end{displaymath}
  Since $\sum_{i\in \SS} u_i^2 \leq \sum_{i\in \SS} v_i^2 = 1$, it follows that $\abs{u_{k}} \leq v_{k}$.
  As such, we have both that $\abs{u_{k}} \leq v_{k}$ and $\abs{u_{\ell}} \geq v_{\ell}$.
  We have that
  \begin{align*}
    \max_{i, j\in \SS} \frac{\abs{\hat \GG_i(\vec u)}/v_i}{\abs{\hat \GG_j(\vec u)}/v_j}
    & \geq  \Bigr(\frac{1-\zeta}{1+\zeta}\Bigr)^2 \max_{i, j\in \SS}  \frac{\abs{\GG_i(\vec u)}/v_i}{\abs{\GG_j(\vec u)}/v_j}
    = \Bigr(\frac{1-\zeta}{1+\zeta}\Bigr)^2 \max_{i, j\in \SS} \frac{\abs{h_i'(u_i^2)}\abs {u_i}/v_i}{\abs{h_j'(u_j^2)}\abs {u_j}/v_j} \\
    &\geq \Bigr(\frac{1-\zeta}{1+\zeta}\Bigr)^2 \frac{\abs{h_{\ell}'(u_{\ell}^2)}\abs {u_{\ell}}/v_{\ell}}{\abs{h_{k}'(u_{k}^2)}\abs {u_{k}}/v_{k}}
    \geq \Bigr(\frac{1-\zeta}{1+\zeta}\Bigr)^2\frac{(1+\Delta)\abs{h_{\ell}'(v_{\ell}^2)}\abs{u_{\ell}}/v_{\ell}}{\abs{h_{k}'(v_{k}^2)}\abs{u_{k}}/v_{k}} \\
    &\geq (1+\Delta)\Bigr(\frac{1-\zeta}{1+\zeta}\Bigr)^2\frac{\abs{u_{\ell}}/v_{\ell}}{\abs{u_{k}}/v_{k}} \ .
  \end{align*}
  In the second to last inequality, we use the monotonicity of $h_i'$ (see \cref{lem:h-props}) along with the assumption that one of the following holds:  either (1) $h_{\ell}'(u_{\ell}^2) \geq (1+\Delta)h_{\ell}'(v_{\ell}^2)$ or (2) $h_{k}'(u_{k}^2) \leq (1+\Delta)^{-1} h_{k}'(v_{k}^2)$.
  In the last inequality, we use \cref{obs:stationary-criterion} to note that $\abs{h_{\ell}'(v_{\ell}^2)} = \abs{h_{k}'(v_{k}^2)}$.

  We now only need bound $(1 + \Delta)\Bigr(\frac{1-\zeta}{1+\zeta}\Bigr)^2$.
  We first note that $\Bigr(\frac{1-\zeta}{1+\zeta}\Bigr)^2=\Bigr(1 - \frac{2\zeta}{1+\zeta}\Bigr)^2 \geq (1-2\zeta)^2 \geq 1 - 4 \zeta$.
  Thus, $(1+\Delta)\Bigr(\frac{1-\zeta}{1+\zeta}\Bigr)^2 \geq 1 + \Delta - 4\zeta - 4\zeta\Delta$.
  Using the upper bounds on $\zeta$, we see that
$1 + \Delta - 4\zeta - 4\zeta\Delta \geq 1 + \Delta - \frac 1 2 \Delta - \frac 1 4 \Delta \geq 1 + \frac 1 4 \Delta$.
  Thus, we obtain
  \begin{displaymath}
    \max_{i, j\in \SS} \frac{\abs{\hat \GG_i(\vec u)}/v_i}{\abs{\hat \GG_j(\vec u)}/v_j} \geq \left(1 + \frac 1 4 \Delta\right) \max_{i, j \in \SS} \frac{\abs{u_i}/v_i}{\abs{u_j}/v_j} \ . \qedhere
  \end{displaymath}
\end{subproof}

    \begin{claim}\label{claim:robust-gi-frac-trapping}
      Suppose $\Delta > 0$,
      $\eta \geq \frac 4 3 \Big(\frac {\alpha \delta}{\beta \gamma}\Big)^{\frac \delta \gamma} \abs{\SS}^{\frac \delta \gamma (\delta - \gamma)}\Delta$,
      and $\frac{\abs{u_{\ell}} / v_{\ell}}{\abs{u_{k}}/v_{k}}\geq (1+\eta)^2$.
      Then one of the following holds: either
      (1) $\abs{h_{\ell}'(u_{\ell}^2)} \geq (1+\Delta)\abs{h_{\ell}'(v_{\ell}^2)}$ or
      (2) $\abs{h_{k}'(u_{k}^2)} \leq (1+\Delta)^{-1} \abs{h_{k}'(v_{k}^2)}$.
    \end{claim}
    \begin{subproof}
      Before proceeding, we note that for $y^2 \geq x^2$ (with $x, y \in \R$), we have that \[\sign(h_i'(x^2)) = \sign(h_i'(y^2)) = \sign(h_i''(t))\] for all $t \in [x^2, y^2]$.
      As such, we may use \cref{lem:F-robust-implications} to see:
      \begin{align}\label{eq:hi-change}
        \abs{h_i'(y^2)} - \abs{h_i'(x^2)}
        &= \int_{x^2}^{y^2}\abs{h_i''(t)} dt
        \geq \beta \int_{x^2}^{y^2} t^{\delta - 1} dt
        \geq \frac \beta \delta [\abs{y}^{2\delta} - \abs{x}^{2\delta}]
      \end{align}


      By the assumption $\frac{\abs{u_{\ell}} / v_{\ell}}{\abs{u_{k}}/v_{k}}\geq (1+\eta)^2$, one of the following must hold:
      (1) $\abs{u_{\ell}} / v_{\ell} \geq (1+\eta)$ or
      (2) $\abs{u_{k}}/v_{k} \leq (1+\eta)^{-1}$.
      We consider these cases separately, and demonstrate that in each case one of our desired results holds.
      \resetcasecount
      \begin{case}
        $\abs{u_{\ell}} / v_{\ell} \geq (1+\eta)$.
      \end{case}
      \begin{caseblock}
        We obtain that
        \begin{align*}
          \abs{h_{\ell}'(u_{\ell}^2)} - \abs{h_{\ell}'(v_{\ell}^2)}
          &\geq \abs{h_{\ell}'((1+\eta)^2v_{\ell}^2) - h_{\ell}'(v_{\ell}^2)}
          %&\geq \beta x^{2\delta - 2}((1+\eta)^2v_{\ell}^2 - v_{\ell}^2)
          = \frac\beta\delta v_{\ell}^{2\delta}[(1+\eta)^2 - 1]
          \geq 2\eta \frac\beta\delta v_{\ell}^{2\delta}
        \end{align*}
        where the first inequality uses the monotonicity of $h_{\ell}'$ (see \cref{lem:h-props}), and the second inequality uses \cref{eq:hi-change}.
        We note that for any $i \in \SS$,
        \begin{align}\label{eq:vi2del-lb}
          v_{i}^{2\delta}
          &= \frac{\gamma}{\alpha} v_{i}^{2(\delta-\gamma)} \cdot \frac \alpha \gamma v_{i}^{2\gamma}
          \geq \frac{\gamma}{\alpha} v_{i}^{2(\delta-\gamma)} \abs{h_i'(v_{i}^2)}
          \geq \frac{\gamma}{\alpha} \Big(\frac {\beta \gamma}{\alpha \delta}\Big)^{\frac \delta \gamma} \abs{\SS}^{-\frac \delta \gamma (\delta - \gamma)} \abs{h_{i}'(v_{i}^2)}
        \end{align}
        using \cref{lem:F-robust-implications} for the first inequality and \cref{lem:vi-spread} for the final inequality.
        As such, we obtain:
        \begin{align*}
          \abs{h_{\ell}'(u_{\ell}^2)} - \abs{h_{\ell}'(v_{\ell}^2)}
          &\geq 2\eta \Big(\frac {\beta \gamma}{\alpha \delta}\Big)^{\frac \delta \gamma} \abs{\SS}^{-\frac \delta \gamma (\delta - \gamma)} \abs{h_{\ell}'(v_{\ell}^2)}
        \end{align*}

        By the lower bound on $\eta$, we obtain $\abs{h'_{\ell}(u_{\ell}^2)} - \abs{h_{\ell}'(v_{\ell}^2)} \geq 2 \Delta \abs{h_{\ell}'(v_{\ell}^2)} \geq \Delta \abs{h_{\ell}'(v_{\ell}^2)}$ as desired.
      \end{caseblock}
      \begin{case}
        $\abs{u_{k}}/v_{k} \leq (1+\eta)^{-1}$.
      \end{case}
      \begin{caseblock}
        Note that $\abs{u_{k}} \leq (1 + \eta)^{-1}v_{k}$.
        We apply \cref{eq:hi-change} to obtain
        \begin{displaymath}
          \abs{h_{k}'(v_{k}^2)} - \abs{h_{k}'(u_{k}^2)}
          \geq \abs{h_{k}'(v_{k}^2) - h_{k}'((1 + \eta)^{-2}v_{k}^2)}
          \geq \frac{\beta}{\delta}v_{k}^{2\delta}[1 - (1+\eta)^{-2}]
        \end{displaymath}
        Using the bound $\eta \geq 1$, we see that
        \begin{displaymath}
          1 - (1+\eta)^{-2}
          = \Big[1 + \frac 1 {1+\eta}\Big]\Big[1 - \frac 1 {1+\eta}\Big]
          = \Big[1 + \frac 1 {1+\eta}\Big]\Big[\frac \eta {1+\eta}\Big]
          \geq \frac 3 4 \eta
        \end{displaymath}
        we obtain
        \begin{displaymath}
          \abs{h_{k}'(v_{k}^2)} - \abs{h_{k}'(u_{k}^2)}
          \geq \abs{h_{k}'(v_{k}^2) - h_{k}'((1 + \eta)^{-2}v_{k}^2)}
          \geq \eta \frac{\beta}{\delta}v_{k}^{2\delta} \ .
        \end{displaymath}
        As such, $\abs{h_k'(v_k^2)} - \abs{h_k'(u_k^2)} \geq \frac {3\beta}{4\delta} v_k^{2\delta} \eta$.
%        where the inequality uses in part the monotonicity of $h_{k}'$ (see \cref{lem:h-props}) and the equality uses the mean value theorem.
        Applying \cref{eq:vi2del-lb}, we obtain
        \begin{displaymath}
          \abs{h_{k}'(v_{k}^2)} - \abs{h_{k}'(u_{k}^2)}
          \geq \frac 3 4 \eta \Big(\frac {\beta \gamma}{\alpha \delta}\Big)^{\frac \delta \gamma} \abs{\SS}^{-\frac \delta \gamma (\delta - \gamma)} \abs{h_{k}'(v_{k}^2)}
          \geq \frac 3 4 \Delta \abs{h_{k}'(v_{k}^2)} \ .
        \end{displaymath}
        Rearranging terms yields $\abs{h_{k}'(u_{k}^2)} \leq \abs{h_{k}'(v_{k}^2)}(1-\Delta)$.
        As $(1+\Delta)^{-1} = \frac{1+\Delta - \Delta}{1+\Delta} = 1 - \frac {\Delta}{1+\Delta} \geq 1 - \Delta$, it follows that $\abs{h_{k}'(u_{k}^2)} \leq (1+\Delta)^{-1} \abs{h_{k}'(v_{k}^2)}$ as desired. \qedhere
      \end{caseblock}
    \end{subproof}

    \noindent  To use these claims, we set parameters $\Delta = \frac 3 4 \Big(\frac{\beta \gamma}{\alpha \delta}\Big)^{\frac \delta \gamma}\abs{\SS}^{-\frac \delta \gamma (\delta - \gamma)} \eta$ and $\zeta = \min(\frac 1 8 \Delta, \frac 1 {16})$.
    By \cref{lem:F-robust-implications}, it follows that $\min_{i \in \SS} \abs{\partial_i F(\vec u)} = \min_{i \in \SS} \abs{g_i'(u_i)} \geq 2\frac \beta \gamma \tcompress^{1 + 2\delta}$.
    We note that $\epsilon \leq \frac{\beta}{8\delta}\tcompress^{1+2\delta} \leq \frac 1 {16} \min_{i \in \SS} \abs{\partial_i F(\vec u)}$, and also that
    \begin{displaymath}
      \epsilon
      \leq \frac \beta {8\delta}\Big(\frac {\beta \gamma}{\alpha \delta}\Big)^{\frac \delta \gamma}\big(\frac 1 {\abs{\SS}}\big)^{\frac \delta \gamma(\delta - \gamma)}\tcompress^{1+2\delta}\eta
      \leq \frac 1 {6} \Delta \frac \beta \delta \tcompress^{1+2\delta}
      \leq \frac 1 {12} \Delta \min_{i \in \SS}\abs{\partial_i F(\vec u)} \ .
    \end{displaymath}
    As such, $\epsilon \leq \zeta \min_{i \in \SS} \abs{\partial_i F(\vec u)}$, and we may apply our claims.
    We apply \cref{claim:robust-gi-frac-trapping} followed by \cref{claim:robust-GI-progress-single-step} to complete the proof of part~\ref{lem:robust-GI-progress:it:1}.


    We now prove part~\ref{lem:robust-GI-progress:it:3}.
    We will make use of the following additional claim.
    \begin{claim}\label{claim:robust-increasing-hi-un}
      Suppose that $\Delta > 0$,
      that \[\eta \geq \frac 4 3 \Big(\frac {\alpha \delta}{\beta \gamma}\Big)^{\frac \delta \gamma} \abs{\SS}^{\frac \delta \gamma(\delta - \gamma)}\Delta,\]
      and that $\frac{\abs{u_{\ell}} / v_{\ell}}{\abs{u_{k}}/v_{k}}\geq (1+\eta)^2$.
      If $\epsilon \leq \frac{3}{32} \tcompress^2\frac{2\Delta + \Delta^2}{(1+\Delta)^2} \cdot \big(\frac{\beta\gamma}{\alpha \delta \abs{\SS}^\delta}\big)^{\frac 1 {2\gamma}} \frac{\beta}{\delta \abs{\SS}^\delta}$, then there exists $i \in \SS$ such that $\abs{\GG_i(\vec u)} \geq \abs{v_i}$.
    \end{claim}
    \begin{subproof}
      We define $i^* = \argmax_{i \in \SS} \abs{h_i'(u_i^2)}$.
      There exists $\lambda = \abs{h_i'(v_i^2)}$ for all $i \in \SS$ (by \cref{obs:stationary-criterion}).
      Since $\abs{u_\ell} \geq \abs{v_\ell}$, the monotonicity of the $h_i'$s with $h_i'(0) = 0$ (see \cref{lem:h-props}) implies that $\abs{h_i'(u_{\ell}^2)} \geq \abs{h_i'(v_\ell^2)} = \lambda$.
      In particular, $\abs{h_{i^*}(u_{i^*}^2)} \geq \lambda = h_{i^*}(v_{i^*}^2)$. %, and hence $\abs {u_{i^*}} \geq \abs{v_{i^*}}$.

      We proceed in the following two cases, which by \cref{claim:robust-gi-frac-trapping} cover all possible cases.
      \resetcasecount
      \begin{case}
        $\abs{h_\ell'(u_\ell^2)} \geq (1+\Delta)\lambda$.
      \end{case}
      \begin{caseblock}
        Since $\abs{h_i'(u_{i^*}^2)} \geq \abs{h_\ell'(u_\ell^2)}$, it follows that $\abs{h_{i^*}'(u_i^2)} \geq (1+\Delta)\lambda$.
        Since $\sum_{i \in \SS} u_i^2 \leq \sum_{i \in \SS} v_i^2 = 1$ implies the existence of $i \in \SS$ such that $u_i^2 \leq v_i^2$, it follows that $u_k^2 < v_k^2$ and hence that $\abs{h_k'(u_k^2)} \leq \lambda$.
        In particular, we obtain $\frac{\abs{h_{i^*}'(u_{i^*}^2)}}{\abs{ h_k'(u_k^2)}} \geq \frac{(1+\Delta)\lambda}{\lambda} \geq (1+\Delta)$.
      \end{caseblock}
      \begin{case}
        $\abs{h_k'(u_k^2)} \leq (1+\Delta)^{-1}\lambda$.
      \end{case}
      \begin{caseblock}
        Using that $\abs{h_{i^*}(u_{i^*}^2)} \geq \lambda$, we obtain $\frac{\abs{h_{i^*}'(u_{i^*}^2)}}{\abs{ h_k'(u_k^2)}} \geq \frac{\lambda}{(1+\Delta)^{-1}\lambda} \geq (1+\Delta)$.
      \end{caseblock}
    \noindent
    In both cases, we obtain
    \begin{equation}\label{eq:96305269}
      \frac{\abs{h_{i^*}'(u_{i^*}^2)}}{\abs{h_k'(u_k^2)}}
      \geq (1+\Delta)
    \end{equation}
    We use this fact to bound $\GG_{i^*}(\vec u)^2$ from below.
    \begin{align*}
      \frac{1}{\GG_{i^*}(\vec u)^2}
      &= \frac{\sum_{i=1}^\dn\GG_i(\vec u)^2}{\GG_{i^*}(\vec u)^2}
      = \frac{\sum_{i=1}^\dn[h_i'(u_i^2)u_i]^2}{[h_{i^*}'(u_{i^*}^2)u_{i^*}]^2} \\
      &\leq \frac{\sum_{i=1}^\dn u_i^2 - [1 - (1+\Delta)^{-2}]u_k^2}{u_{i^*}^2}
      \leq \frac{1 - [1 - (1+\Delta)^{-2}]\tcompress^2}{u_{i^*}^2} \\
      &= \frac{(1+\Delta)^2[1-\tcompress^2] + \tcompress^2}{(1+\Delta)^2 u_{i^*}^2} \ .
    \end{align*}
    In the above, for the first inequality, we use our bound from \cref{eq:96305269} and that $\abs{h_{i^*}'(u_{i^*}^2)} \geq \abs{h_i'(u_i^2)}$ for all $i \in [\dn]$.
    To see that this holds for $i \in \compl \SS$, we note that by \cref{cor:tcompress} treating $\nabla F$ as a 0-approximation of itself that $\abs{\GG_i(\vec u)} \leq \frac 1 2 \abs{u_i}$.
    In particular, since $\norm{\GG(\vec u)} = 1 = \norm{\vec u}$, there exists $j \in [\dn]$ such that $\abs{\GG_j(\vec u)} \geq \abs{u_j}$.
    Hence, $1 < \frac{\abs{\GG_j(\vec u)}/{\abs{u_j}}}{\abs{\GG_i(\vec u)}/\abs{u_i}} =\frac{h_j'(u_j^2)}{h_i'(u_i^2)}$ implies that $\abs{h_i'(u_i^2)}$ is not maximal for any $i \in \compl \SS$.
    In particular, $\ell = \argmax_{i \in [\dn]} \abs{h_i'(u_i^2)}$.

    Continuing, we obtain:
    \begin{align*}
      \frac{\GG_{i^*}(\vec u)^2}{u_{i^*}^2}
      &\geq \frac{(1+\Delta)^2}{(1+\Delta)^2[1-\tcompress^2] + \tcompress^2}
      = 1 + \tcompress^2 \frac{(1+\Delta)^2 - 1}{(1+\Delta)^2[1-\tcompress^2] + \tcompress^2} \\
      &= 1 + \tcompress^2\frac{2\Delta + \Delta^2}{(1+\Delta)^2 - \tcompress[(1+\Delta)^2 - 1]}
      \geq 1 + \tcompress^2 \frac{2\Delta + \Delta^2}{(1+\Delta)^2} \ .
      % =1 + \tcompress^2[1 - (1+\Delta)^{-2}] \ .
    \end{align*}
    Applying \cref{lem:G-est-error}, we see that:
    \begin{displaymath}
      \abs{\hat \GG_{i^*}(\vec u)}
      \geq \abs{\GG_{i^*}(\vec u)} - 4 \delta \abs{\SS}^\delta \epsilon / \beta
      \geq \abs{u_{i^*}}\sqrt{1 + \tcompress^2\frac{2\Delta+\Delta^2}{(1+\Delta)^2}}
      - 4 \delta \abs{\SS}^\delta \epsilon / \beta \ .
    \end{displaymath}
    Noting that $\abs{u_{i^*}} \geq \abs{v_{i^*}}$ and applying the lower bound from \cref{lem:vi-spread}, we obtain
    \begin{align*}
      \frac{\abs{\hat \GG_{i^*}(\vec u)}}{\abs{u_{i^*}}}
      &\geq \sqrt{1 + \tcompress^2\frac{2\Delta+\Delta^2}{(1+\Delta)^2}}
      - 4 \frac{\delta \abs{\SS}^\delta \epsilon}{\beta\abs{u_{i^*}}} \\
      &\geq \sqrt{1 + \tcompress^2\frac{2\Delta+\Delta^2}{(1+\Delta)^2}} - 4\big(\frac{\alpha \delta \abs{\SS}^\delta}{\beta \gamma}\big)^{\frac 1 {2\gamma}} \delta \abs \SS^\delta \epsilon / \beta \ .
    \end{align*}
    From the Taylor expansion of $f(x) = \sqrt{1+x}$, we see that $f(x) \geq 1 + \frac 1 2 x - \frac 1 8 x^2$.
    When $x \in [0, 1]$, we have that $f(x) \geq 1 + \frac 3 8 x$.
    In particular,
    \begin{displaymath}
      \frac{\abs{\hat \GG_{i^*}(\vec u)}}{\abs{u_{i^*}}}
      \geq 1 + \frac 3 8 \tcompress^2\frac{2\Delta+\Delta^2}{(1+\Delta)^2}
      - 4\big(\frac{\alpha \delta \abs{\SS}^\delta}{\beta \gamma}\big)^{\frac 1 {2\gamma}} \delta \abs \SS^\delta \epsilon / \beta \ .
    \end{displaymath}
    By the bound of $\epsilon \leq \frac{3}{32} \tcompress^2\frac{2\Delta + \Delta^2}{(1+\Delta)^2} \cdot \big(\frac{\beta\gamma}{\alpha \delta \abs{\SS}^\delta}\big)^{\frac 1 {2\gamma}} \frac{\beta}{\delta \abs{\SS}^\delta}$, we see that $\frac{\abs{\hat \GG_{i^*}(\vec u)}}{\abs{u_{i^*}}} \geq 1$.
  \end{subproof}
  Recall that to apply \cref{claim:robust-increasing-hi-un}, it suffices
  \begin{displaymath}
    \epsilon \leq \frac{3}{32} \tcompress^2\frac{2\Delta + \Delta^2}{(1+\Delta)^2} \cdot \big(\frac{\beta\gamma}{\alpha \delta \abs{\SS}^\delta}\big)^{\frac 1 {2\gamma}} \frac{\beta}{\delta \abs{\SS}^\delta}.
  \end{displaymath}
  We choose $\Delta = \frac 3 4 \frac {\beta \gamma}{\alpha \delta} \Big( \frac{\beta \gamma}{\alpha \delta\abs{\SS}^\delta} \Big)^{\frac{\delta - \gamma}{\gamma}}\eta$.
  We note that $\Delta \in (0, 1)$ since $\eta \in (0, 1)$.
  Thus, $\frac{2\Delta + \Delta^2}{(1+\Delta)^2} \geq \frac 1 2 \Delta$.
  % , and when $\Delta > 1$, then $\frac{2\Delta + \Delta^2}{(1+\Delta)^2} \geq 1 - \frac{1}{(1+\Delta)^2} \geq \frac 3 4 \geq 1 2$.
  % As such, $\frac{2\Delta + \Delta^2}{(1+\Delta)^2} \geq \frac 1 2\max(\Delta, 1)$, and in particular,
  It follows:
  \begin{align*}
    \frac{3}{32} \tcompress^2\frac{2\Delta + \Delta^2}{(1+\Delta)^2} \cdot \big(\frac{\beta\gamma}{\alpha \delta \abs{\SS}^\delta}\big)^{\frac 1 {2\gamma}} \frac{\beta}{\delta \abs{\SS}^\delta}
    &\geq \frac 9 {256}\tcompress^2 \cdot \frac {\beta \gamma}{\alpha \delta} \Big( \frac{\beta \gamma}{\alpha \delta\abs{\SS}^\delta} \Big)^{\frac{\delta - \gamma}{\gamma}}\eta \cdot \big(\frac{\beta\gamma}{\alpha \delta \abs{\SS}^\delta}\big)^{\frac 1 {2\gamma}} \frac{\beta}{\delta \abs{\SS}^\delta} \\
    &\geq \frac{9}{256} \frac \beta \delta \cdot \tcompress^2 \cdot \Big(\frac{\beta \gamma}{\alpha \delta}\Big)^{\frac {2\delta + 1}{2\gamma}}\abs{\SS}^{-\frac {\delta}{\gamma}(\frac 1 2 + \delta - \gamma) - \delta}\eta .
  \end{align*}
  In particular, it suffices that $\epsilon \leq \frac{9}{256} \frac \beta \delta \cdot \tcompress^2 \Big(\frac{\beta \gamma}{\alpha \delta}\Big)^{\frac {2\delta + 1}{2\gamma}}\abs{\SS}^{-\frac {\delta}{\gamma}(\frac 1 2 + \delta - \gamma) - \delta}\eta$ in order to apply \cref{claim:robust-increasing-hi-un} with the choice of $\Delta = \frac {\beta \gamma}{\alpha \delta} \Big( \frac{\beta \gamma}{\alpha \delta\abs{\SS}^\delta} \Big)^{\frac{\delta - \gamma}{\gamma}}\eta$.
  By actually applying \cref{claim:robust-increasing-hi-un}, we complete the proof.
\end{proof}

We now create a time bound for driving a new coordinate of $\vec u(0)$ to be small under the gradient iteration based on the preceding \cref{lem:robust-GI-progress}.
\begin{prop}\label{prop:ui-spread-time-bound}
  Let $\{ \vec u(n) \}_{n=0}^\infty$ be a sequence defined recursively in $\SS^{\dn - 1}$ by $\vec u(n) = \hat \GG(\vec u(n-1))$.
  Define the sets $\SS_n := \{ i \suchthat \abs{u_i(n)} \geq \tcompress \}$.
  Suppose $\abs {\SS_0} \geq 2$,
  $\SS_0 \subset [\dm]$,
  $\vec v\in \porth^{\dn - 1}$ is the stationary point of $\GG/{\sim}$ such that $v_i \neq 0$ if and only if $i \in \SS_0$,
  $\norm{\Pmap_0 \vec u} \leq \frac 1 {2\sqrt{1+2\delta}}$,
  and fix an $\eta \in (0, 1]$.
  Let
  \begin{displaymath}
    N = \Big\lceil \frac 3 {2\eta} \big(\frac{\alpha \delta}{\beta \gamma}\big)^{\frac \delta \gamma}\dm^{\frac \delta \gamma(\delta - \gamma)} \Big[\frac 1 \gamma \ln(\frac{4 \alpha \delta}{\beta \gamma}) + \frac \delta \gamma \ln \dm\Big]\Big\rceil + 2N_{\ref{prop:GI-Loop-Small-Coords-Error}} \ .
  \end{displaymath}
  If $\max_{i, j \in \SS_0} \frac {\abs{u_i(0)}/v_i}{u_j(0)/v_j} \geq (1+\eta)^2$,
  $\max_{i \in \SS_0} \abs{u_i}/v_i \geq 1$,
  and $\epsilon \leq \epsdiverge{\eta, [\dm]}$, then there exists $j \in \SS_0$ such that $\norm{\Pmap_{\compl \SS_0 \cup \{j\}} \vec u(n)} \leq 4\epsilon \delta (\abs {\SS_0}-1)^\delta / \beta$ for all $n \geq N$.
\end{prop}
\newcommand{\Nspread}[1]{\ensuremath{N_{\ref{prop:ui-spread-time-bound}}\left(#1\right)}}
For future reference, we define the expression $\Nspread{\eta}$ to be the value of $N$ in \cref{prop:ui-spread-time-bound} above.
\begin{proof}[\proofword\@of \cref{prop:ui-spread-time-bound}]
  We first use \cref{cor:P0small-closure} to see that $\norm{\Pmap_0 \vec u(n)} \leq \frac{1}{2\sqrt{1+2\delta}}$ for all $n$.
  Further, by repeated application of \cref{cor:tcompress} (with $A = [\dm]$), we see that $\compl \SS_0 \subset \compl \SS_1 \subset \compl \SS_2 \subset \cdots$, and in particular $\SS_0 \supset \SS_1 \supset \SS_2 \supset \cdots$.
  We let $N_0$ be the least integer such that $\SS_{N_0}$ is a strict subset of $\SS_0$.
  In order to compress notation, we define the constant $\kappa := \frac 3 4 \fcondexpand^{\frac{\delta}{\gamma}}\dm^{-\frac \delta \gamma (\delta - \gamma)}$.

  The proof has two parts.
  First we bound $N_0$.
  Then, we apply the small coordinate analysis from \cref{prop:GI-Loop-Small-Coords-Error} to $\vec u(N_0)$ to see that $\norm{\Pmap_{\compl \SS_{N_0}} \vec u(n)}$ becomes small as desired.
  The first part of the proof will rely on the following claim.

  \begin{claim}\label{claim:gi-expand-recursed}
    If $n < N_0$, then
    (1) $\max_{i, j \in \SS_n}\frac{\abs{u_i(n)}/v_i}{\abs{u_j(n)}/v_j} \geq (1+\kappa\eta)^n(1+\eta)^2$ and (2) $\max_{i \in \SS_n} \abs {u_i}/v_i \geq 1$.
  \end{claim}
  \begin{subproof}
    We proceed by induction on $n$.
    The base case $n=0$ is true by the givens of this Lemma.
    If the inductive hypothesis holds for some $k < N_0 - 1$, then we see that:
    \begin{displaymath}
      \max_{i, j \in \SS} \frac{\abs{u_i(k)}/v_i}{\abs{u_j(k)}/v_j} \geq (1+\kappa\eta)^k(1+\eta)^2 \geq (1+\eta)^2 \ .
    \end{displaymath}
    As such, we may apply \cref{lem:robust-GI-progress} to see that
    \begin{displaymath}
      \max_{i, j \in \SS} \frac{\abs{u_i(k+1)}/v_i}{\abs{u_j(k+1)}/v_j}
      \geq (1+\kappa\eta) \max_{i, j \in \SS} \frac{\abs{u_i(k)}/v_i}{\abs{u_j(k)}/v_j}
      \geq (1+\kappa\eta)^{k+1}(1+\eta)^2 \ .
    \end{displaymath}
    Further, part~\ref{lem:robust-GI-progress:it:3} of \cref{lem:robust-GI-progress} implies that $\max_{i\in \SS_k} \abs{u_i(k+1)/v_i} \geq 1$.
  Since $\SS_{k+1} \supset \SS_k$, it follows that $\max_{i\in \SS_{k+1}} \abs{u_i(k+1)/v_i} \geq 1$.
  \end{subproof}
  \noindent
  We now derive an upper bound for $N_0$.
  By construction, $N_0 \geq 1$.
  We note that
  \begin{displaymath}
    \max_{i, j \in \SS_{N_0-1}}\frac{\abs{u_i(N_0)}/v_i}{\abs{u_j(N_0)}/v_j}
    \leq \max_{i, j \in \SS_{N_0-1}} \frac{1/v_i}{\abs{u_j}}
    \leq \tcompress^{-1}\Big(\frac{\alpha \delta \abs {\SS_0}^\delta}{\beta \gamma}\Big)^{\frac 1 {2\gamma}}
    \leq \Big(\frac{4\alpha \delta}{\beta \gamma}\Big)^{\frac 1 \gamma}\dm^{\frac \delta \gamma} ,
  \end{displaymath}
  where we use that $\vec u$ and $\vec v$ are unit vectors in the first inequality, the bounds from the definition of $\SS_{N_0-1}$ and \cref{lem:vi-spread} for the second inequality, and that $\abs {\SS_0} \leq \dm$ combined with the definition of $\tcompress$ in the final inequality.
  From \cref{claim:gi-expand-recursed}, we obtain $\max_{i, j \in \SS_{N_0-1}}\frac{\abs{u_i(N_0-1)}/v_i}{\abs{u_j(N_0-1)}/v_j} \geq (1+\kappa\eta)^{N_0-1}(1+\eta)^2 \geq (1+\kappa\eta)^{N_0+1} \geq (1+\kappa\eta)^{N_0}$ since $\kappa \leq 1$.
  It follows that $(1+\kappa \eta)^{N_0} \leq \big(\frac{4\alpha \delta}{\beta \gamma}\big)^{\frac 1 \gamma}\dm^{\frac \delta \gamma}$, and in particular,
  \begin{displaymath}
    N_0 \leq \frac{\frac 1 \gamma \ln(\frac{4 \alpha \delta}{\beta \gamma}) + \frac \delta \gamma \ln \dm}{\ln(1+\kappa \eta)} \ .
  \end{displaymath}
  We now simplify our bound on $N_0$ using the Taylor expansion of $\ln(1+x) \geq x - \frac 1 2 x^2$.
  In particular, when $x \in [0, 1]$, $\ln(1+x) \geq \frac 1 2 x$.
  Since $\kappa \leq 1$ and $\eta \leq 1$, it follows that $\ln(1+\kappa \eta) \geq \frac 1 2 \kappa \eta$.
  In particular,
  \begin{displaymath}
    N_0 \leq \frac 2 {\kappa \eta}\Big[\frac 1 \gamma \ln\Big(\frac{4 \alpha \delta}{\beta \gamma}\Big) + \frac \delta \gamma \ln \dm \Big] \ .
  \end{displaymath}

  We now construct the final time bound for our lemma.
  Fix $j \in \SS_0 \setminus \SS_{N_0}$.
  By applying \cref{prop:GI-Loop-Small-Coords-Error} to $\vec u(N_0)$, we obtain that $\norm{\Pmap_{\compl \SS_0 \cup \{j\}} \vec u(n)} \leq \norm{\Pmap_{\compl \SS_{N_0}} \vec u(n)} \leq 4 \delta \abs{\SS_{N_0}}^\delta\epsilon / \beta$ for all $n \geq N_0 + 2N_{\ref{prop:GI-Loop-Small-Coords-Error}}$.
\end{proof}

\subsection{Jumping Out of Stagnation}\label{sec:perturb-step-analysis}

In this section, we analyze the effect of taking a random jump on the sphere from a starting point $\vec p \in \sphere^{\dn - 1}$.
In particular, we analyze steps~\ref{alg:step:draw-jump} and~\ref{alg:step:jump1} of \textsc{FindBasisElement} and demonstrate that under the random jump $\vec w \leftarrow \vec u \cos(\norm{\vec x}) + \frac{\norm{\vec x}}{\vec x}\sin(\norm{\vec x})$ from step~\ref{alg:step:jump1}, we with non-negligible probability obtain a new starting vector $\vec w$ from which running the \textsc{GI-Loop} causes a coordinate of $\vec w$ to be driven towards zero under \cref{prop:ui-spread-time-bound}.

We first recall that for $\vec p \in \sphere^{\dn - 1}$, the tangent space of the sphere $\sphere^{\dn - 1}$ is $T_{\vec p}\sphere^{\dn - 1} = \vec p^{\perp}$.
Geometrically, this can be interpreted as the plane perpendicular to $\vec p$ treating $\vec p$ as the plane's origin.
In this section, we will be particularly interested in the map $\vec x \mapsto \vec u \cos(\norm{\vec x}) + \frac{\vec x}{\norm{\vec x}}\sin(\norm{\vec x})$ from step~\ref{alg:step:jump1} of \textsc{FindBasisElement}.
This map is sometimes referred to as the exponential map on the sphere $\sphere^{\dn - 1}$.
That is, at any $\vec p \in \sphere^{\dn - 1}$ the exponential map $\exp_{\vec p} : T_{\vec p} \sphere^{\dn - 1} \rightarrow \sphere^{\dn - 1}$ is defined as
\begin{displaymath}
  \exp_{\vec p}(\vec x) =
  \vec p \cos(\norm {\vec x}) + \frac{\vec x}{\norm{\vec x}}\sin(\norm{\vec x})  ,
\end{displaymath}
where it is understood that $\exp_{\vec p}(\vec 0) = \vec p$.

We now proceed in showing that the random jump from steps~\ref{alg:step:draw-jump} and~\ref{alg:step:jump1} of \textsc{FindBasisElement} is able to break stagnation of the gradient iteration algorithm without causing any harm.
By breaking stagnation, we mean that if $\SS \subset [\dm]$ is the set of large coordinates---i.e., $\abs{u_i} \geq \tcompress$ if and only if $i \in \SS$---then with constant probability, applying the random jump to $\vec u$ should set up the preconditions of \cref{prop:ui-spread-time-bound}.
By causing no harm, we mean that if coordinates in $\compl \SS$ are very small---i.e., $\norm{\Pmap_{\compl \SS} \vec u} \leq 4\delta \abs \SS^\delta \epsilon / \beta$---then by applying the random jump, the coordinates in $\compl \SS$ remain small---i.e., $\norm{\Pmap_{\compl \SS} \vec u} \leq \tcompress$.
As we apply the gradient iteration for sufficiently many steps between random jumps in step~\ref{alg:step:gi-in-main-loop} of \textsc{FindBasisElement}, any coordinates of $\vec u$ which are small after a random jump return to being very small before the next random jump.
In this manner, the random jump causes no harm.

We first provide conditions under which the random jump causes no harm.

\begin{lem}\label{lem:jump-small-coords}
  Let $\vec u \in \SS^{\dn - 1}$.
  Let $\SS \subset [\dm]$ be such that $\norm{\Pmap_{\compl \SS} \vec u} \leq 4 \delta \abs \SS^\delta \epsilon / \beta$.
  Suppose that
  $\epsilon \leq \frac 1 {8\sqrt{2(1+2\delta)}} \tcompress \frac{\beta}{\delta \abs \SS^\delta}$,
  and suppose that $\sigma \leq \frac 1 {2\sqrt{2(1+2\delta)}} \tcompress$.
  If $\vec w$ is drawn uniformly at random from $\sigma \sphere^{\dn - 1} \cap \vec u^\perp$ and $\vec w = \exp_{\vec u}(\vec x)$, then $\norm{\Pmap_{\compl \SS} \vec u} \leq \frac{\tcompress}{\sqrt{2(1+2\delta)}}$.
\end{lem}
\begin{proof}
    We note:
  \begin{align*}
    \norm{\Pmap_{\compl \SS} \vec w}
    &= \Norm{\Pmap_{\compl \SS} [\vec u \cos (\norm{\vec x})
      + \frac {\vec x}{\norm{\vec x}}\sin(\norm{\vec x})] } \\
    &\leq \norm{\Pmap_{\compl \SS} \vec u} + \abs{\sin(\norm{\vec x})}
    \leq \norm{\Pmap_{\compl \SS} \vec u} + \norm{\vec x}
    \leq \norm{\Pmap_{\compl \SS} \vec u} + \sigma \\
    &\leq \frac \tcompress {2\sqrt{2(1+2\delta)}} +  4\epsilon \delta \abs \SS^\delta / \beta
    \leq \frac{\tcompress}{\sqrt{2(1+2\delta)}}.
  \end{align*}
  In the above, the first inequality uses the triangle inequality, that $\abs {\cos(\norm{\vec x})} \leq 1$ to obtain the first summand, and that $\norm{\Pmap_{\compl \SS}\vec u} \leq 1$ and $ \norm{\frac {\vec x}{\norm{\vec x}}} = 1$ to obtain the second summand.
  The second inequality uses the Taylor series of $\sin$ to bound $\sin(\norm {\vec x}) \leq \norm {\vec x}$.
  The third inequality uses that $\norm {\vec x} = \sigma$ since $\vec x$ is drawn from a sphere with radius $\sigma$.
  The fourth inequality uses the bounds on $\sigma$ and $\norm{\Pmap_{\compl \SS} \vec u}$.
  The final inequality uses the upper bound on $\epsilon$.
\end{proof}

Before proceeding stating conditions under which the random jump breaks stagnation, we first state two minor technical results which will useful in showing that the random jump actually creates a significant change in the coordinates of interest.


\begin{fact}\label{fact:perturb-sphere-0sep}
  Let $\sigma \geq 0$, and suppose that $\vec x$ is drawn uniformly at random from the sphere $\sigma \sphere^{n-1}$.
  If $\XX \ni \vec 0$ is a $k$-dimensional subspace of $\R^n$,
  then with probability at least $(1-\exp(-\tfrac{1}{16} k))(1 - \exp(-\tfrac{2-\sqrt 3}{2} (n-k))$, $\norm{\Pmap_{\XX} \vec x}^2 \geq \frac k {4 n}\sigma^2$.
\end{fact}
\def\cprobi{\ensuremath{C_{\ref{fact:perturb-sphere-0sep}}}}
For later usage, we denote by $\cprobi := \left(1-\exp\left(-\frac 1 {16}\right)\right)\left(1-\exp\left(-\frac {2-\sqrt 3}{2}\right)\right)$, which is a constant lower bound on the probability that is obtained in \cref{fact:perturb-sphere-0sep} with $0 < k < n$.
\begin{proof}[\proofword\@of \cref{fact:perturb-sphere-0sep}]
  We consider the following sampling process for constructing $\vec x$: (1) draw $\vec w \sim \NN(\vec 0, \Id)$, and (2) let $\vec x \leftarrow \sigma\frac{\vec w}{\norm{\vec w}}$.
  We note that this process is equivalent to drawing $\vec x$ from $\sigma \sphere^{n - 1}$ uniformly at random almost surely.
  Further, $\norm{\Pmap_{\XX} \vec w}^2$ and $\norm{\Pmap_{\XX^\perp} \vec w}^2$ are independent random variables which are distributed according to the chi-squared distribution with $k$ and $n-k$ degrees of freedom respectively.
  In particular, applying \cref{cor:chi2-concentration}, we see that with probability at least
  $$\left(1-\exp\left(-\tfrac{1}{16} k\right)\right)\left(1 - \exp\left(-\tfrac{2-\sqrt 3}{2} (n-k)\right)\right),$$
  both of the events $\norm{\Pmap_{\XX} \vec w}^2 \geq \frac 1 2 k$ and $\norm{\Pmap_{\XX^\perp} \vec w}^2 \leq 2(n-k)$ occur.

  We proceed in the setting in which these events occur.
  We see that
  \begin{displaymath}
    \frac 1 {\sigma^2} \norm{\Pmap_{\XX} \vec x}^2
    = \frac{\norm{\Pmap_{\XX} \vec w}^2}{\norm{\Pmap_{\XX} \vec w}^2 + \norm{\Pmap_{\XX^\perp} \vec w}^2}
    \geq \frac{\norm{\Pmap_{\XX} \vec w}^2}{\norm{\Pmap_{\XX} \vec w}^2 + 2(n - k)} .
  \end{displaymath}
  We note that for any $C \geq 0$, the function $f(t) = \frac t {t+C} = 1 - C(t+C)^{-1}$ has derivative $f'(t) = C(t+C)^{-2} \geq 0$.
  In particular, $f$ is an increasing function.
  As such, we obtain:
  \begin{displaymath}
    \frac 1 {\sigma^2} \norm{\Pmap_{\XX} \vec x}^2
    \geq \frac{\frac 1 2 k}{\frac 1 2 k + 2(n - k)}
    \geq \frac{\frac 1 2 k}{2 k + 2(n - k)}
    = \frac k {4n}. \qedhere
  \end{displaymath}
\end{proof}

\begin{lem}\label{lem:pert-good-growth}
  Let $\SS \subset [\dm]$ be such that $\abs \SS \geq 2$.
  Suppose that $\vec u \in \sphere^{\dn - 1}$ and
  that $\tau \leq \min_{i \in \SS} \abs {u_i}$.
  Let $\mathcal X := T_{\vec u} \sphere^{\dn - 1} \cap \spn(\{\myZv_i \suchthat i \in \SS\})$.
  Let $\vec x \in \mathcal X$ and let $s \in \{+, -\}$ be a sign.
  We define $\Lambda_s(\vec x) := \{ i \in \SS \suchthat \sign(u_i) = s \sign(x_i)\}$.
  Then, $\norm{\Pmap_{\Lambda_s} \vec x} \geq \frac \tau {\sqrt 2} \norm{\vec x}$.
\end{lem}
\begin{proof}
  Since $\vec u \perp \vec x$, it follows that $\ipCanonical{\vec u}{\Pmap_{\Lambda_+}\vec x} = - \ipCanonical{\vec u}{\Pmap_{\Lambda_-}\vec x}$.
  Further, it can be seen that
  \begin{align*}
    \norm{\Pmap_{\Lambda_+}\vec x}
    = \norm{\vec u}\norm{\Pmap_{\Lambda_+}\vec x}
    \geq \ipCanonical{\vec u}{\Pmap_{\Lambda_+}\vec x}
    =-\ipCanonical{\vec u}{\Pmap_{\Lambda_-}\vec x}
    \geq \tau \norm[1]{\Pmap_{\Lambda_-} \vec x}
    \geq \tau \norm{\Pmap_{\Lambda_-} \vec x}
  \end{align*}
  using that $1 = \norm{\vec u}$ for the first equality, the Cauchy-Schwartz inequality for the first inequality, the lower bound on $\abs{u_i} \geq \tau$ for the second inequality, and the relationship $\norm[1]\argdot \geq \norm[2]\argdot$ for the final inequality.
  By similar reasoning swapping the roles of $\Lambda_+$ and $\Lambda_-$, we obtain:
  \begin{displaymath}
    \norm{\Pmap_{\Lambda_-} \vec x} \geq \tau \norm{\Pmap_{\Lambda_+}\vec x} \ .
  \end{displaymath}

  We note that one of $\norm{\Pmap_{\Lambda_+} \vec x}$ and $\norm{\Pmap_{\Lambda_-} \vec x}$ must be at least $\frac 1 {\sqrt 2} \norm{\vec x}$ by the Pytha\-gorean Theorem.
  In particular, both $\norm{\Pmap_{\Lambda_+} \vec x}$ and $\norm{\Pmap_{\Lambda_-} \vec x}$ are at least $\frac \tau {\sqrt 2} \norm{\vec x}$.
\end{proof}

The following fact will be useful when bounding individual coordinates of $\exp_{\vec u} (\vec x)$ for the random jump.
\begin{fact}\label{fact:sin-cos-bounds1}
  The trigonometric functions $\sin t$ and $\cos t$ can be lower bounded as follows:
  \begin{enumerate}
  \item When $t \in [0, 1]$, then $\sin t \geq \frac 2 3 t$.
  \item $\cos t \geq 1 - \frac 1 2 t^2$.
  \end{enumerate}
\end{fact}
\begin{subproof}
  We use the Taylor series of $\sin t$ and $\cos t$.
  For $\cos t$, this is a direct implication of the Taylor expansion.
  For $\sin t$, we note that $\sin t \geq t - \frac 1 3 t^3 \geq \frac 2 3  t$.
\end{subproof}

In the remaining Lemmas of this section, we provide conditions under which the random jump from step~\ref{alg:step:jump1} of \textsc{FindBasisElement} sets up the preconditions of \cref{prop:ui-spread-time-bound} with constant probability.
We first deal with the case where we are stagnated.
%We are stagnated if we do not have the necessary preconditions for progress under \cref{prop:ui-spread-time-bound}:
We say that the gradient iteration is stagnated for a choice of $\vec u$ if for the fixed point $\vec v$ of $\GG/{\sim}$ such that $v_i \neq 0$ if and only if $i$ is a ``large'' coordinate of $\vec u$, there is no $i$ among the large coordinates such that $\abs{u_i} > \abs{v_i}$ with a sufficient gap (as defined in the preconditions of \cref{prop:ui-spread-time-bound}).
We demonstrate that with at least constant probability, stagnation can be escaped by the random jump.
In the following Lemma, $C_{\ref{lem:lpert-analysis-expected}}$ is a strictly positive universal constant.
\begin{lem}\label{lem:lpert-analysis-expected}
  Let $\SS \subset [\dm]$ contain at least 2 elements.
  Let $\vec u \in \SS^{\dn - 1}$.
  Let $\vec v \in \porth^{\dn - 1}$ be the fixed point of $\GG / {\sim}$ such that $v_i \neq 0$ if and only if $i \in \SS$.
  Let $\eta := C_{\ref{lem:lpert-analysis-expected}} \frac{\sigma}{\sqrt \dn}(\frac {\beta \gamma}{\alpha \delta\abs \SS^\delta})^{\frac 1 \gamma} \tcompress^2$.
  Suppose that $\vec w$ is a random jump of $\vec u$ created according to the following process:
  Draw $\vec x$ uniformly at random from $\sigma \sphere^{\dn - 1} \cap \vec u^\perp$ and let $\vec w = \exp_{\vec u}(\vec x)$.


  If $\abs{u_i} \geq \tcompress$ for all $i \in \SS$,
  if $\norm{\Pmap_{\compl \SS} \vec u} \leq 4 \epsilon \delta \abs \SS^\delta / \beta$,
  if $\epsilon \leq \epsdiverge{\eta, \abs \SS}$,
  if $\sigma \leq \frac{1}{6\sqrt{2 \dn}}\tcompress^2 $,
  and if $\frac {\abs{u_i}}{v_i} < (1+\eta)^2$ for all $i \in \SS$,
  then with probability at least $\cprobi$, there exists $i \in \SS$ such that $\frac{\abs {w_i}}{v_i} \geq (1+\eta)^2$.
\end{lem}
\begin{proof}
  The main crux of the argument is captured in the following two claims.
  These claims use the construction of $\vec w$ and the choice of $\vec u$ from the lemma statement as unstated givens.
  \begin{claim}\label{claim:gi-precond-setup}
    Fix a constant $\Delta > 0$.
    Define $\kappa := \norm{\Pmap_{\compl \SS } \vec u}^2 + (1+\Delta)^2 - 1$. Suppose that $\kappa \leq \frac 1 2 (\frac{\beta \gamma}{\alpha \delta \abs \SS})^{\frac 1 {2\gamma}}$, and
    that $\frac{\abs{u_i}}{v_i} \leq 1 + \Delta$ for all $i \in \SS$ and that
    \begin{displaymath}
    {12\sqrt{2\dn}}\Big(\frac{\alpha \delta \abs \SS^\delta}{\beta \gamma}\Big)^{\frac 1 {\gamma}}\kappa / \tcompress^2
    \leq \sigma
    \leq \frac 1 {6\sqrt {2 \dn}} \tcompress^2 \ ,
    \end{displaymath}
    then with probability at least $\cprobi$, there exists $j \in \SS$ such that $\frac{\abs{w_j}}{v_j} \geq 1 + \Delta$.

    \vnote{Use case:  We will be plugging into the Lemma 6.15 preconditions to make $\abs{u_i}/\abs{v_i} \geq (1+\eta)^2$.  As such, we choose $\Delta$ large enough that $1+\Delta \geq (1 + \eta)^2$.  For this purpose, we may assume that $\eta \leq 1$.
    At the end, we will need to determine the appropriate $\epsilon$.}
  \end{claim}
  % \resetcasecount
  % \begin{case}
  %   Suppose that $\abs{u_i} \leq v_i + \Delta$ for all $i \in \SS$.
  % \end{case}
  \begin{subproof}
    We prove this claim in several parts.
    First, we demonstrate a lower bound on $\abs{u_i}$ in terms of $v_i$ for each $i \in \SS$.
    Then, we demonstrate that for some $j \in \SS$, $x_j$ is sufficiently large to make $\abs{w_j}/v_j \geq 1 + \Delta$.

    We now proceed with constructing a lower bound on the $\abs {u_i}$s.
    We fix a $j \in \SS$.
    \begin{align}
      u_j^2
      &= 1 - \norm{\Pmap_{\compl \SS}\vec u}^2 - \sum_{i \in \SS \setminus \{j\}} u_i^2
      = 1 - \norm{\Pmap_{\compl \SS}\vec u}^2 - \sum_{i \in \SS \setminus \{j\}} \frac{u_i^2}{v_i^2}v_i^2 \nonumber \\
      &\geq 1 - \norm{\Pmap_{\compl \SS}\vec u}^2 - (1+\Delta)^2\sum_{i \in \SS \setminus \{j\}} v_i^2 % \nonumber \\
      = 1 - \norm{\Pmap_{\compl \SS}\vec u}^2 - (1+\Delta)^2[1 - v_j^2] \nonumber \\
      % &= 1 - \norm{\Pmap_{\compl \SS} \vec u}^2 - \sum_{i \in \SS} \frac{u_i^2}{v_i^2}v_i^2 + \frac{u_j^2}{v_j^2}v_j^2  \nonumber \\
      &\geq v_j^2(1+\Delta)^2 - [(1+\Delta)^2-1 + \norm{\Pmap_{\compl \SS} \vec u}^2]
      = v_j^2(1+\Delta)^2 - \kappa . \label{eq:nearv-coord-lb}
    \end{align}

    We now demonstrate that with a random jump from $\vec u$, one of the coordinates $j \in \SS$ increases sufficiently from the lower bound in \cref{eq:nearv-coord-lb} with the desired probability.
    First, we note that there exists a 1-dimensional subspace $\mathcal \XX \subset \vec u^\perp \cap \spn(\myZv_{i_1}, \myZv_{i_2})$, where $i_1, i_2 \in \SS$.
    Let $\vec p$ be a unit vector in $\mathcal \XX$.
    We may apply \cref{fact:perturb-sphere-0sep} to obtain with probability at least $\cprobi$
    that $\abs{\ipCanonical{\vec p}{\vec x}} \geq \frac \sigma {2\sqrt{\dn - 1}} \geq \frac \sigma {2\sqrt \dn}$.
    We proceed under the assumption that this event occurs.

    Letting $\Lambda_+ := \{ i \in \{i_1, i_2\} \suchthat \sign(x_i) = \sign(u_i) \}$, we apply \cref{lem:pert-good-growth} to obtain $\norm{\Pmap_{\Lambda_+} \vec x} \geq \frac \tcompress {\sqrt 2} \norm{\vec x} \geq \frac 1 {2\sqrt {2\dn}} \sigma \tcompress$.
    In particular, there exists $j \in \SS$ such that $\sign(u_j)x_j \geq \frac 1 {2\sqrt {2\dn}} \sigma \tcompress$.
    It only remains to be seen that for this choice of $j$, $\abs{w_j}/\abs{v_j} \geq 1 + \Delta$.

    We note (using that $\norm{\vec x} = \sigma$):
    \begin{equation}\label{eq:lpert-1}
      w_j^2
      = [\exp_{\vec u}(\vec x)]_j^2
      \geq u_j^2 \cos^2(\sigma) + 2 u_j \cos( \sigma ) \frac{x_j}{\sigma}\sin(\sigma)
    \end{equation}
    Using \cref{fact:sin-cos-bounds1}, we see that
    \begin{displaymath}
      \cos^2(\sigma)
      \geq [1 - \frac 1 2 \sigma^2]^2
%      = [1-\frac 1 2 \sigma^2]^2
      \geq 1 - \sigma^2 \ .
    \end{displaymath}
    Further, since $\sigma \leq \tcompress \leq 1 < \frac \pi 3$, we see that $\cos(\sigma) \geq \frac 1 2$.
    Thus,
    \begin{displaymath}
      2 u_j \cos( \sigma ) \frac{x_j}{\sigma}\sin(\sigma)
      \geq u_j \frac{x_j}{\sigma}\sin(\sigma)
      \geq \frac 2 3 u_j x_j
      \geq \frac 1 {3\sqrt{2\dn}} \sigma \tcompress^2
    \end{displaymath}
    where we use \cref{fact:sin-cos-bounds1} in the second inequality and the lower bounds on $x_j$ and $u_j$ in the final inequality.
    Continuing from \cref{eq:lpert-1}, we obtain:
    \begin{align*}
      w_j^2
      &\geq (1-\sigma^2)u_j^2 + \frac 1 {3\sqrt{2\dn}} \sigma \tcompress^2
      \geq u_j^2[1-\sigma^2 + \frac 1 {3\sqrt {2\dn}}\sigma \tcompress^2] \\
      &\geq u_j^2[1+\frac 1 {6\sqrt{2\dn}} \sigma \tcompress^2]
      \geq \big[v_j^2(1+\Delta)^2 - \kappa \big] \cdot [1+\frac 1 {6\sqrt{2\dn}} \sigma \tcompress^2]
    \end{align*}
    by using the upper bound on $\sigma$ in the third inequality, and by applying \cref{eq:nearv-coord-lb} in the final inequality.
    Using the lower bound on $\sigma$, we see that
    \begin{align*}
    w_j^2
    &\geq [v_j^2(1+\Delta)^2 - \kappa]\Big[1 + 2\Big(\frac{\alpha \delta}{\beta \gamma}\abs\SS^\delta\Big)^{\frac 1 {\gamma}}\kappa \Big] \\
    &= v_j^2(1+\Delta)^2 + \kappa\left(2v_j^2\Big(\frac{\alpha \delta}{\beta \gamma}\abs\SS^\delta\Big)^{\frac 1 {\gamma}}(1+\Delta)^2 - 1 - 2\Big(\frac{\alpha \delta}{\beta \gamma}\abs\SS^\delta\Big)^{\frac 1 {\gamma}}\kappa\right) \\
    &\geq v_j^2(1+\Delta)^2 + \kappa\left(2 - 1 - 1\right)
    = v_j^2(1+\Delta)^2  ,
    \end{align*}
    where we use the lower bound on $v_j^2$ from \cref{lem:vi-spread} and the assumed upper bound on $\kappa$ in the final inequality.
    Rearranging terms completes the proof.
  \end{subproof}

  \begin{claim}\label{claim:gi-precond-setup2}
    Let $\lambda \in (0, 1]$ and set $\sigma = \frac {\lambda} {6\sqrt{2\dn}} \tcompress^2$.
    Suppose $\eta = \frac{C_1 \lambda}{\dn}\Big(\frac{\beta \gamma}{\alpha \delta \abs \SS^\delta}\Big)^{\frac 1 \gamma} \tcompress^4$ (where $C_1$ is a universal constant which happens to satisfy $C_1 \in (0, 1)$),
    and suppose $\epsilon \leq \epsdiverge{\eta, \SS}$.
    Then, with probability at least $\cprobi$, there exists $i \in \SS$ such that $\frac{\abs{w_i}}{v_i} \geq (1 + \eta)^2$.
  \end{claim}
  \begin{subproof}
  During the proof, we will wish to apply \cref{claim:gi-precond-setup} with $1+\Delta = (1+\eta)^2$.
  Since $\eta \leq 1$, we have that
  \begin{displaymath}
    (1+\Delta)^2
    = (1+\eta)^4
    = 1 + 4\eta + 6\eta^2 + 4\eta^3 + \eta^4
    \leq 1 + 15 \eta \ .
  \end{displaymath}
  As such, we may bound the expression $\kappa := \norm{\Pmap_{\compl \SS} \vec u}^2 + (1+\Delta)^2 - 1$ by
  \begin{displaymath}
    \kappa
    \leq 4 \delta \abs \SS^\delta \epsilon / \beta + 15 \eta
    < 16 \eta ,
  \end{displaymath}
  where we use a loose version of our bound $\epsilon \leq \epsdiverge{\eta, \SS}$ in the final inequality.
  We note that with the universal constant $C_1 = \frac 1 {2304} = \frac 1 {12\sqrt 2 \cdot 6\sqrt 2 \cdot 16}$, we obtain that
  \begin{displaymath}
    12\sqrt{2\dn}\Big(\frac{\alpha \delta \abs \SS^\delta}{\beta \gamma}\Big)^{\frac 1 \gamma} \frac{\kappa}{\tcompress^2}
    \leq 16 \cdot 12\sqrt{2\dn}\Big(\frac{\alpha \delta \abs \SS^\delta}{\beta \gamma}\Big)^{\frac 1 \gamma} \frac{\eta}{\tcompress^2}
    = \frac{\lambda}{6\sqrt{2\dn}} \tcompress^2
    = \sigma
  \end{displaymath}
  by using the upper bound on $\kappa$ in the inequality,
  by using the given choice of $\eta$ in the first equality,
  and by using the choice of $\sigma$ in the second equality.
  As such, we may apply \cref{claim:gi-precond-setup} to obtain that with probability at least $\cprobi$, there exists $i \in \SS$ such that $\abs{w_i} / v_i \geq (1+\eta)^2$.
   \end{subproof}
   To complete the proof, we apply \cref{claim:gi-precond-setup2}.
%    and $\eta$ as a function of $\sigma$.
   We note that
   \begin{displaymath}
     \eta = O\Big(\frac{\sigma}{\sqrt{\dn}}\Big(\frac{\beta \gamma}{\alpha \delta \abs \SS^\delta}\Big)^{\frac 1 \gamma}\tcompress^2\Big).
   \end{displaymath}
   In particular, it suffices that $\epsilon$ be upper bounded by $O\big(\epsdiverge{\frac{\sigma}{\sqrt{\dn}}(\frac{\beta \gamma}{\alpha \delta \abs \SS^\delta})^{\frac 1 \gamma}\tcompress^2, \abs \SS} \big)$.
\end{proof}

In the following two Lemmas, we consider the case where the gradient iteration is not stagnated, and we demonstrate with at least constant probability the random jump does not move us into stagnation.
In \cref{lem:jump-with-large-coord}, we deal with the case that the preconditions of \cref{prop:ui-spread-time-bound} are actually met, and we demonstrate that with some constant probability, applying the random jump does not cause the essential preconditions for gradient iteration progress to be undone.
Finally, in \cref{lem:jump-with-small-coord}, we demonstrate that if there is a coordinate of $\vec u$ which is not known to be small but has decreased beneath the threshold $\tcompress$, then applying the random jump leaves that coordinate small with constant probability.
In essence, these Lemmas demonstrate that the random jump does not undo unforeseen progress of the gradient iteration.
\begin{lem}\label{lem:jump-with-large-coord}
  Let $\SS \subset [\dm]$,
  let $\vec u \in \sphere^{\dn - 1}$,
  let $\eta > 0$ be a constant,
  and let $\vec v \in \porth^{\dn - 1}$ be the fixed point of $\GG/{\sim}$ such that $v_i \neq 0$ if and only if $i \in \SS$.
  %Suppose that $\abs{u_i} \geq \tcompress$ for all $i \in \SS$.
  Let $\vec w$ be constructed according to the following random process:
  Draw $\vec x$ uniformly at random from $\sigma \sphere^{\dn - 1} \cap \vec u^\perp$, and let $\vec w = \exp_{\vec u}(\vec x)$.

  If $\abs{u_i} \geq \tcompress$ for all $i \in \SS$,
  if there exists $j \in \SS$ such that $\abs{u_j} \geq (1+\eta)^2v_j$,
  and if $\sigma \leq \frac 2 {3\sqrt {2 \dn}} \tcompress$,
  then with probability at least $\frac 1 2 \cprobi$ we obtain $\abs{w_j} \geq \abs {u_j}$ and in particular $\abs{w_j} \geq (1+\eta)^2v_j$.
\end{lem}
\begin{proof}
  Since $\abs{u_j} > v_j$, it follows that $\vec v$ is not a canonical vector, and in particular that $\abs{\SS} \geq 2$.
  We set $A = \{ i, j \}$ by choosing $i \neq j$ such that $i \in \SS$.
  We apply \cref{fact:perturb-sphere-0sep} to see that with probability at least $\cprobi$, $\norm{\Pmap_A \vec x} \geq \frac 1 {2\sqrt \dn} \sigma$.
  Further, by the spherical symmetry of the distribution of $\vec x$, with probability at least $\frac 1 2 \cprobi$ both $\sign(u_j) x_j \geq 0$ and $\norm{\Pmap_A \vec x} \geq \frac 1 {2\sqrt \dn} \sigma$.
  We proceed under the assumption that this event occurs.

  Applying \cref{lem:pert-good-growth} with $\tau = \tcompress$, we see that $\abs{x_j} \geq \frac \tcompress {\sqrt 2} \norm{\Pmap_{A} \vec x} \geq \frac \tcompress {2\sqrt{2\dn}}\sigma$.
  As such, we obtain:
  \begin{align*}
    \abs{w_j}
    &= \abs{(\exp_{\vec u}(\vec x))_j}
    = \abs{u_j \cos(\sigma) + \frac 1 \sigma x_j \sin(\sigma)}
    \geq \abs{u_j (1-\frac 1 2 \sigma^2) + \frac 2 3 x_j} \\
    &\geq \abs{u_j}(1 - \frac 1 2 \sigma^2) + \frac \tcompress {3\sqrt{2\dn}} \sigma
    \geq \abs {u_j} - \frac 1 2 \sigma^2 + \frac \tcompress {3\sqrt{2\dn}} \sigma
    \geq \abs {u_j},
  \end{align*}
  where we use that $\norm{\vec x} = \sigma$ in the second equality,
  \cref{fact:sin-cos-bounds1} in the first inequality,
  that $\abs {u_j} \leq 1$ in the third inequality,
  and the bound on $\sigma$ in the final inequality.
\end{proof}

\begin{lem}\label{lem:jump-with-small-coord}
  Let $\vec u \in \sphere^{\dn - 1}$
  Suppose there exists $j \in [\dn]$ such that $\abs{u_j} \leq \tcompress$.
  Let $\vec w$ be a random jump of $\vec u$ constructed by the following process:
  Draw $\vec x$ uniformly at random from $\sigma \sphere^{\dn - 1} \cap \vec u^\perp$, and let $\vec w = \exp_{\vec u}(\vec x)$.

  If $\sigma \leq \frac 1 2 \tcompress$, then with probability at least $\frac 1 2$, $\abs{w_j} \leq \tcompress$.
\end{lem}
\begin{proof}
  We will assume without loss of generality that $u_j \geq 0$.
  Using the spherical symmetry of the sampling process, we see that with probability at least $\frac 1 2$, $x_j \leq 0$.
  We proceed under the assumption that this event occurs.
  We first upper bound $w_j$:
  \begin{displaymath}
    w_j
    = (\exp_{\vec u}(\vec x))_j
    = u_j \cos(\sigma) + \frac 1 \sigma x_j \sin(\sigma)
    \leq u_j \leq \tcompress .
  \end{displaymath}
  since both $\cos(\sigma) \leq 1$ and $x_j \leq 0$.
  Further, we may also lower bound $w_j$:
  \begin{align*}
    w_j
    &= u_j \cos(\sigma) + \frac 1 \sigma x_j \sin(\sigma)
    \geq u_j ( 1 - \frac 1 2 \sigma^2 ) - \abs{x_j}
    \geq - \frac 1 2 \tcompress \sigma^2  - \sigma \\
    &\geq - \frac 1 8 \tcompress^3 - \frac 1 2 \tcompress
    > - \tcompress,
  \end{align*}
  where we use \cref{fact:sin-cos-bounds1} to bound $\cos(\sigma)$ and $\sin(\sigma) \leq \sigma$ to bound $\sin(\sigma)$ in the first inequality,
  we use $0 \leq u_j \leq \tcompress$ in the second inequality,
  we use the given bound $\sigma \leq \frac 1 2 \tcompress^2$ in the third inequality,
  and we use $\tcompress \leq 1$ in the final inequality.
\end{proof}

\subsection{Gradient Iteration Proof of Robustness}

We now have all of the technical tools needed to prove that \textsc{RobustGI-Recovery} robustly recovers the hidden basis elements.
To do so, we first demonstrate that \textsc{FindBasisElement} can be used to approximate a single undiscovered basis element.
We then show that by repeated application of \textsc{FindBasisElement}, all hidden basis elements may be recovered.
In particular, we now prove this section's main theoretical results (\cref{thm:single-recovery-main,thm:full-recovery-main}).
We restate each theorem with more precise bounds before its proof.

For clarity, we denote strictly positive universal constant by $C_0, C_1, C_2, ... $.
\begin{thm}\label{thm:single-recovery-main-reprise}
  Suppose $\sigma \in \left(0, \frac 1 {6\sqrt {2\dn(1+2\delta)}} \tcompress^2\right]$ and
  \begin{displaymath}
    \epsilon \leq C_0 \epsdiverge{\frac{\sigma}{\sqrt \dn}\left(\frac {\beta \gamma}{\alpha \delta \dm^\delta}\right)^{\frac 1 \gamma}\tcompress^2, [\dm]}\dn^{-\delta} \ .
  \end{displaymath}
  Let $p_{\ref{thm:single-recovery-main-reprise}} \in (0,1)$.
  Suppose $N_1 \geq 2\Nsc$,
  $N_2 \geq 2\Nsc+C_0\Nspread{\frac{\sigma}{\sqrt \dn}(\frac {\beta \gamma}{\alpha \delta \dm^\delta})^{\frac 1 \gamma}\tcompress^2}$,
  and $I \geq C_1 \dm \lceil \log(\dm / p_{\ref{thm:single-recovery-main-reprise}}) \rceil$.
  Let $\pi$ be a permutation of $[\dm]$, let $s_1, \dotsc, s_k \in \{\pm 1\}$, and suppose that $\norm{s_i \gvec \mu_i - \myZv_{\pi(i)}} \leq 4\sqrt 2 \delta \epsilon / \beta$ for each $i \in [k]$.

  If we execute $\gvec \mu_{k+1} \leftarrow \textsc{FindBasisElement}(\{\gvec \mu_1, \dotsc, \gvec \mu_k\}, \sigma)$, then with probability at least $1 - p_{\ref{thm:single-recovery-main-reprise}}$, there will exist $s_{k+1} \in \{\pm 1\}$ and an index $j \in [\dm] \setminus [k]$ such that $\norm{s_{k+1} \gvec \mu_{k+1} - \myZv_{\pi(j)}} \leq 4\sqrt 2 \delta \epsilon / \beta$.
\end{thm}
\begin{proof}
  We define the set $A_1 := \{ \pi(\ell) \suchthat \ell \in [k] \}$.
  Notice that $\abs {A_1} = k$.
  By \cref{lem:main-loop-precondition}, we see that $\norm{(\Pmap_0 + \Pmap_{A_1}) \vec u} \leq 4(\dm - \abs {A_1})^\delta\delta \epsilon / \beta$ at the beginning of the first execution of the main loop of \textsc{FindBasisElement}.
  We now establish the following loop invariant.
  \begin{claim}\label{claim:main-loop-invariant}
    Suppose that at the start of the $i$\textsuperscript{th} iteration of the main loop of \textsc{FindBasisElement}, there exists $A_i \subset [\dm]$ such that $\norm{(\Pmap_0 + \Pmap_{A_i}) \vec u} \leq 4 (\dm - \abs {A_i})^\delta \delta \epsilon / \beta$.
    Then,
    \begin{enumerate}
    \item\label{main-loop-invariant:item:1}
      At the end of the $i$\textsuperscript{th} iteration of the main loop, there exists $A_{i+1} \subset [\dm]$ such that $A_{i+1} \supset A_i$ and $\norm{(\Pmap_0 + \Pmap_{A_{i+1}})\vec u} \leq 4(\dm - \abs{A_{i+1}})^\delta \epsilon / \beta$.
    \item\label{main-loop-invariant:item:2}
      If $\abs{A_i} \leq \dm - 2$, then with probability at least $\frac 1 2 \cprobi$, $A_{i+1}$ from part~\ref{main-loop-invariant:item:1} is a strict superset of $A_i$.
    \end{enumerate}
  \end{claim}
  \begin{subproof}
    We define $\SS_i := [\dm] \setminus A_i$.
    We proceed in our analysis at the start of the $i$\textsuperscript{th} iteration of the main loop of \textsc{FindBasisElement}.
    We view $\SS_i$ as being the set of large coordinates of $\vec u$.
    If for each $\ell \in \SS_i$, $\abs{u_\ell} \geq \tcompress$, then this is true in the informal sense that we have considered throughout our discussions.
    However, this is not guaranteed, and we must proceed in distinct cases.
    In all cases, we will make use of the following two facts (without explicitly saying we are doing so) when applying previous lemmas about the random jump and its effects:
    \begin{enumerate}
    \item At the start of the current iteration of the main loop, $\norm{\Pmap_{\compl \SS_i} \vec u} \leq 4 \delta \abs{\SS_i}^\delta \epsilon/\beta $.
    \item At the end of the execution of line~\ref{alg:step:jump1} of \textsc{FindBasisElement}, $\norm{\Pmap_{\compl \SS_i} \vec w} \leq \frac{\tcompress}{\sqrt{2(1+2\delta)}}$.
    In particular, this means $\norm{\Pmap_0 \vec w} \leq \frac 1 {\sqrt{2(1+2\delta)}}$ and $\norm{\Pmap_{\compl \SS_i} \vec w} \leq \tcompress$.
    \end{enumerate}
    To see the first fact, we use that $\norm{\Pmap_{\compl \SS_i} \vec u} = \norm{(\Pmap_0 + \Pmap_{A_i})\vec u} \leq 4 \delta (\dm - \abs{A_i})^\delta \delta \epsilon / \beta = 4\delta \abs{\SS_i}^\delta \epsilon/\beta$.
    To see the second fact, we apply \cref{lem:jump-small-coords} and recall also that $\tcompress < 1$ and $\delta > 0$.

    We let $\vec v \in \porth^{\dn - 1}$ be the fixed point of $\GG/{\sim}$
    such that $v_j \neq 0$ if and only if $j \in \SS_i$.
    We define
    $\eta := C_{\ref{lem:lpert-analysis-expected}} \frac{\sigma}{\sqrt \dn}(\frac {\beta \gamma}{\alpha \delta \dm^\delta})^{\frac 1 \gamma}\tcompress^2$.
    \resetcasecount
    \begin{case}
      $\abs{u_j} \geq \tcompress$ and $\abs{u_j} < (1+\eta)^2v_j$ for all $j \in \SS_i$.
    \end{case}
    \begin{caseblock}
      If $\abs{\SS_i} \geq 2$, then we apply
      \cref{lem:lpert-analysis-expected} to see that with probability at
      least $\cprobi$, at the end of line~\ref{alg:step:jump1} of
      \textsc{FindBasisElement} there exists $\ell \in \SS_i$ such that
      $\abs{w_\ell}/v_\ell \geq (1+\eta)^2$.
      If this happens, we apply \cref{prop:ui-spread-time-bound} to see
      that at the end of end of the current iteration of the main loop of \textsc{FindBasisElement}, there exists $j
      \in \SS_i$ such that $\norm{\Pmap_{\compl \SS_{i} \cup \{j\}} \vec u}
      \leq 4\epsilon\delta(\abs {\SS_i} - 1)^\delta / \beta$.
      In particular, when this occurs, we define $A_{i+1} := A_i \cup \{j\}$,
      and we see that $\norm{\Pmap_{\compl \SS_{i} \cup \{j\}} \vec u} =
      \norm{(\Pmap_0 + \Pmap_{A_{i+1}})\vec u} \leq 4\epsilon\delta(\dm - \abs
      {A_{i+1}})^\delta / \beta$ at the end of the $i$\textsuperscript{th}
      iteration of the main loop.

      If it occurs that there is no $\ell \in \SS_i$ such that
      $\abs{w_\ell}/v_\ell \geq (1+\eta)^2$, we define $A_{i+1} := A_i$ and
      apply \cref{prop:GI-Loop-Small-Coords-Error} to see that at
      the end of the $i$\textsuperscript{th} iteration of the main loop,
      $\norm{(\Pmap_0 + \Pmap_{A_{i+1}})\vec u} \leq 4\epsilon\delta(\dm -
      \abs {A_{i+1}})^\delta / \beta$.
    \end{caseblock}
    \begin{case}
      $\abs{u_j} \geq \tcompress$ for all $j \in \SS_i$ and there exists $\ell \in [\dm]$ such that $\abs{u_\ell} \geq (1+\eta)^2v_\ell$.
    \end{case}
    \begin{caseblock}
      We apply \cref{lem:jump-with-large-coord} to see that with
      probability at least $\frac 1 2 \cprobi$, at the end of
      line~\ref{alg:step:jump1} of \textsc{FindBasisElement} there exists
      $\ell \in \SS_i$ such that $\abs{w_\ell}/v_\ell \geq (1+\eta)^2$.
      When this occurs, we apply \cref{prop:ui-spread-time-bound} to see
      that at the end of the current iteration of the main loop of \textsc{FindBasisElement}, there exists $j
      \in \SS_i$ such that $\norm{\Pmap_{\compl \SS_{i} \cup \{j\}} \vec u}
      \leq 4\epsilon\delta(\abs {\SS_i} - 1)^\delta / \beta$.
      In particular, we define $A_{i+1} := A_i \cup \{ j
      \}$, and we see that $\norm{\Pmap_{\compl \SS_{i} \cup \{j\}} \vec u} =
      \norm{(\Pmap_0 + \Pmap_{A_{i+1}})\vec u} \leq 4\epsilon\delta(\dm - \abs
      {A_{i+1}})^\delta / \beta$ at the end of the $i$\textsuperscript{th}
      iteration of the main loop.

      If it happens that there is no $\ell \in \SS_i$ such that
      $\abs{w_\ell}/v_\ell \geq (1+\eta)^2$, we define $A_{i+1} := A_i$ and
      apply \cref{prop:GI-Loop-Small-Coords-Error} to see that at
      the end of the $i$\textsuperscript{th} iteration of the main loop,
      $\norm{(\Pmap_0 + \Pmap_{A_{i+1}})\vec u} \leq 4\epsilon\delta(\dm -
      \abs {A_{i+1}})^\delta / \beta$.
    \end{caseblock}
    \begin{case}
      There exists $\ell \in \SS_i$ such that $\abs{u_\ell} < \tcompress$.
    \end{case}
    \begin{caseblock}
      We apply \cref{lem:jump-with-small-coord} to see that with probability at least $\frac 1 2$, $\abs{w_\ell} \leq \tcompress$ at the end of the execution of line~\ref{alg:step:jump1} of \textsc{FindBasisElement}.
      If this occurs, we define $A_{i+1} := A_i \cup \{\ell\}$, and otherwise we define $A_{i+1} := A_i$.
      Then, applying \cref{prop:GI-Loop-Small-Coords-Error}, we see that $\norm{(\Pmap_0 + \Pmap_{A_{i+1}})\vec u} \leq 4(\dm - \abs{A_{i+1}})^\delta \epsilon / \beta$.
    \end{caseblock}
    \noindent
    Note that in all three cases, we have the following summary outcome:  If $\abs {\SS_i} \geq 2$, then with probability at least $\frac 1 2 \cprobi$, there exists $A_{i+1}$ a strict superset of $A_i$ such that
    $\norm{(\Pmap_0 + \Pmap_{A_{i+1}})\vec u}
    \leq 4\epsilon\delta(\dm - \abs {A_{i+1}})^\delta / \beta$.
    Further, it is guaranteed that there exists $A_{i+1} \supset A_i$ (where the superset is not necessarily strict) such that
    $\norm{(\Pmap_0 + \Pmap_{A_{i+1}})\vec u}
    \leq 4\epsilon\delta(\dm - \abs {A_{i+1}})^\delta / \beta$ at the end of the current iteration of the main loop of \textsc{FindBasisElement}.
    Noting that $\abs{\SS_i} \geq 2$ if and only if $\abs{A_i} \leq \dm - 2$ completes the proof of the claim.
  \end{subproof}
  To complete the proof, we will apply \cref{claim:main-loop-invariant} and study the state of $\vec u$ at the return statement of line~\ref{alg:step:exit} of \textsc{FindBasisElement}.

  To begin with, we note that if $A_{I+1}$ can contain at most $\dm - 1$ elements, since otherwise $\abs{A_{I+1}} = \dm$ would imply that $\norm{\vec u} = \norm{(\Pmap_0 + \Pmap_{A_{I+1}})\vec u} = 0$.
  Since all steps of \textsc{FindBasisElement} maintain that $\vec u \in \sphere^{\dn - 1}$, this would contradict that $\vec u$ is a unit vector.

  If $\abs{A_{I+1}} = \dm - 1$, then the loop invariant from \cref{claim:main-loop-invariant} implies that $A_{I+1} \supset A_1$, and hence the lone $j \in A_{I+1}$ satisfies $j \not \in \{\pi(1), \dotsc, \pi(\abs{A_1})\}$.
  By applying \cref{lem:hbe-error-bound}, we see that there exists $s_{k+1} \in \{\pm 1\}$ such that
  $\norm{s_{k+1}\vec u - \myZv_j}
  \leq \norm{(\Pmap_0 + \Pmap_{A_{I+1}})\vec u}^2 \sqrt 2
  \leq 4\sqrt 2 \delta \epsilon / \beta$ as desired.

  It only remains to be seen that $\abs{A_{I+1}} \geq \dm - 1$ with the claimed probability.
  To see this, it suffices to show that the size of $\abs{A_i}$ increases at least $\dm - k - 1$ times during the execution of the main loop.
  We will make use of the following claim:
  \begin{claim}\label{claim:main-probability-accumulation}
    Suppose that at the beginning of the $i_j$\textsuperscript{th} iteration of the main loop of \textsc{FindBasisElement} that $\abs{A_i} < \dm - 1$.
    Let $\eta \in (0, 1)$.
    If $N \geq \log(\frac 1 \eta) / \log((1 - \frac 1 2 \cprobi)^{-1})$, then after $N$ additional iterations of the main loop, with probability at least $1 - \eta$, $A_{i+N}$ is a strict superset of $A_i$.
  \end{claim}
  \begin{subproof}
%    After each additional iteration, .
    Using the probability bound $\frac 1 2 \cprobi$ from \cref{claim:main-loop-invariant} and that the random jumps in \textsc{FindBasisElement} are independent of each other, we see that $\Pr[A_{i+N} = A_i]$ is bounded by
    \begin{align*}
      \Pr[A_{i+N} = A_i]
      &\leq (1 - \frac 1 2 \cprobi)^N
      \leq (1-\frac 1 2 \cprobi)^{\log(\frac 1 \eta) / \log((1 - \frac 1 2 \cprobi)^{-1})} \\
      &= (1-\frac 1 2 \cprobi)^{\log_{(1 - \frac 1 2 \cprobi)}(\eta)}
      = \eta
    \end{align*}
    As such, $\Pr[A_{i+N} \text{ is a strict superset of } A_i ] \geq 1 - \eta$ since this is the complement event (by the loop invariant from \cref{claim:main-loop-invariant}).
  \end{subproof}
  We apply \cref{claim:main-probability-accumulation} with the choice of $\eta = p_{\ref{thm:single-recovery-main-reprise}} / (\dm - k - 1)$.
  By taking a union bound, we see that when $I \geq C_1(\dm-k-1) \lceil \log((\dm-k-1) / p_{\ref{thm:single-recovery-main-reprise}} ) \rceil$ with the choice of $C_1 = \frac 1 {\log((1-\frac 1 2 \cprobi)^{-1})}$, then with probability $1 - p_{\ref{thm:single-recovery-main-reprise}}$,  $\abs{A_{I+1}} \geq \abs{A_1} + {\dm - k - 1} = \dm - 1$ as desired.
  In particular, it suffices that $I \geq C_1 \dm \lceil \log(\dm / p_{\ref{thm:single-recovery-main-reprise}})\rceil$.
\end{proof}

\begin{thm}\label{thm:full-recovery-main-reprise}
  Suppose $\sigma \in (0,\, \frac 1 {6\sqrt {2\dn(1+2\delta)}} \tcompress^2]$,
  \begin{displaymath}
    \epsilon \leq C_0 \epsdiverge{\frac{\sigma}{\sqrt \dn}\left(\frac {\beta \gamma}{\alpha \delta \dm^\delta}\right)^{\frac 1 \gamma}\tcompress^2, [\dm]}\dn^{-\delta} \ ,
  \end{displaymath}
  $N_1 \geq 2\Nsc $,
  $N_2 \geq 2\Nsc + C_0\Nspread{\frac{\sigma}{\sqrt \dn}(\frac {\beta \gamma}{\alpha \delta \dm^\delta})^{\frac 1 \gamma}\tcompress^2}$,
  $p_{\ref{thm:full-recovery-main-reprise}} \in (0, 1)$,
  and $I \geq C_2 \dm \lceil \log(\dm / p_{\ref{thm:full-recovery-main-reprise}}) \rceil$.
  If we execute $\gvec \mu_1, \dotsc, \gvec \mu_{\hat \dm}\leftarrow \Call{RobustGI-Recovery}{\hat m}$ for some integer $\hat \dm \in [\dm, \dn]$,
  then $\gvec \mu_1, \dotsc, \gvec \mu_\dm$ forms a $4\sqrt{2}\delta \epsilon / \beta$-approximation to the hidden basis.
  More precisely, there exists a permutation $\pi$ of $[\dm]$ and signs $s_1, \dotsc, s_\dm \in \{+1, -1\}$ such that $\norm{ s_i \gvec \mu_i - \myZv_{\pi(i)} } \leq 4 \sqrt{2} \delta \epsilon / \beta$ for each $i \in [\dm]$.
\end{thm}
\begin{proof} %[\proofword\@of \cref{thm:robust-all-recovery-reprise}]
  We let $\gvec \mu_1, \dotsc, \gvec \mu_\dm$ denote the first $\dm$ approximate basis elements returned by \textsc{RobustGI-Recovery}.
  We proceed by induction on the following statement (with $k \in [\dm] \cup \{0\}$).  \newline \newline
  \noindent\textbf{Inductive Hypothesis:}
  With probability at least $1 - kp_{\ref{thm:full-recovery-main-reprise}} / \dm$,
  there exist sign values $s_1, \dotsc, s_k$ and a permutation $\pi_k$ of $[\dm]$ such that $\norm{s_i \gvec \mu_i - \myZv_{\pi_k(i)}}\leq 4 \sqrt{2} \delta \epsilon / \beta$ for each $i \leq k$.
  \newline\newline
  %
  The base case $k = 0$ holds trivially.
  Suppose that the inductive hypothesis holds for some $k = n$ with $n < \dm$.
  In order to apply \cref{thm:single-recovery-main-reprise}, we set $p_{\ref{thm:single-recovery-main-reprise}} = \frac 1 \dm p_{\ref{thm:full-recovery-main-reprise}}$.
  In order to apply \cref{thm:single-recovery-main-reprise},
  we require that $I \geq C_1 \dm \lceil \log(\dm^2 / p_{\ref{thm:full-recovery-main-reprise}}) \rceil$ (where $C_1$ is as in \cref{thm:single-recovery-main-reprise}), for which it suffices that $I \geq 2C_1 \dm \lceil \log(\dm / p_{\ref{thm:full-recovery-main-reprise}}) \rceil$.
  In particular, it suffices that $C_2 = 2C_1$.

  We now consider the case $k = n$, and
  we operate conditionally on the case that there exist sign values $s_1, \dotsc, s_n$ and a permutation $\pi_n$ of $[\dm]$ such that $\norm{s_i \gvec \mu_i - \myZv_{\pi_n(i)}}\leq 4 \sqrt{2} \delta \epsilon / \beta$ for each $i \leq n$.
  By \cref{thm:single-recovery-main-reprise}, with probability at least $1 - \frac 1 \dm p_{\ref{thm:full-recovery-main-reprise}}$ there exists $j \in [\dm] \setminus \{\pi_n(i) \suchthat i \in [n]\}$ and a sign $s$ such that $\norm{s\gvec \mu_{n+1} - \myZv_j} \leq 4 \sqrt{2} \delta \epsilon / \beta$.
  Defining $s_{n+1} := s$ and $\pi_{n+1}$ to be a permutation of $[\dm]$ such that $\pi_{n+1}(n+1) = j$ and $\pi_{n+1}(i) = \pi_n(i)$ for $i \leq n$ gives the result for $\gvec \mu_{n+1}$.
  Further, we see that the probability that the inductive hypothesis holds for $k = n + 1$ is lower bounded by $(1 - np_{\ref{thm:full-recovery-main-reprise}} / \dm)(1 - p_{\ref{thm:full-recovery-main-reprise}} / \dm) \geq 1 - (n+1)p_{\ref{thm:full-recovery-main-reprise}} / \dm$ as desired.

  Applying induction on $k$ completes the proof.
\end{proof}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> simplexframework - Copy/ica-analysis.tex <==
\section{A Provably Robust Algorithm for Independent Component Analysis}
\label{sec:robust-ICA}

In addition to being a very popular technique for blind source separation, Independent Component Analysis (ICA) has been of recent interest in the computer science theory community.
Frieze, et al.~\citep{FriezeJK96} gave an early analysis of ICA in the setting where the underlying source distributions are continuous uniform distributions. The analysis of this setting was simplified in a cryptographic context by~\citep{Nguyen2009}.
More recently, there have been a number of works which discuss provable ICA in the presence of additive Gaussian noise~\citep{Vempala2011,AroraGMS12,Belkin2012,DBLP:conf/stoc/GoyalVX14}. 

In this section, we
show how our {\sef} framework can be used to analyze ICA.
In so doing, we provide the first analysis of a general perturbed ICA model.
We assume throughout this section that $\vec X = A \vec S$ is an ICA model where realizations of $\vec X$ and $\vec S$ are both in $\R^\dn$ (i.e., we consider the fully determined setting in which the number of latent sources equals the ambient dimension of the space).
For a random variable $Y$, we denote its $r$\textsuperscript{th} moment $m_r(Y) := \E[Y^r]$ and its order $r$ cumulant by $\kappa_r(Y)$.
We make the following assumptions:
%\begin{enumerate}[label=B\arabic{enumi}., ref=B\arabic{enumi}, topsep=3pt,partopsep=0pt,itemsep=0pt,parsep=3pt]
\begin{assump}
  \label{ICA-A:first}
  \label{ICA-A:ambiguities}
  $\vec S$ has identity covariance.
\end{assump}
\begin{assump}
  \label{ICA-A:min-kappa4}
  For all $i \in [\dn]$, $\abs{\kappa_4(S_i)} > 0$
\end{assump}
\begin{assump}
  \label{ICA-A:max-m8}
  For all $i \in [\dn]$, $m_8(S_i) < \infty$.
\end{assump}
\begin{assump}
  \label{ICA-A:last} \label{ICA-A:A-orth} $A$ is an orthogonal matrix
  and $\vec S$ has $\vec 0$ mean.
\end{assump}
%\end{enumerate}

\Cref{ICA-A:ambiguities} is commonly used within the ICA literature in order to minimize the ambiguities of the ICA model.
\Cref{ICA-A:min-kappa4} is commonly made for cumulant-based ICA algorithms which are used in practice.
\Cref{ICA-A:max-m8} will play an important role in our error analysis for cumulant estimation.
We include \cref{ICA-A:A-orth} in order to simplify the exposition and more quickly highlight how our framework applies to ICA.
It is common in many ICA algorithms to preprocess the data by placing the data in isotropic position (this is typically referred to as whitening) so that it has $\vec 0$ mean and identity covariance.
After this preprocessing step, $A$ is of the desired form.
By including the final assumption, we remove the necessity of analyzing the whitening step and propagating the resulting error.
Our approach can be generalized to include an error analysis of the whitening step.

We first recall from the discussion on ICA in \cref{sec:example-befs} that the function $F: \sphere^{\dn - 1} \rightarrow \R$ defined by $F(\vec u) := \kappa_4( \ipCanonical{\vec u}{\vec X})$ is a basis encoding function with associated contrasts $g_i(x) := x^4 \kappa_4(S_i)$ (for $i \in [\dn]$) and hidden basis elements $\myZv_i := A_i$ (for $i \in [\dn]$).
We now see that this choice of $F$ is actually a robust {\sef}.

\begin{lem}\label{lem:cum4-BEF-robustness}
  Define $\kappa_{\min} := \min_{i \in [\dn]} \abs{\kappa_4(S_i)}$ and $\kappa_{\max} := \max_{i \in [\dn]}\abs{\kappa_4(S_i)}$.
  Let $F : \sphere^{\dn - 1} \rightarrow \R$ be defined by $F(\vec u) := \kappa_4(\ipCanonical{\vec u}{\vec X})$.
  Then, $F$ is a $(2\kappa_{\max}, 2\kappa_{\min}, 1, 1)$-robust {\sef}.
  % with associated contrasts $g_i(x) := x^4 \kappa_4(S_i)$ and hidden basis elements $\myZv_i := A_i$ (for $i \in [\dn]$).
\end{lem}
\begin{proof}
  Using the definition of $h_i$ from \cref{sec:extrema-structure}, we obtain for all $i \in [\dn]$ that $h_i(x) = g_i(\sign(x)\sqrt{\abs x}) = x^2 \kappa_4(S_i)$.
  Taking derivatives, we see that $h_i''(x) = 2 \kappa_4(S_i)$, and hence that $2 \kappa_{\min} \leq \abs {h_i''(x)} \leq 2 \kappa_{\max}$.
  Recalling \cref{defn:BEF-robust} with $(\alpha, \beta, \gamma, \delta) = (2\kappa_{\max}, 2\kappa_{\min}, 1, 1)$ completes the proof.
\end{proof}

We do not have direct access to $F$.
Instead, we will estimate $F$ from samples.
We note that for any $\vec u \in \sphere^{\dn-1}$, $\var(\ipCanonical{\vec u}{\vec X}) = 1$.
For a 0-mean random variable $Y$ with unit variance, the fourth cumulant is known to take on a very simple form:  $\kappa_4(Y) = m_4(Y) - 3$.
This provides a natural sample estimate for the fourth cumulant in our setting.
Given samples $y \ind 1, y \ind 2, \dotsc, y \ind N$ of a random variable $Y$, we will estimate $\kappa_4(Y)$ by $\hat \kappa_4(y \ind i) := \frac 1 N \sum_{i=1}^N (y \ind i) ^4 - 3$.

Let $p_{\vec Y}$ denote the probability density function of a random vector $\vec Y$.
In order to handle a perturbation away from the ICA model, we will consider metrics
of the form $\mu_k(\vec X, \vec Y) := \int_{t\in \R^{\dn}} \norm{\vec t}^8 \abs{p_{\vec X}(\vec t) - p_{\vec Y}(\vec t)} \mathrm d \vec t$ on the space of probability densities. \vnote{Can use $(1+\norm{t})^8$ rather than $\norm{t}^8$ in order to make it so that $\mu_r(\vec X, \vec Y) \leq \mu_s(\vec X, \vec Y)$ whenever $r \leq s$.}%
We will assume sample access to a random variable $\tvec X$ such that $\mu_8(\vec X, \tvec X)$ is sufficiently small (to be quantified later).
Given samples $\tvec x \ind 1, \tvec x \ind 2, \dotsc, \tvec x \ind N$ i.i.d.\ from $\tvec X$, we estimate $F$ by the function $\hat F(\vec u) := \frac 1 N \sum_{i=1}^N \ipCanonicalp{\vec u}{\tvec x\ind i}^4 - 3$.
The gradient of $\hat F$ is easily computed as $\nabla \hat F(\vec u) = \frac 4 N \sum_{i=1}^N \ipCanonicalp{\vec u}{\tvec x \ind i}^3 \tvec x \ind i $ and acts as an estimate of $\nabla F$.
% and $\HH \hat F(\vec u) = \frac {12} N \sum_{i = 1}^N \ipCanonicalp{\vec u}{\tvec x \ind i}^2 \tvec x \ind i \tvec x \ind i^T$.
As such, we have all of the information required to implement \textsc{RobustGI-Recovery} using $\pertgF:= \nabla \hat F$.

We now provide uniform bounds on the estimate errors for $\nabla F$ under this model.

\begin{lem}\label{lem:ICA-BEF-error-bounds}
  Fix $\delta > 0$ and $\eta > 0$.
  Let $M_8 := \max_{i \in [\dn]} m_8(S_i)$.
  Let $\tvec X$ be a random vector in $\R^\dn$ such that $\mu_8(\vec X, \tvec X)$ is finite.
  Suppose that $\tvec x \ind 1, \tvec x \ind 2, \dotsc, \tvec x \ind N$ are drawn i.i.d.\ from $\hat {\vec X}$ with $N \geq \frac{d^4[M_8 + \mu_8(\vec X, \tvec X)]}{\eta^2 \delta}$.
  If $\hat F(\vec u) := \frac 1 N \sum_{i=1}^\dn \ipCanonicalp{\vec u}{\tvec x\ind i}^4 - 3$ and $F(\vec u) := \kappa_4(\ipCanonical{\vec u}{\vec X})$,
  then with probability $1 - \delta$ the following bounds hold for all $\vec u \in \sphere^{\dn - 1}$: (1) $\abs{F(\vec u) - \hat F(\vec u)} \leq (\eta+\mu_4(\vec X, \tvec X))d^2$ and (2) $\norm{ \nabla F(\vec u) - \nabla \hat F(\vec u)} \leq 4(\eta + \mu_4(\vec X, \tvec X))\dn^2$. % and (3) $\norm{\HH F(\vec u) - \HH \hat F(\vec u)} \leq 12(\eta + \mu_4(\vec X, \tvec X)) \dn^2$.
\end{lem}
\begin{proof}
  In this proof, we proceed with the convention that we are indexing with respect to the hidden basis in which $\myZv_i := A_i$ for all $i \in [\dn]$.
  In particular, this implies $X_i = \ipCanonical{A_i}{\vec X} = S_i$.
  
  We use multi-index notation to compress our discussion as follows:
  $J \in [\dn]^k$ will denote a multi-index $J = (j_1, j_2, \dotsc, j_k)$ such that each $j_\ell \in [\dn]$.
  For a vector $\vec v$, $v_J$ denotes the product $\prod_{\ell = 1}^k v_{j_\ell}$.
  Our objective function $\hat F(\vec u)$ may be expanded as a polynomial of the $u_j$s as follows:
  \begin{align*}
    \hat F(\vec u) 
    &= \frac 1 N \sum_{i=1}^N \ipCanonicalp{\vec u}{\tvec x \ind i}^4 - 3
%    &= \frac 1 N \sum_{i=1}^N \sum_{j_1 = 1}^\dn \cdots \sum_{j_4 = 1}^\dn u_{j_1}u_{j_2}u_{j_3}u_{j_4} \hat x_{j_1} \ind i \hat x_{j_2} \ind i \hat x_{j_3} \ind i \hat x_{j_4} \ind i
    = \frac 1 N \sum_{i=1}^N \sum_{J \in [\dn]^4} u_J \hat x_J(i) - 3 \\
    &= \sum_{J \in [\dn]^4} u_J \biggr[\frac 1 N \sum_{i=1}^N \hat x_J \ind i\biggr] - 3 \ .
  \end{align*}
  By a similar argument, it can be shown that $F(\vec u) = \sum_{J \in [\dn]^4} u_J \E[X_J] - 3$.
  We obtain the error bound $\abs{\hat F(\vec u) - F(\vec u)} \leq \sum_{J \in [\dn]^4} u_J \abs{ \frac 1 N \sum_{i=1}^\dn \hat x_J(i) - \E[X_J] }$.
  Similarly, we can bound the error estimate for $\nabla F(\vec u)$: % and $\HH F(\vec u)$.
  \begin{align*}
    \norm{\nabla \hat F(\vec u) - \nabla F(\vec u)}
    &= 4 \sum_{J \in [\dn]^3} u_J \biggr\lVert\frac 1 N \sum_{i=1}^{N} \hat x_J \ind i \tvec x \ind i - \E[X_J \vec X]\biggr\rVert. % \\
    % \norm{\HH \hat F(\vec u) - \HH F(\vec u)}
    % &= 12 \sum_{J \in [\dn]^2} u_J \biggr\lVert \frac 1 N \sum_{i=1}^{N} \hat x_J \ind i \tvec x \ind i \tvec x \ind i ^T - \E[X_J \vec X \vec X^T] \biggr\rVert \ .
  \end{align*}
  With $J \in [\dn]^4$, we define $\varepsilon_J := \frac 1 N \sum_{i=1}^N \hat x_J(i) - \E[X_J]$ and $\varepsilon_{\max} := \max_{J \in [\dn]^4} \abs {\varepsilon_J}$.
  Using that each $\vec u$ is a unit vector, we see that $\abs{\sum_{J \in [\dn]^k} u_J} \leq \norm[1]{\vec u}^k \leq \dn^{k/2}$.
  Using the norm inequalities that for vector $\vec v \in \R^\dn$ and matrix $A \in \R^{\dn \times \dn}$, $\norm{\vec v} \leq  \max_{i \in [\dn]} \abs {v_i} \sqrt \dn$ and $\norm{A} \leq \max_{(i, j) \in [\dn]^2} \abs{a_{ij}} \dn$, we are able to obtain the following bounds for all $\vec u \in \sphere^{\dn - 1}$:  $\abs{\hat F(\vec u) - F(\vec u)} \leq \dn^2 \varepsilon_{\max}$ and $\norm{\nabla \hat F(\vec u) - \nabla F(\vec u)} \leq 4 \dn^2 \varepsilon_{\max}$. % , and $\norm{ \HH \hat F(\vec u) - \HH F(\vec u) } \leq 12 \dn^2 \varepsilon_{\max}$.
  All that remains is to bound $\varepsilon_{\max}$.
  To do so, we will bound each $\varepsilon_J$ using Chebyshev's inequality.
  
  For each $J \in [\dn]^4$, we obtain under the sampling process that
  \begin{align*}
    \var\biggr(\frac 1 N \sum_{i = 1}^{N}\hat x_J \ind i\biggr)
    &= \frac 1 {N^2} \var\biggr(\sum_{i = 1}^{N}\hat x_J \ind i\biggr)
    = \frac 1 {N} \var( \hat X_J )
    \leq \frac 1 N \E[(\hat X_J)^2] \\
    &\leq \frac 1 N \E[\hat X_{j_1}^4 \hat X_{j_2}^4]^{\frac 1 2}\E[\hat X_{j_3}^4 \hat X_{j_4}^4]^{\frac 1 2}
    \leq \frac 1 N \biggr({\prod_{\ell=1}^{4}}\E[\hat X_{j_\ell}^8]\biggr)^{\frac 1 4}
    \leq \frac 1 N \max_{\ell \in [\dn]} \E[\hat X_\ell^8]
  \end{align*}
  where the first equality uses that variance is order-2 homogeneous\index{homogeneity}, the second equality uses independence, the first inequality follows from the formula $\var(\hat X_J) = \E[(\hat X_J)^2] - \E[\hat X_J]^2$, and
  the second and third inequalities use the Cauchy-Schwartz inequality.
  We bound $\max_{\ell \in [\dn]} \E[\hat X_\ell^8]$ as:
  \begin{align*}
    \E[\hat X_\ell^8]
    &= \int_{\vec t \in \R^\dn} t_{\ell}^8 p_{\tvec X}(\vec t) \mathrm d \vec t \\
    &= \int_{\vec t \in \R^\dn} t_{\ell}^8 p_{\vec X}(\vec t) \mathrm d \vec t +
      \int_{\vec t \in \R^\dn} t_{\ell}^8 (p_{\tvec X}(\vec t) - p_{\vec X}(\vec t)) \mathrm d \vec t
    \leq M_8 + \mu_8(\vec X, \tvec X) \ .
  \end{align*}
  Thus, $\var\bigr(\frac 1 N \sum_{i = 1}^{N}\hat x_J \ind i\bigr) \leq \frac 1 N (M_8 + \mu_8(\vec X, \tvec X))$.

  Chebyshev's inequality states that for any random variable $Y$ and any $k > 0$, $\Pr[\abs{ Y - \E[Y] } \geq k \sqrt{\var(Y)}] \leq \frac 1 {k^2}$.
  We fix any $J \in [\dn]^4$, choose $Y = \frac 1 N \sum_{i = 1}^N \hat x_J(i)$, and choose $k = \frac{\dn^2}{\sqrt \delta}$.
  We obtain that with probability at least $1 - \delta / {\dn^4}$,
  \begin{equation}\label{eq:Chebyshev-bound}
    \Abs{\frac 1 N \sum_{i=1}^N \hat x_J(i) - \E[\hat X_J]} < \frac{\dn^2}{\sqrt \delta} \sqrt{\frac 1 N (M_8 + \mu_8(\vec X, \tvec X))} \leq \eta
  \end{equation}
  by our given bound on $N$.
  Taking a union bound, then with probability at least $1 - \delta$, the bound in \cref{eq:Chebyshev-bound} holds for all $J \in [\dn]^4$.

  We then obtain the following bound on each $\varepsilon_{J}$ for each $J \in [\dn]^4$ (with probability at least $1-\delta$):
  \begin{align*}
    \abs{\varepsilon_{J}}
    &= \Abs{\frac 1 N \sum_{i=1}^N \hat x_J(i) - \E[X_J]}
    \leq \eta + \abs{\E[\hat X_J] - \E[X_J]} \\
    &= \eta + \Abs{\int_{\vec t \in \R^4} t_J[p_{\tvec X}(\vec t) - p_{\vec X}(\vec t)] \mathrm d \vec t }
    \leq \eta + \mu_4(\tvec X, \vec X) \ .
  \end{align*}
  To obtain the result, we use $\varepsilon_{\max} \leq \eta + \mu_4(\tvec X, \vec X)$ in our previously derived uniform bounds over all $\vec u \in \sphere^{\dn-1}$ of $\abs{\hat F(\vec u) - F(\vec u)} \leq \dn^2 \varepsilon_{\max}$ and $\norm{\nabla \hat F(\vec u) - \nabla F(\vec u)} \leq 4 \dn^2 \varepsilon_{\max}$. % and $\norm{ \HH \hat F(\vec u) - \HH F(\vec u) } \leq 12 \dn^2 \varepsilon_{\max}$.
\end{proof}

We now state our result for ICA.
We assume $\vec X = A \vec S$ is an ICA model satisfying \crefrange{ICA-A:ambiguities}{ICA-A:A-orth} with associated constants $\kappa_{\min} := \min_{i \in [\dn]} \abs{\kappa_4(S_i)}$, $\kappa_{\max} := \max_{i \in [\dn]} \abs{\kappa_4(S_i)}$, and $M_8 := \max_{i \in [\dn]} m_8(S_i)$.
We assume $\tvec X$ is a perturbed ICA model, and we approximate the {\sef} $F(\ipCanonical{\vec u}{\vec X}) := \kappa_4(\ipCanonical{\vec u}{\vec X})$ from an i.i.d.\@ sample $\tvec x(1), \dotsc, \tvec x(\NN)$ of $\tvec X$.
That is, we define $\hat F(\vec u) := \frac 1 \NN \sum_{i=1}^\dn \ipCanonicalp{\vec u}{\tvec x \ind i}^4 - 3$ and compute its gradient as $\nabla \hat F(\vec u) := \frac 4 \NN \sum_{i=1}^\dn \ipCanonicalp{\vec u}{\tvec x \ind i}^3\tvec x \ind i$.
% $\HH \hat F(\vec u) := \frac {12} \NN \sum_{i=1}^\dn \ipCanonicalp{\vec u}{\tvec x \ind i}^2\tvec x \ind i \tvec x \ind i ^T$.
We further assume that we are working in a computation model which can perform the following operations in $O(\dn)$ time:  Inner products in $\R^\dn$, scalar operations including basic arithmetic operations, trigonometric functions, square roots, and branches on conditionals.
In the following, $C_1, C_2, \dotsc$ are positive universal constants.

\begin{thm}\label{thm:ICA-result-reprise}
Fix $\delta > 0$ and $\varepsilon > 0$.
Suppose  $\sigma \leq \frac{C_0}{\dn^2}\frac{\kappa_{\min}}{\kappa_{\max}}$,
$\varepsilon \leq C_1 \sigma \big( \frac{\kappa_{\min}}{\kappa_{\max}} \big)^{9/2}\dn^{-6}$, 
$\mu_4(\tvec X, \vec X) \leq C_2 \frac{\kappa_{\min}}{d^2}\varepsilon$, and
$\NN \geq \frac{C_3 \dn^8[M_8 + \mu_8(\tvec X, \vec X)]}{\kappa_{\min}^2 \varepsilon^2 \delta}$.
 Suppose we execute $\hat A_1, \dotsc, \hat A_\dn \leftarrow \textsc{RobustGI-Recovery}(\dn, \sigma, \nabla \hat F, N_1, N_2, I)$, where  
 $N_1 \geq C_4 \big\lceil \log_2(\log_2(\frac{1}{\varepsilon}))\big\rceil$, 
 $N_2 \geq C_5 \big\lceil \frac {\dn^{2.5}}{\sigma} \big(\frac {\kappa_{\max}}{\kappa_{\min}}\big)^3 \log(\dn \cdot \frac{\kappa_{\max} }{\kappa_{\min}}) \big\rceil + \big\lceil \log_2(\log_2(\frac{1}{\varepsilon}))\big\rceil$,
 and $I \geq C_6 \dn \log (\dn / \delta)$.
 Then, with probability at least $1 - \delta$,
 $\hat A_1, \dotsc, \hat A_\dn$ is a $\varepsilon$-recovery of $A_1, \dotsc A_\dn$.
 % there exists a permutation $\pi$ of $[\dn]$ and sign values $s_i \in \{ \pm 1 \}$ such that $\norm{\hat A_i - s_i A_{\pi(i)}} \leq \varepsilon$ for all $i \in [\dn]$.
 \textsc{RobustGI-Recovery} recovers such $\hat A_i$s in $C_7 \NN[\dn^4 + \dn^2 N_1 + \dn^2 I N_2]$ time.
\end{thm}
% \vnote{Note on constant values:  $C = \frac{\sqrt 2}{80 \sqrt 3 \times 16^{5/2}} = \frac{\sqrt 2}{81920 \sqrt 3}$}
\begin{proof}
  % We first wish to show that with probability at least $1-\delta$ over the sampling process of $\hat {\vec X}$, $\hat F$ is a $\frac{\kappa_{\min}}{2\sqrt 2}\varepsilon$-approximation to $F$.
  By \cref{lem:ICA-BEF-error-bounds} with the choice of $\eta = O(\frac{\kappa_{\min}}{\dn^2}\varepsilon)$, we obtain that with probability at least $1 - \frac \delta 2$, 
  \begin{align*}
    \norm{\nabla F(\vec u) - \nabla \hat F(\vec u)}
    &\leq 4(\eta + \mu_4(\vec X, \hat {\vec X}))d^2
    \leq O\Big(\frac{\kappa_{\min}}{\dn^2}\varepsilon + \frac{\kappa_{\min}}{\dn^2}\varepsilon\Big)d^2
    = O(\kappa_{\min} \varepsilon), 
  \end{align*}
  for all $\vec u \in \sphere^{\dn - 1}$.
  In particular, $\hat F$ is an $O(\kappa_{\min}\varepsilon)$-approximation to $F$.

  We recall from \cref{lem:cum4-BEF-robustness} that $F$ is an $(2\kappa_{\max}, 2\kappa_{\min}, 1, 1)$-robust {\sef}.
  As such, we may apply \cref{cor:robust-all-recovery-error-version} to obtain that $\textsc{RobustGI-Recovery}$ returns vectors $\hat A_1, \dotsc, \hat A_\dn$ of the desired form.
  Finally, we note that within our computational model for this theorem, computations of $\nabla \hat F(\vec u)$ take $O(\NN \dn)$ time.
  Thus, applying \cref{thm:running-time} with $\hat \dm = \dn$ yields the claimed time bound.
\end{proof}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> simplexframework - Copy/macros.tex <==
\usepackage{amsmath}

\newcommand{\abs}[1]{{\ensuremath | #1 |}}
\newcommand{\Abs}[1]{\ensuremath \left| #1 \right|}
\newcommand{\restr}[1]{\ensuremath \vert_{#1}}

% \def\eps{\epsilon}
% \renewcommand{\epsilon}{\varepsilon}

\newcommand{\ip}[2]{\ensuremath{\langle #1,\, #2 \rangle}}
\newcommand{\Ip}[2]{\ensuremath{\left\langle #1,\, #2 \right\rangle}}
\newcommand{\nCr}[2]{{{#1}\choose{#2}}}
\newcommand{\norm}[2][]{\ensuremath{\lVert #2 \rVert_{#1}}}
\newcommand{\Norm}[2][]{\ensuremath{\left\lVert #2 \right\rVert_{#1}}}
\newcommand{\norms}[1]{{\lVert#1\rVert}^2}
\newcommand{\sym}{\ensuremath{\mathrm{sym}}}
\newcommand{\rw}{\ensuremath{\mathrm{rw}}}

% Math blackboard bold characters
\newcommand{\C}{\mathbb{C}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Z}{\mathbb{Z}}
\renewcommand{\Pr}{\mathbb{P}}

% mathcal letters
\newcommand{\CC}{\mathcal{C}}
\newcommand{\DD}{\mathcal{D}}
%\newcommand{\GG}{\mathcal{G}}
\newcommand{\GG}{G}
\newcommand{\RR}{\mathcal{R}}
\newcommand{\HH}{\mathcal{H}}
\newcommand{\LL}{\mathcal{L}}
\newcommand{\MM}{\mathcal{M}}
\newcommand{\NN}{\mathcal{N}}
\renewcommand{\SS}{\mathcal{S}}
\newcommand{\XX}{\mathcal{X}}

% boldface for Greek characters
\newcommand{\gvec}[1]{\ensuremath{\boldsymbol{#1}}}

% Math operators
\DeclareMathOperator{\arc}{arc}
\DeclareMathOperator{\argmax}{arg\ max}
\DeclareMathOperator{\argmin}{arg\ min}
\DeclareMathOperator{\cov}{cov}
\DeclareMathOperator{\conv}{conv}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\poly}{poly}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\spn}{span}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\var}{var}

\newcommand{\grad}{\nabla}

% Vector style
\renewcommand{\vec}[1]{\ensuremath{\mathbf{#1}}}

% Specialized dots and inner products
\newcommand*{\Cdot}[1][1.25]{%
  \mathpalette{\CdotAux{#1}}\bullet%
}
\newdimen\CdotAxis
\newcommand*{\CdotAux}[3]{%
  {%
    \settoheight\CdotAxis{$#2\vcenter{}$}%
    \sbox0{%
      \raisebox\CdotAxis{%
        \scalebox{#1}{%
          \raisebox{-\CdotAxis}{%
            $\mathsurround=0pt #2#3$%
          }%
        }%
      }%
    }%
    % Remove depth that arises from scaling.
    \dp0=0pt %
    % Decrease scaled height.
    \sbox2{$#2\bullet$}%
    \ifdim\ht2<\ht0 %
      \ht0=\ht2 %
    \fi
    % Use the same width as the original \cdot.
    \sbox2{$\mathsurround=0pt #2#3$}%
    \hbox to \wd2{\hss\usebox{0}\hss}%
  }%
}

\newcommand{\argdot}{\Cdot[.8]}
\newcommand{\vecdot}{\Cdot[0.5]}
\newcommand{\ipCanonical}[2]{\ip{#1}{#2}}
\newcommand{\ipCanonicalp}[2]{\ip{#1}{#2}}


%%% Local Variables: 
%%% mode: plain-tex
%%% TeX-master: "main"
%%% End: 


==> simplexframework - Copy/matrix-tie-in.tex <==
The main intuition for why the gradient iteration converges to a hidden basis direction comes from two key concepts (working in $\porth^{\dn - 1}$ with a {\psef}):
\begin{enumerate}
\item\label{item:expand-all-explanation-ordering} For each iteration there is an implicit ordering $i \prec_n j$ if $h_i'(u_i(n)) < h_j'(u_j(n))$ such that the ratio
\begin{equation}\label{eq:power-iteration-expand-demo}
  \frac{u_{i}(n+1)}{u_{j}(n+1)} 
  = \frac{\GG_{i}(\vec u(n))}{\GG_{j}(\vec u(n))}
  = \frac{h_{i}'(u_{i}(n)^2)u_{i}(n)}{h_{j}'(u_{j}(n)^2)u_{j}(n)}
\end{equation}
expands from $u_i(n)/u_j(n)$ if and only if $i \succ_n j$.
\item The function $n \mapsto \max_i h_i'(u_i(n)^2)$ is non-decreasing and $n \mapsto \min_i h_i'(u_i(n))$ is non-increasing\footnote{See \cref{lem:increasing-maxhi'}.  We don't actually prove that $n \mapsto \min_i \abs{h_i'(u_i(n))}$ is non-decreasing as we don't end up needing this fact, but the proof closely resembles that of \cref{lem:increasing-maxhi'} with the roles of $\max$ and $\min$ swapped and the also ordering role of $<$ reversed to $>$.}.  As such, the maximal expansionary effect seen between coordinates in part \ref{item:expand-all-explanation-ordering} can only increase with each iteration.
\end{enumerate}
These two ideas provide intuition for why the gradient iteration should drive coordinates to zero until a hidden basis direction $\myZv_i$ is recovered.
By repeated use of the gradient iteration, we expect $u_j(n) \rightarrow 0$ for some $j$ in order to support the expansion of the fraction $u_i(n) / u_j(n)$.

Interestingly, these two observations hold even if \cref{assumpt:convex} is relaxed to allow functions $g_i$ where $g_i(\sqrt{x})$ is convex but not \textit{strictly} convex, and if \cref{assumpt:deriv0} is omitted\footnote{In particular, the proof of \cref{lem:increasing-maxhi'} holds under this relaxation.}.
We conjecture that guarantees similar to those of matrix eigenvector recovery via the power iteration are achievable for more generic odeco functions satisfying such relaxed assumptions.
However, formulating precise statements for when odeco basis recovery works in such relaxed conditions is beyond the scope of this paper.

Where the analysis of odeco functions is more challenging in our
setting than in the matrix and tensor settings is that the ordering
$\prec_n$ changes with $n$.
In the matrix setting, each $h_i'(u_i(n)^2) = \lambda_i$ is simply the
$i$\textsuperscript{th} eigenvalue making the ordering $\prec_n$ fixed
for all $n$.
If $\lambda_1$ corresponds to a maximal eigenvalue with multiplicity 1
and $u_i(0) \neq 0$, then it is not difficult to see that
$\abs{u_1(n)}/ \abs{u_i(n)} \rightarrow \infty$ as $n \rightarrow
\infty$ under the power iteration by repeated application of
\eqref{eq:power-iteration-expand-demo} for all $i \neq 1$; indeed,
this is a standard proof of convergence to the top eigenvector in the
matrix setting.
In the odeco function setting $\prec_n$ is not fixed.
Because we cannot directly chain together applications of
\eqref{eq:power-iteration-expand-demo}, we do the following.
\begin{enumerate}
\item In \cref{sec:gi-divergence-criteria} we rely on an interplay between the coordinates of $\vec u(n)$ in the $\prec_n$ ordering and the coordinate values of a fixed point $\vec v$ of $\GG$ to create a globally expanding ratio which forces a coordinate of $\vec u(n)$ to zero.
\item In \cref{sec:ae-attraction} we use stable-unstable manifold theory to show $\{\vec u(n)\}_{n=0}^\infty$ converges to a hidden basis direction $\myZv_i$ given almost any starting point. 
\end{enumerate}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> simplexframework - Copy/notation_chart.tex <==
\begin{longtable}{|c|X|}\hline
  $\grad$ & The gradient operator. \\
  $\HH$ & The Hessian operator. \\
  $\partial_i$ & The derivative operator with respect to the $i$\textsuperscript{th} basis element of the space, i.e.\@ $\myZv_i$. \\
  % When working in $[\dn]$, this is the derivative with respect to the direction $\myZv_i$. \\
  $\Jacob f_{\vec x}$ & The Jacobian of $f$ evaluated at $\vec x$. \\
  $A \disunion B$ & The union operation between two disjoint sets $A$ and $B$. \\
  $f \restr D$ & The restriction of $f$ to the domain $D$. \\
  $[\vec u]$ & The equivalence class $\{ \vec v \suchthat \vec v \sim \vec u\}$. \\
  % $\phi$ & The map from $S^{\dn - 1} / {\sim}$ to $\porth^{\dn - 1}$ given by $\phi_i([\vec u]) = \abs{u_i}$.\\
  % $\mu$ & The distance metric on $S^{\dn-1}/\sim$ defined by $\mu([\vec u], [\vec v]) := \norm{\phi(\vec u) - \phi(\vec v)}$. \\
  $[k]$ & The set $\{1, 2, \dotsc, k\}$. \\
  $\lceil \bullet \rceil$ & This is the ceiling operator, i.e.\@ $\lceil x \rceil$ is the least integer which is greater than or equal to $x$. \\
  $\abs \bullet$ & The modulus or absolute value operation. \\
  $\norm \bullet$ & The standard Euclidean 2-norm. \\
  $\ip \bullet \bullet$ & The standard Euclidean inner product, i.e., the dot product. \\
  % $A$ & The matrix $A$. \\
  % $a_{ij}$ & The entry contained in the $i$\textsuperscript{th} row and $j$\textsuperscript{th} column of $A$. \\
  % $B(\vec x, r)$ & The open ball centered at $\vec x$ with radius $r$. \\
  $\overline{B(\vec x, r)}$ & The closed ball centered at $\vec x$ with radius $r$. \\
  $\indicator{E}$ & The indicator function of the event $E$. \\
  $\dn$ & Dimensionality of the ambient space. \\
  $\myZv_i$ & The vectors $\myZv_1, \dotsc, \myZv_\dm$ are the hidden basis elements encoded within {\ansef}.  The vectors $\myZv_{\dm+1},\dotsc, \myZv_{\dn}$ are chosen arbitrarily in order to make $\myZv_1, \dotsc, \myZv_\dn$ an orthonormal basis of $\R^\dn$. \\
  $\E$ & The expectation operator for random variables. \\
  $\fg$ & {\Ansef} with expanded form $\fg(\vec u) = \sum_{i=1}^\dm \alpha_i g(\beta_i u_i)$, defined on page~\pageref{defn:sef}. \\
  $\bar F$ & The {\psef} associated with {\sef} $\fg$. \\
  $\GG$ & The gradient iteration functions associated with {\ansef} $\fg$. \\
  $\Id$ & The identity matrix. \\
  $\dm$ & Number of distinguished hidden basis vectors $\myZv_1, \dotsc, \myZv_\dm$.  Note that $\dm \leq \dn$. \\
  $\Pmap_{\SS}$ & The projection matrix $\sum_{i \in \SS} \myZv_i\myZv_i^T$. \\  
  % $\pmap_{\vec v}$ & The local coordinate map onto the projective space of the sphere:  $\pmap_{\vec v} : S^+_{\vec v} \rightarrow T_{\vec v}S^{\dn - 1}$ defined as $\pmap_{\vec v}(\vec u) := \frac{\vec u}{\ip{\vec u}{\vec v}}$.\\
  $\porth^{\dn-1}$ & The all positive orthant of $S^{\dn - 1}$:  $\{\vec u \in S^{\dn - 1} \suchthat u_i \geq 0 \text{ for all } i \in [\dn] \}$. \\
  $\orthsymb_{\vec v}^{\dn-1}$ & It is assumed that $\vec v \in \R^\dn$ is a vector of signs ($v_i \in \{+1, -1\}$ for all $i \in [\dn]$).
  Then, $\orthsymb_{\vec v}^{\dn-1} := \{\vec u \in S^{\dn - 1} \suchthat v_iu_i \geq 0 \}$ is the orthant of $S^{\dn - 1}$ containing $\vec v$. \\
  % $\vec p_i$ & A basis vector of the tangent space $T_{\vec v}S^{\dn -1}$. \\
  $S^{\dn - 1}$ & The unit sphere in $\R^\dn$:  $\{\vec u \in \R^\dn \suchthat \norm {\vec u} = 1\}$. \\
  $\compl \SS$ & The complement of $\SS$, typically $[\dn] \setminus \SS$. \\
  % $S^+_{\vec v}$ & The hemisphere $\{\vec u \suchthat \norm{\vec u} = 1 \text{ and } \ip{\vec u}{\vec v} > 0\}$. \\
  $\sign(\bullet)$ & The sign indicator on $\R$ defined by $\sign(x) :=
  \begin{cases}
    x/\abs{x} & \text{if $x \neq 0$} \\
    0 & \text{if $x = 0$} \\
  \end{cases}
$ . \\
  $\sim$ & The equivalence relation defined on $S^{\dn - 1}$ given by $\vec u \sim \vec v$ if for each $i \in [\dn]$, $\abs{u_i} = \abs{v_i}$. \\
  % $T_{\vec v} M$ & Tangent space of a manifold $M$ at the point $\vec v$. \\
  % $\vec v$ & A vector $\vec v$. \\
  % $v_i$ & The $i$\textsuperscript{th} element of $\vec v$.
  %        When $\vec v \in \R^\dn$, indexing is done with respect to the hidden basis $\myZv_1, \dotsc, \myZv_\dn$.
  %        In this case, the $i$\textsuperscript{th} element is $v_i := \ip{\vec v}{\myZv_i}$. \\
  $\Pr$ & The probability operator for random events. \\\
  $T_{\vec v} S^{\dn - 1}$ & The tangent space of $S^{\dn - 1}$ at $\vec v$, i.e.\@ $T_{\vec v} S^{\dn - 1} = \vec v^\perp$. \\
  $\vec v \elpow r$ & Vector $\vec v$ taken to the element-wise exponent of $r$, i.e., $(\vec v \elpow r)_i = v_i^r$.\\
  $\vol_{k-1}$ & The canonical volume measure on $S^{k-1}$.  When $k = \dn$, the subscript is often suppressed. \\ \hline
\end{longtable}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> simplexframework - Copy/optima-structure.tex <==
% At its most basic level, the proposed {\sef} primitive is of interest because the problem of learning a hidden basis $\myZv_1, \dotsc, \myZv_\dm$ in our space simplifies into a simple optimization problem, namely recovering the local maxima of $\abs \fg$.
% This is due to \cref{thm:gen-simplex-optima} which we prove in this section.

% Throughout this section, we will assume unless otherwise stated that $F$ is {\ansef} with associated tuples $\{(\sigma_{i+}, \sigma_{i-}, g_i, \myZv_i) \suchthat i \in [\dm]\}$.
The optima structure of $\fg$ relies on the hidden convexity implied by \cref{assumpt:convex}.
To capture  this structure, we define $h_i : [-1, 1] \rightarrow \R$ as $h_i(x) := g_i(\sign(x) \sqrt{\abs x})$ for $i \in [\dm]$ and $h_i := 0$ for $i \in [\dn] \setminus [\dm]$.
Thus,
\begin{equation}
  \label{eq:fg-via-his}
  \fg(\vec u) % = \sum_{i=1}^\dn h_i(\sign(u_i) u_i^2) 
    = \sum_{i=1}^\dm h_i(\sign(u_i) u_i^2) \ .
\end{equation}
These $h_i$ functions capture the convexity from \cref{assumpt:convex}.
Indeed, the functions $h_i$ have the following properties:

\begin{lem} \label{lem:h-props}
The following hold for all $i \in [\dm]$:
  \begin{compactenum}
  \item \label{lem:h-props:hi-convex} The magnitude function $\abs{h_i(t)}$ is strictly convex. 
  \item \label{lem:h-props:hi-deriv0} $h_i'(0) = 0$.
  \item \label{lem:h-props:hi-continuous} $h_i$ is continuously differentiable.
  \item \label{lem:h-props:hi-increase} 
    The derivative's magnitude function $\abs{h_i'(t)}$ is strictly increasing as a function of $\abs t$.
    In particular, $\abs{h_i'(t)} > 0$ for all $t \neq 0$.
  \item\label{lem:h-props:sign} Fix $I$ to be one of the intervals $(0, 1]$ or $[-1, 0)$.
    If $h_i$ is strictly convex on $I$, then $\sign(t)h_i'(t) > 0$ for all $t \in I$, and otherwise $\sign(t)h_i'(t) < 0$ for all $t \in I$.
  \end{compactenum}
\end{lem}
\begin{proof}
  We first show parts~\ref{lem:h-props:hi-deriv0} and \ref{lem:h-props:hi-continuous}.
  We compute the derivative of $h_i$ to see
  \begin{displaymath}
    h_i'(x) =
    \begin{cases}
      \frac 1 2 g_i'(\sign(x)\sqrt {\abs x} )/\sqrt {\abs x} & \text{if } x \neq 0 \\
      0 & \text{if } x = 0
    \end{cases}    
  \end{displaymath}
  where the derivative at the origin is due to \cref{assumpt:gsymmetries,assumpt:deriv0}.
  Since the derivative $h_i'(t)$ exists for all $t$, and since one of $\pm h_i$ is convex on either of the intervals $[0, 1]$ and $[-1, 0]$, it follows that $h_i'$ is continuous \citep[Corollary 4.2.3]{hiriart1996convex}.

  To see part~\ref{lem:h-props:hi-increase}, we note that $h_i'(0) = 0$ and apply \cref{assumpt:convex} to see that $h_i'$ is strictly monotonic on $[0, 1]$.
  As such, $\abs{h_i'(t)}$ is strictly increasing on $[0, 1]$.
  The symmetries of \cref{assumpt:gsymmetries} imply that $\abs{h_i'(t)}$ is strictly increasing more generally as a function of $\abs{t}$.

  To see part~\ref{lem:h-props:sign}, we note that $h_i'(t) = h_i'(0) + \int_0^t h_i''(x) \, dx = \int_0^t h_i''(x) \, dx$.
  Then, we use \cref{assumpt:convex} to obtain the stated correspondence between $\sign(h_i''(x))$ (which is +1 on $I$ if $h_i$ is convex and $-1$ otherwise) and $\sign(h_i'(t))$.

  To see that $\abs{h_i}$ is strictly convex, it suffices to use that $\abs{h_i}$ is continuously differentiable and to show that $\frac d {dt}\abs{h_i(t)}$ is strictly increasing.
  Note that $\frac d {dt}\abs{h_i(t)} = \sign(h_i(t))h_i'(t)$, and also that $\sign(h_i(t)) = \sign(\int_0^t h_i'(t)) = \sign(t h_i'(t))$ by part~\ref{lem:h-props:sign}.
  It follows that $\sign(\frac d {d t} \abs{h_i(t)}) = \sign(t)$.
  Taking this sign into account, part~\ref{lem:h-props:hi-increase} implies part~\ref{lem:h-props:hi-convex}.
\end{proof}


% \begin{lem} \label{lem:h-props}
% Let $\sigma_{i+}=1$ if $h_i$ is convex on $[0,1]$, $\sigma_{i+}=-1$ otherwise. 
% Let $\sigma_{i-}=1$ if $h_i$ is convex on $[-1,0]$, $\sigma_{i-}=-1$ otherwise.
% Let $I_+ = [0, 1]$ and let $I_- = [-1, 0]$.
% With $s \in \{+, -\}$ a symbol, the following hold for all $i \in [\dm]$:
%   \begin{compactenum}
%   \item \label{lem:h-props:hi-convex} The function $\sigma_{is} h_i$ is strictly convex on the domain $I_s$. 
%   \item \label{lem:h-props:hi-deriv0} $h_i'(0) = 0$.
%   \item \label{lem:h-props:hi-continuous} $h_i$ is continuously differentiable.
%   \item \label{lem:h-props:hi-increase} 
%     The derivative function $\sigma_{is} h_i'$ is strictly increasing on $I_s$.
%     As such, $s\sigma_{is} h_i'(x) > 0$ for all $x \in I_s \setminus \{0\}$.
%   \end{compactenum}
% \end{lem}
% \begin{vlong}
% \begin{proof}
%   That $\sigma_{is} h_i$ is strictly convex follows directly from \cref{assumpt:convex} when $s$ is $+$ and from \cref{assumpt:gsymmetries,assumpt:convex} when $s$ is $-$.
%   That $h_i'(0) = 0$ is an implication of \cref{assumpt:deriv0}.
%   That $h_i$ is continuously differentiable follows from the fact that 
%   \begin{displaymath}
%     h_i'(x) =
%     \begin{cases}
%       \frac 1 2 g_i'(\sign(x)\sqrt {\abs x} )/\sqrt {\abs x} & \text{if } x \neq 0 \\
%       0 & \text{if } x = 0
%     \end{cases}    
%   \end{displaymath}
%   exists everywhere, and is thus continuous due to the convexity of $\sigma_{is} h_i$ \citep[see][Corollary 4.2.3]{hiriart1996convex}.
  
%   Part~\ref{lem:h-props:hi-increase} can be seen using properties of strictly convex functions.
%   % Let $D_+$ denote the right derivative function.
%   % By strict convexity, $D_+ (\sigma_{is} h_i)$ is a strictly increasing functions on $I_s$. 
%   Since $\sigma_{is} h_i$ is differentiable and strictly convex on $I_s$, it follows that $\sigma_{is} h_i'$ is strictly increasing on $I_s$.
%   Since $\sigma_{is} h_i'(0) = 0$, we obtain in particular that $s \sigma_{is} h_i'(x) > 0$ for all $x \in I_s \setminus \{0\}$.
%   % $\sigma_{is} h_i'(x)$ and $D_+ (\sigma_{is} h_i)(x)$ coincide for each $x \in I_s$.
%   % As such, $\sigma_{is} h_i'$ is strictly increasing on $I_s$.
%   % \vnote{This should probably include a citation.}
%   % We refer the reader to~\cite[Remark ]{hiriart1996convex} for details.
% \end{proof}
%\end{vlong}

In order to avoid dealing with unnecessary sign values, we restrict ourselves to analyzing the optima structure of $\abs{\fg}$ over the domain $\porth^{\dn - 1}$ (the all positive orthant of the sphere).
Due to the symmetries of the of the problem (\cref{assumpt:gsymmetries}), it is actually sufficient to analyze the maxima structure of $\abs F$ on $\porth^{\dn - 1}$ in order to fully characterize the maxima of $\abs F$ on the entire sphere $S^{\dn - 1}$.

% We demonstrate that this can be done without loss of generality using \cref{lem:orth-transform} below.
% We identify each orthant by a sign vector $\vec v$ where each $v_i \in \{+1, -1\}$, and in particular we define $\orthsymb_{\vec v} := \{ \vec u \in S^{\dn - 1} \suchthat v_iu_i \ge 0 \text{ for each } i \in [\dn]\}$ as the orthant of $S^{\dn - 1}$ containing $\vec v$.
% % Then, we have the following result:
% \begin{lem}\label{lem:orth-transform}
%   Let $F$ be {\ansef} with hidden basis $\myZv_1, \dotsc, \myZv_\dn$, and
%   let $\vec v = \sum_{i=1}^\dn s_i\myZv_i$ for sign values $s_i \in \{\pm 1\}$.
%   Define an isometry $\psi : S^{\dn - 1} \rightarrow S^{\dn - 1}$ by $\psi_i(\vec u) := s_i u_i$.
%   Then the function $\tilde F := \fg \circ \psi$ is {\ansef}.
%   % In particular, $\tilde F\restr{\porth^{\dn-1}}$ is the pullback of $F\restr{\orthsymb_{\vec v}^{\dn-1}}$ with respect to $\psi$. 
% \end{lem}
% \begin{vlong}
% \begin{proof}
%   To construct $\tilde F = \sum_{i=1}^\dm \tilde g_i(\ip{\vec u}{\tilde \myZv_i})$, we set $\tilde \myZv_i = s_i \myZv_i$ and $\tilde g_i = g_i$ for each $i \in [\dm]$.
%   By construction, $\tilde F$ is {\ansef}.
%   Further, for any $\vec u \in S^{\dn - 1}$ we have that 
%   \begin{displaymath}
%     \fg \circ \psi(\vec u) = \sum_{i=1}^\dm g_i(s_i u_i)
%     = \sum_{i=1}^\dm g_i( \ip{\vec u}{\tilde \myZv_i} )
%     = \tilde F(\vec u) \ . \qedhere
%   \end{displaymath}
% \end{proof}
% \end{vlong}
% \vskip-7pt
% In essence, \cref{lem:orth-transform} allows us to relabel any orthant $Q_{\vec v}$ as being the all positive orthant.
% In \cref{lem:orth-transform}, $\psi\restr{\porth^{\dn - 1}} : \porth^{\dn - 1} \rightarrow \orthsymb_{\vec v}$ is a diffeomorphism achieved by reflecting appropriate hidden basis coordinate directions.
% Thus, for any $\vec u \in Q_{\vec v}$, $\vec u$ is a maximum of $\abs{F}\restr{Q_{\vec v}}$ if and only if $\psi^{-1}(\vec u) \in \porth^{\dn - 1}$ is a maximum of $\abs{\tilde F}\restr{\porth^{\dn - 1}}$.
% % demonstrates that by a simple manipulation of the signs of $\myZv_i$, we may relabel any of the hidden orthants $\orthsymb_{\vec v}$ of $S^{\dn - 1}$ as being the all positive orthant $\porth^{\dn - 1}$ within a new BEF $\tilde F$.
% As such, it will suffice when proving \cref{thm:gen-simplex-optima} to show that for {\ansef} $\fg$, the vectors $\myZv_1, \myZv_2, \dotsc, \myZv_\dm$ give a complete enumeration of the maxima of $\abs{\fg} \restr{ \porth^{\dn - 1} }$.

\begin{vlong}
To characterize the extrema structure of the restriction of $\abs F$ to $\porth^{\dn - 1}$, we will use its derivative structure expanded in terms of the $h_i$ functions.
It will be useful to establish some relationships between the $g_i$ and $h_i$ functions.
We denote by $\indicator \bullet$ the indicator function, and we use the convention that any summand containing a $\indicator{\textsc{False}}$ coefficient is 0 even if the term is indeterminant (e.g., $\indicator{\textsc{False}}/0 = 0$ and $\infty\cdot\indicator{\textsc{False}} = 0$).

\begin{lem}\label{lem:h-g-relations}
  The following hold for each $i \in [\dm]$:
  \begin{compactenum}
  \item For $x \in [0, 1]$, $g_i'(x) = 2 h_i'(x^2) x$ and $h_i'(x^2) = \frac{g'(x)}{2 x}\indicator{x \neq 0}$.
  \item For $x \in [0, 1]$, $g_i''(x) = \indicator{x\neq 0}[4 h_i''(x^2)x^2 + 2 h_i'(x^2)]$
  \item Fox $x \in (0, 1]$, $h_i''(x^2) = \frac 1 4 [g_i''(x)/x^2 - g_i'(x)/x^3]$.
  \end{compactenum}
\end{lem}
\begin{proof}
  By construction, $h_i(x^2) = g_i(x)$.
  Taking derivatives, we obtain $2 h_i'(x^2)x = g_i'(x)$.
  Since $h_i'(0) = 0$ by \cref{assumpt:deriv0}, $h_i'(x^2) = \frac{ g_i'(x) }{2 x}\indicator{x \neq 0}$.

  Taking a second derivative away from $x = 0$, we see that $g_i''(x) = 4 h_i''(x^2)x^2 + 2h_i'(x^2)$.
  At $x = 0$, the right derivative is given by:
  \begin{align*}\label{eq:g-second-deriv}
    \partial_+ g_i'(0) &= \lim_{c \rightarrow 0^+} \frac{g_i'(c) - g_i'(0)}{c}
    = 2 \lim_{c \rightarrow 0^+} \frac 1 2 \frac{g_i'(\sqrt c)}{\sqrt c} \\
    &= 2 \lim_{c \rightarrow 0^+} \Big(\frac d {dx} g_i(\sqrt x)\Big)\Big|_{x = c} 
    = 2 \Big(\frac d {dx} g_i(\sqrt x)\Big)\Big|_{x = 0}
    = 0 \ .
  \end{align*}
  In the above, the second equality uses that $g_i'(0) = 0$, a fact which is implied by \cref{assumpt:deriv0} (in particular, $\abs{g_i'(0)} \leq \abs{\lim_{h \rightarrow 0^+} \frac{g(\sqrt h) - g(0)}{\sqrt h}} \leq \abs{\lim_{h \rightarrow 0^+} \frac{g(\sqrt h) - g(0)}{h}} = 0$ since $h \leq \sqrt h$ in a neighborhood of the origin).
  The fourth equality uses that $\frac d {dx} g_i(\sqrt x)$ is continuous due to the convexity of $g_i(\sqrt x)$ \citep[Corollary 4.2.3]{hiriart1996convex}.
  The final equality uses \cref{assumpt:deriv0}.
  
  The argument in \eqref{eq:g-second-deriv} also holds if we replace
  $g_i(x)$ with $g_i(-x)$ since $g_i(-x)$ also satisfies
  \cref{assumpt:gsymmetries,assumpt:deriv0,assumpt:convex,assumpt:origin-val}.
  Hence, $\partial_- g_i'(0) = 0$ and $g_i''(0) = 0$.
  We thus obtain the formula on $[0, 1]$ of
  \begin{displaymath}
    g_i''(x) = \indicator{x\neq 0}[4h_i''(x^2)x^2 + 2h_i'(x^2)]
  \end{displaymath}
  as desired.

  When $x \neq 0$, we may rearrange terms to obtain:
  \begin{displaymath}
    h_i''(x^2) 
    = \frac{g_i''(x) - 2h_i'(x^2)}{4x^2}
    = \frac{g_i''(x)}{4x^2} - \frac{g_i'(x)}{4x^3} \ . \qedhere
  \end{displaymath}
\end{proof}

As $F(\vec u) = \sum_{i=1}^\dm g_i(u_i)$ has first and second order derivatives of $\grad F(\vec u) = \sum_{i=1}^\dm g_i'(u_i)\myZv_i$ and $\HH F(\vec u) = \sum_{i = 1}^\dm g_i''(u_i) \myZv_i \myZv_i^T$, we obtain the following derivative formulas for $F(\vec u)$ in terms of the $h_i$ functions for any $\vec u \in \porth^{\dn - 1}$:
\end{vlong}
\begin{vshort}
  We denote by $\indicator \bullet$ the indicator function of a Boolean variable with the convention that any summand containing a $\indicator{\textsc{False}}$ coefficient is 0 even if the term is undefined (e.g., $\indicator{\textsc{False}}/0 = 0$ and $\infty\cdot\indicator{\textsc{False}} = 0$).
  We obtain the following derivative formulas for $F(\vec u)$ in terms of the $h_i$ functions for any $\vec u \in \porth^{\dn - 1}$:
\end{vshort}
\begin{vlong}
\begin{align}
  \label{eq:F-derivs}
  \grad F(\vec u) &= 2\sum_{i=1}^\dm h_i'(u_i^2)u_i \myZv_i &
  \HH F(\vec u) &= \sum_{i=1}^\dm\indicator{u_i\neq 0}[4 h_i''(u_i^2) + 2 h_i'(u_i^2)]\myZv_i \myZv_i^T
\end{align}
\end{vlong}
\begin{vshort}
  $\grad F(\vec u) = 2\sum_{i=1}^\dm h_i'(u_i^2)u_i \myZv_i$ and 
  $\HH F(\vec u) = \sum_{i=1}^\dm\indicator{u_i\neq 0}[4 h_i''(u_i^2) + 2 h_i'(u_i^2)]\myZv_i \myZv_i^T$.
\end{vshort}

The first derivative necessary condition for $\vec u \in S^{\dn - 1}$ to be an extrema of $F$ over $\porth^{\dn - 1}$ can be obtained using the Lagrangian function $\LL : \overline{B(0, 1)}  \times \R$ defined as $\LL(\vec u, \lambda) := \fg(\vec u) - \lambda [\norm{\vec u}^2 - 1]$.
In particular, a point $\vec u \in \porth^{\dn - 1}$ is a critical point of $\fg$ with respect to $\porth^{\dn - 1}$ \processifversion{vlong}{(that is, it satisfies the first order necessary conditions to be a local maximum of $F$ with respect to $\porth^{\dn - 1}$)} if and only if there exists $\lambda \in \R$ such that $(\vec u, \lambda)$ is a critical point of $\LL$.
The following result then enumerates the critical points of $\fg$ with respect to the $\porth^{\dn - 1}$.
\begin{lem}\label{lem:fg-crit-points}
  Let $\vec u \in \porth^{\dn - 1}$ and $\lambda \in \R$.
  The pair $(\vec u, \lambda)$ is a critical point of $\LL$ if and only if $\lambda \indicator{u_i \neq 0} = h_i'(u_i^2)$ for all $i \in [\dn]$.
\end{lem}
\vnote{The remainder of this section can be cut and summarized in the short version, if need be.}
\begin{proof}
  We set the derivative
  \begin{vlong}
  \begin{equation}\label{eq:Lagrangian-deriv}
  \frac{\partial}{\partial u_i} \LL(\vec u, \lambda) = \partial_i F(\vec u) - 2 \lambda u_i = 2h_i'(u_i^2) u_i - 2\lambda u_i  
  \end{equation}
  \end{vlong}
  \begin{vshort}
    $\frac{\partial}{\partial u_i} \LL(\vec u, \lambda) = \partial_i F(\vec u) - 2 \lambda u_i = 2h_i'(u_i^2) u_i - 2\lambda u_i$
  \end{vshort}
   equal to 0 to obtain $h_i'(u_i^2) u_i = \lambda u_i$.
   If $u_i = 0$, then $h_i'(u_i^2) = h_i'(0) = 0$ by \cref{assumpt:deriv0}.
   Otherwise, $h_i'(u_i^2) = \lambda$.
\end{proof}

While there are exponentially many (with respect to $\dm$) critical points of $F$ as a function on the sphere, it turns out that only the hidden basis directions correspond to maxima of $F$ on the sphere. The proof of the following statements 
uses the convexity structure from \cref{lem:h-props}.

%All other critical points are either saddle points or minima.
%This is formalized in the following Propositions.

\begin{prop}\label{prop:absfg-maxima-canonical}
  If $j \in [\dm]$, then $\myZv_j$ is a strict local maximum of $\abs \fg$ with respect to $\porth^{\dn - 1}$.
\end{prop}
\begin{vlong}
\begin{proof}
  We will prove the case where $h_j$ is strictly convex on $[0, 1]$ and note that the case $h_j$ is strictly concave is exactly the same when replacing $\fg$ with $-\fg$.

  We first note that $\fg(\myZv_j) = h_j(1) > 0$ since $h_j'$ is strictly increasing (see \cref{lem:h-props}).
  In particular, using continuity of each $g_i$, it follows that $\fg(\vec u) > 0$ on a neighborhood of $\myZv_j$, and it suffices to demonstrate that $\fg$ takes on a maximum with respect to % $\porth^{\dn - 1}$ 
  $S^{\dn-1}$ at $\myZv_j$.
  Letting $D_{\vec u}$ denote the derivative operator with respect to the variable $\vec u$ and continuing from \cref{eq:Lagrangian-deriv}, we obtain
  \begin{equation}
    \label{eq:Lagrangian-hessian}
    D_{\vec u}^2 \LL(\vec u, \lambda)
    = \HH F(\vec u) - 2\lambda D_{\vec u} \vec u
    = \sum_{i=1}^\dm \indicator{u_i \neq 0}[4h_i''(u_i^2) u_i^2 + 2h_i'(u_i^2)]\myZv_i\myZv_i^T - 2 \lambda I \ .
  \end{equation}

  We now use the Lagrangian criteria for constrained extrema (see e.g., \citep[chapter 11]{luenberger2008linear} for a discussion of the first order necessary and second order sufficient conditions for constrained extrema) to show that $\myZv_j$ is a maximum of $\fg \restr{\porth^{\dn - 1}}$.
  From \cref{lem:fg-crit-points}, we see that $(\myZv_j, h_j'(1))$ is a critical point of $\LL$.
  Further, for any non-zero $\vec v$ such that $\vec v \perp \myZv_j$, we obtain
  $\vec v^T (D_{\vec u}^2\LL)(\vec \myZv_j, h_j'(1))\vec v = -2h_j'(1) \norm{\vec v}^2$.
  As $h_j'(1) > 0$, it follows that $\vec v^T (D_{\vec u}^2\LL)(\vec \myZv_j, h_j'(1))\vec v < 0$.
  Thus, $\myZv_j$ is a local maximum of $\fg$.
\end{proof}
\end{vlong}

\begin{prop}\label{prop:absfg-maxima-no-extra}
  If $\vec v \in \porth^{\dn - 1}$ is not contained in the set $\{\myZv_i \suchthat i \in [\dm]\}$, then $\vec v$ is not a local maximum of $\abs \fg$ with respect to $\porth^{\dn - 1}$.
\end{prop}
\begin{vshort}
\cref{thm:gen-simplex-optima} follows from \cref{prop:absfg-maxima-canonical,prop:absfg-maxima-no-extra}.
\end{vshort}
\begin{vlong}
\begin{proof}
  We first consider the case in which $v_i = 0$ for all but at most one $i \in [\dm]$.
  We will call this $i \in [\dm]$ for which $v_i \neq 0$ as $j$ if it exists and otherwise let $j \in [\dm]$ be arbitrary.
  Fix any $\vec w \in \porth^{\dn - 1}$ such that $w_j > v_j$ and $w_i = 0$ for $i \in [\dm] \setminus \{j\}$.
  Such a choice is possible since $\vec v \neq \myZv_j$ implies $v_j < 1$.
  Then, $\abs{\fg(\vec v)} = \abs{h_j(v_j^2)}$ and $\abs{\fg(\vec w)} = \abs{h_j(w_j^2)}$.
  Since $\abs{h_j(t)}$ is a strictly increasing function on $[0, 1]$ from $\abs{h_j(0)} = 0$ (see \cref{lem:h-props}), it follows that $\abs{\fg(\vec w)} > \abs{\fg(\vec v)}$.
  Since $\vec w$ can be constructed in any open neighborhood of $\vec v$, $\vec v$ is not a local maximum of $\abs \fg$ on $\porth^{\dn - 1}$.


  Now, we consider the case where $\vec v$ is an extremum (either a maximum or a minimum) of $\abs \fg$ with respect to $\porth^{\dn - 1}$ such that there exists $j, k \in [\dm]$ distinct such that $v_j > 0$ and $v_k > 0$.
  We will demonstrate that this implies that $\vec v$ is a minimum of $\abs \fg$.
  % Construct the vector $\vec w = \vec e_j - \vec e_k$.  Then, $\vec w \in \R^\dn \cap \vec v^\perp$, and $\vec w^T D^2_{\vec u}\LL(\vec v, \lambda^*)\vec w = 4[h_j''(\psi_j(\vec v))v_j^2 + h_k''(\psi_k(\vec v))v_k^2]$.
  % Note that for any $\delta > 0$, strict convexity of $h$ implies that 

  We use the notation for a vector $\vec u$, $\vec u \elpow k := \sum_i u_i^k \vec e_i$ is the coordinate-wise power.
  Fix $\eta > 0$ sufficiently small that for all $\delta \in (-\eta, \eta)$ we have that $\vec w(\delta) := (\vec v\elpow 2 + \delta \myZv_j - \delta \myZv_k)\elpow{1/2} \in \porth^{\dn - 1}$.
  We now consider the difference $\fg(\vec w(\delta)) - \fg(\vec v)$ for a non-zero choice of $\delta \in (-\eta, \eta)$:
  \begin{align*}
    \fg(\vec w(\delta))-\fg(\vec v) 
    &= h_j(w_j(\delta)^2) - h_j(v_j^2) + h_k(w_k(\delta)^2) - h_k(v_k^2) \\
    &= h_j'(x_j(\delta)^2)[w_j(\delta)^2 - v_j^2] + h_k'(x_k(\delta)^2)[w_k(\delta)^2 - v_k^2] \\
    &= \delta[h'_j(x_j(\delta)^2) - h'_k(x_k(\delta)^2)] \ ,
  \end{align*}
  where $x_i(\delta) \in (v_j, w_j(\delta))$ and $x_i(\delta) \in (w_k(\delta), v_k)$ under the mean value theorem.

  As $\vec v$ must be an extremum of $\fg$ in order to be an extremum of $\abs \fg$, there exists $\lambda$ such that the pair $(\vec v, \lambda)$ is a critical point of $\LL$.
  Let $\SS = \{ i \suchthat v_i \neq 0\}$.
  \Cref{lem:fg-crit-points} implies that $\lambda = h_i'(v_i^2)$ for all $i \in \SS$.
  In particular, $\sign(h_i'(v_i^2))$ is the same for each $i \in \SS$, and we will call this sign value $s$.
  Under \cref{eq:fg-via-his}, we have $\fg(\vec v) = \sum_{i \in \SS} h_i(v_i^2)$.
  By \cref{lem:h-props}, $sh_i$ is strictly increasing from $sh_i(0)=0$ on $\pinterval$ for each $i \in \SS$.
  As such, $\fg(\vec v)$ is separated from 0 and $\sign(\fg(\vec v)) = s$.
  Further,
  \begin{displaymath}
    s[\fg(\vec w(\delta))-\fg(\vec v)] 
    = s\delta[h'_j(x_j(\delta)^2) - h'_k(x_k(\delta)^2)]
    < s\delta[\lambda - \lambda] = 0
  \end{displaymath}
  holds by noting that each $sh_i'$ is strictly increasing on $\pinterval$ (by \cref{lem:h-props}).
  Thus, $\vec v$ is a minimum of $\abs \fg$.
\end{proof}


\Cref{thm:gen-simplex-optima} follows by combining \cref{prop:absfg-maxima-canonical,prop:absfg-maxima-no-extra} and using the symmetries of $F$ from \cref{assumpt:gsymmetries}. % \cref{lem:orth-transform}.
\end{vlong}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> simplexframework - Copy/spectral-error-analysis.tex <==
\def\myL{L}
\def\mygap{\delta_\edim}
\def\edim{\ensuremath{k}}
\def\AppendixLabel{Appendix}
\def\wmin{\ensuremath{w_{\mathrm{min}}}}
\def\wmax{\ensuremath{w_{\mathrm{max}}}}
\def\tabs{\mathrm{abs}}
\def\dnold{\dn}
\def\dn{n}
\section{Perturbation Analysis of Spectral Clustering}
\label{sec:spectral-pert-analysis}

We now revisit the spectral clustering method introduced in \cref{sec:example-befs} for performing multi-way clustering of vertices within a graph.
First, in \cref{sec:Laplacian-structure} we briefly describe the structure of the spectral embedding, and note that it leads to a basis recovery problem when working with graphs consisting of $\edim$ connected components.
Then, in \cref{sec:spectral-laplacian-pert,sec:pert-analys-clust}, we show that under a perturbation from the setting of $\edim$ connected components, we are able to recover the underlying clusters using our {\sef} framework.

\subsection{\Sef\@ Structure of the Spectral Embedding}
\label{sec:Laplacian-structure}

We consider an undirected graph $G$ with non-negative edge weights.
The goal in graph clustering is to partition the vertices of $G$ into sets which are internally well connected.
Spectral clustering is commonly used for performing such a clustering.

Spectral clustering proceeds in two steps.
When looking for $\edim$ clusters, the vertices of $G$ are first
embedded into $\R^\edim$ using a process called the \emph{Laplacian
embedding}.
Then, the resulting embedded vertices are clustered within $\R^\edim$ typically using a clustering algorithm defined in Euclidean space such as $k$-means.
Interestingly, when $G$ consists of $\edim$ connected components, the Laplacian embedding induces an orthogonality structure upon the embedded vertices that allows us to construct \ansef\@ with which to perform the clustering. 

To define the Lablacian embedding, we must first introduce some notations.
We denote by $A$ the adjacency matrix of our graph $G$, i.e.\@ $A_{ij}$ is the
weight of the edge connecting vertices $i$ and $j$ if an edge is present and 0
if no edge is present.
We denote by $D$ the diagonal matrix with its $i$\textsuperscript{th} diagonal
entry being the degree of the $i$\textsuperscript{th} vertex, i.e., $D_{ii} :=
\sum_{j} A_{ij}$.
The graph Laplacian is defined by $L := D - A$.

Throughout this section, we will make use of several properties of the graph Laplacian (see \cite{von2007tutorial} for an overview).
A perhaps more intuitive alternate definition of the graph Laplacian  is that for all $\vec x \in \R^\dn$, $\vec x^T L \vec x = \frac 1 2 \sum_{i, j} A_{ij}(x_i - x_j)^2$.
From this characterization, it can be demonstrated that $L$ is positive semi-definite, and that the multiplicity of its $0$ eigenvalue is the same as the number of connected components in $G$.
When $G$ consists of $\edim$ connected components, the Laplacian embedding into $\R^\edim$ is actually formed using the null space of the Laplacian.

In general, the Laplacian embedding is constructed as follows: We let
$X \in \R^{\dn \times \edim}$ be a matrix such that its columns $X =
[\vec x_{\vecdot 1}, \dotsc, \vec x_{\vecdot \edim}]$ are the lowest
$\edim$ eigenvectors of $L$ scaled such that $\norm{\vec x_{\vecdot
    i}} = \sqrt \dn$.
Then, the rows $\vec x_{1 \vecdot}, \dotsc, \vec x_{\dn \vecdot}$ of
$X$ are the embeddings of the $\dn$ vertices of $G$.

% As such, we have by definition that $A_{ij} = 0$ if $i \in S_k$, $j \in S_\ell$, and $k \neq \ell$.

% The degree matrix $D$ is a diagonal matrix with entries $D_{ii} = \sum_{j=1}^\dn A_{ij}$.

% The goal in graph clustering problem is to partition the vertices into sets which are internally well connected.
% One popular set of ideas for graph clustering is spectral clustering.
% Spectral clustering proceeds in two steps:
% \begin{enumerate}
% \item \emph{Laplacian Embedding.}
%   The graph Laplacian is defined by $L := D - A$.
%   Let $X$ be a matrix such that its columns are the bottom $\edim$ eigenvectors of $L$ scaled such that each column has $\sqrt \dn$-norm.
%   If we denote the rows of $X$ by $X = [\vec x_1^T, \dotsc, \vec x_\dn^T]^T$, then the $\vec x_1, \dotsc, \vec x_\dn$ form the embeddings for the vertices of the graph $G$.
% \item \emph{Clustering Step.}
%   Using the properties of the Laplacian embedding, it is assumed that the desired clusters within the graph are mapped to nice point clouds (natural clusters) in the embedded space $\R^\edim$.
%   A clustering algorithm is employed in the embedded space to recover the desired clusters.
% \end{enumerate}

% There are multiple ways of interpreting what spectral clustering accomplishes.
% Here, we start by noting that for a graph consisting of $\edim$ connected components, the spectral embedding takes on a very simple form in which each of the embedded points $\vec x_i$ from the same component are mapped to a single point forming very natural clusters.
% In the upcoming sections, we view the case of a fully connected graph $G$ (as seen in practice) as being a perturbation from the setting of $k$ connected components, and we show that we can recover the desired underlying clusters---i.e., the clusters corresponding to the $\edim$ connected components in the unperturbed graph---assuming that the perturbation is sufficiently small.
% We note that more generally, spectral clustering can also be viewed as a generalization of the NP hard multi-way ratio cut problem \citep[section 5]{von2007tutorial}.
%In particular, when $G$ consists of $\edim$ connected components, the Laplacian embedding takes on a very simple form.
%Further, a fully connected graph (i.e., one which arises in practice) can be viewed as a perturbation from 
%
%When the graph $G$ is fully connected, there are multiple ways of interpreting what this clustering process accomplishes.
%One intuitive goal of graph clustering is minimize certain normalized cuts induced by partitioning the graph into $\edim$ clusters.
%In particular, spectral clustering using the unnormalized graph Laplacian described can be viewed as a relaxation of the NP-hard problem of min ratio cut for a $\edim$-partitioning of the graph $G$ into clusters \citep[section 5]{von2007tutorial}.

The orthogonality structure of the Laplacian embedding is described by the following Lemma (adapted from \citep{BelkinRV14}).
\begin{lem}\label{prop:discrete-simplex}
  Suppose that the graph $G$ consists of $\edim$ connected components with corresponding index sets $S_1, \dotsc, S_\edim$.
  Suppose that $\vec x_1, \dotsc, \vec x_\dn \in \R^\edim$ are the embeddings the of vertices of $G$ under the Laplacian embedding.
  Then, there exists orthogonal unit vectors $\myZv_1, \dotsc, \myZv_\edim$ in $\R^\edim$ such that $\vec x_i = \sqrt{\dn/\abs{S_j}}\myZv_j$ for all $i \in S_j$.
\end{lem}

Using that the embedded vertices for each component of $G$ are orthogonal to each other, we are able to construct \ansef\@ from the embedded data as follows.
\begin{construction}\label{constr:spectral-Fg-L}
  We proceed under the assumptions and notation of \cref{prop:discrete-simplex}.
  Let $g : \R^\edim \rightarrow \R$ be a twice continuously differtiable function satisfying \crefrange{assumpt:first}{assumpt:last}.
  We define the function $F : \R^\edim \rightarrow \R$ by
  \begin{displaymath}
    F(\vec u) := \frac 1 \dn \sum_{i = 1}^\dn g(\ipCanonical{\vec u}{\vec x_i}) \ .
  \end{displaymath}
  By \cref{prop:discrete-simplex}, we see that for all $j \in [\edim]$, there $\abs{S_j}$ copies of the point $\sqrt{\dn / \abs{S_j}} \myZv_j$ among the embedded vertices.
  Defining $w_j := \abs{S_j} / {\dn}$, we may thus equivalently write:
  \begin{equation}\label{eq:f_weighted_form}
    F(\vec u) := \sum_{i = 1}^\edim w_j g(w_j^{-\frac 1 2} \ipCanonical{\vec u}{\myZv_i}) \ .
  \end{equation}
  We define coordinate functions $g_i : \R \rightarrow \R$ by $g_i(t) := w_j g(w_j^{- \frac 1 2} t)$.
  Then, we may write that $F(\vec u) = \sum_{i = 1}^\edim g_i(\ipCanonical{\vec u}{\myZv_i})$.
  As it may be verified that the coordinate functions also satisfy \crefrange{assumpt:first}{assumpt:last}, we obtain that $F$ is \ansef\@.
\end{construction}

When the graph $G$ consists of $\edim$ connected compoenents, the spectral embedding gives rise to \ansef\@.
As such, the gradient iteration algorithm (\cref{alg:gi-generic}) can be used to recover the underlying directions $\myZv_i$ up to sign.
If $\hat \myZv_i$ denote the recovered basis directions, then we may cluster the vertices of $G$ by assigning the $i$\textsuperscript{th} vertex to the cluster $\argmax_{j \in [\edim]} \abs{\ipCanonical{\vec x_i}{\hat \myZv_i}}$.

\subsection{Perturbation of the Spectral Embedding}\index{spectral embedding!perturbation}\label{sec:spectral-laplacian-pert}
We have now seen that when $G$ consists of $\edim$ connected components, the components can be recovered by making use of the \sef\@ structure of the Laplacian embedding described in \cref{prop:discrete-simplex,constr:spectral-Fg-L}.
However when performing spectral clustering, one typically observes a graph which is fully connected and tries to discover natural clusters in such a graph.
We now wish to demonstrate that when an observed graph has an adjacency matrix which is close to that of a ``clean'' graph consisting of $\edim$ connected components, then the clusters corresponding to the connected components in the clean graph can be recovered from the observed graph using spectral clustering.

Our analysis proceeds in two steps.
In this subsection, we analyze the Laplacian embedding induced by a perturbation from the setting of $\edim$ connected components.
This demonstrates that when we are close to the setting of $\edim$ connected components, the orthogonality structure of the Laplacian embedding from \cref{prop:discrete-simplex} is approximately preserved.
Then, in \cref{sec:pert-analys-clust} we apply our gradient iteration error analysis to demonstrate that \textsc{RobustGI-Recovery} (\cref{alg:FullRecovery}) can be employed to robustly recover the desired vertex clusters.

For the remainder of \cref{sec:spectral-pert-analysis}, we assume that $\myL
:= D - A$ is the graph Laplacian constructed from a graph $G$ consisting of
$\dn$ vertices arranged in $\edim$ connected components.
Let $\lambda_1(\myL) \leq \lambda_2(\myL) \leq \cdots \leq \lambda_\dn(\myL)$
denote the eigenvalues of $\myL$.
Under our assumptions, $0 = \lambda_1(\myL) = \lambda_2(\myL) =
\cdots = \lambda_\edim(\myL) < \lambda_{\edim + 1}(\myL)$ \citep[Proposition 2]{von2007tutorial}.
Throughout this section, we denote by $\mygap(\myL) = \lambda_{\edim+1}(\myL)
- \lambda_{\edim}(\myL)$ the eigengap between the null space of $\myL$
(denoted by $\NN(\myL)$) and the range of $\myL$ (denoted as $\RR(\myL)$).
We further assume that $\tilde G$ is a pertubed version of $G$ such that the
graph Laplacian $\tilde L$ constructed from $\tilde G$ satisfies $\tilde \myL
= \myL + H$ for some perturbation $H$.
By the construction, $\tilde L$, $L$, and $H$ are symmetric.
We obtain the following perturbation result for the spectral embedding.

\begin{thm} \label{thm:pert-simplex-embedding}
  Suppose that $\norm H < \mygap(L)$ and that
  $\tilde X = (\tilde x_{\vecdot 1}, \dotsc, \tilde x_{\vecdot \edim})$ contains the lowest $\edim$ eigenvectors of $\tilde \myL$ as its columns, scaled such that $\norm{\tilde x_{\vecdot i}} = \frac 1 {\sqrt \dn}$ for all $i \in [\edim]$.
  Then there exists $X = (x_{\vecdot 1}, \dotsc, x_{\vecdot \edim})$ with columns forming a scaled orthogonal basis of $\NN(\myL)$ such that each $\norm{x_{\vecdot i}} = \frac 1 {\sqrt \dn}$ and $\frac 1 {\sqrt \dn} \norm{X - \tilde X} \leq \frac{2 \norm H}{\mygap(\myL) - \norm H}$.
\end{thm}

\begin{rmk}\label{rmk:pert-simplex-embedding}
    In \cref{thm:pert-simplex-embedding}, the bound on $\frac 1 {\sqrt \dn}\norm{X - \tilde X}$ also implies:
  \begin{compactenum}
    \item If $\vec v \in \R^\edim$ is a unit vector, then $\frac 1 \dn \sum_{i=1}^\dn (\ipCanonicalp{\tilde x_{i \vecdot}}{\vec v} - \ipCanonicalp{ x_{i \vecdot}}{\vec v})^2 \leq \frac{4 \norm H^2}{(\mygap(\myL) - \norm H)^2}$.
    \item $\frac 1 \dn \sum_{i=1}^\dn \norm{\tilde x_{i \vecdot} - x_{i \vecdot}}^2 \leq \frac{4 \norm H^2 \edim}{(\mygap(\myL) - \norm{H})^2}$.
  \end{compactenum}
\end{rmk}

\Cref{thm:pert-simplex-embedding} implies that the
orthogonal basis structure from \cref{prop:discrete-simplex} 
is approximately preserved under a perturbation.
To see the sorts of assumptions under which $\norm H$ is small relative to the eigengap $\mygap(L)$, we refer the reader to the work of \mycitet{Ng et al.}{ng2002spectral}.
In their work, they analyze the spectral embedding quality of the symmetric normalized Laplacian $D^{-1/2}LD^{-1/2}$ under a similar perturbation.

We now proceed with the proof of \cref{thm:pert-simplex-embedding}.
The following Lemma is a direct implication of the $\sin \Theta$ theorem\index{sin $\Theta$ theorem} of  \mycitet{Davis and Kahan}{davis1970rotation}, which is reproduced in \cref{sec:error-bounds-eigenv} as \cref{thm:sin-theta-thm}.
\begin{lem}\label{lem:pert-sin-theta}
  Suppose that $\norm H < \mygap(L)$,
  that $X = (x_{\vecdot 1}, \dotsc, x_{\vecdot \edim})$ is an orthogonal basis of $\NN(\myL)$,
  and that $\tilde X = (x_{\vecdot 1}, \dotsc, x_{\vecdot \edim})$ are the bottom $\edim$ eigenvectors of $\tilde \myL$.
  Then, $\norm{P_{\NN(X)} P_{\RR(\tilde X)}} \leq \frac{\norm H}{\mygap(\myL) - \norm H}$.
\end{lem}

We now decompose the bound from \cref{lem:pert-sin-theta} in order to
write a bound in terms of the actual entries of $X$ and $\tilde X$.
This is complicated by the fact that $X$ is only meaningfully defined up to a
rotation of its columns within the subspace $\NN(\myL)$.
In \cref{lem:pert-sin-theta}, this is reflected by the fact that we are
bounding the change in the projection operators onto the subspaces spanned by
$X$ and $\tilde X$ rather than directly bounding the change in the
eigenvectors themselves.
Indeed, if $X$ and $Y$ contained two different bases of $\NN(\myL)$ in their
columns (with the columns of $X$ and $Y$ scaled to have $\sqrt \dn$-norm),
then $R = \frac 1 \dn X^T Y$ would be the rotation%
\footnote{For our purposes, a rotation matrix is an element of the general
  orthogonal group $O(k)$.
  In particular, we allow orthogonal matrices $R$ with
  determinant satisfying either $\det(R) = +1$ or $\det(R) = -1$.
}
matrix providing a transition between the coordinate systems of these two bases of $\NN(L)$.
If $X$ and $\tilde X$ are constructed from the $\edim$ lowest eigenvectors of
$\myL$ and its perturbation $\tilde \myL$ respectively, then we may view
$\frac 1 n X^T \tilde X$ as being an approximate rotation matrix.
In the following two Lemmas, we deal directly with the issues arising from
this missing rotation in \cref{lem:pert-sin-theta}.
% The following Lemmas provide the key steps in proving \cref{thm:pert-simplex-embedding} by directly taking into account this missing rotation.
\begin{lem}\label{lem:pert-arb-rotation}
  Suppose that $\norm H < \delta (L)$, that $X = (x_{\vecdot 1},
  \dotsc, x_{\vecdot \edim})$ contains an orthogonal basis of
  $\NN( \myL )$ scaled such that each $\norm{x_{\vecdot i}} = \sqrt
  \dn$, and that $\tilde X = (\tilde x_{\vecdot 1}, \dotsc, \tilde
  x_{\vecdot \edim})$ contains the lowest $\edim$ eigenvectors
  of $\tilde \myL$ scaled such that each $\norm{\tilde x_{\vecdot i}}
  = \sqrt \dn$.
  Then, for any rotation matrix $R \in \R^{\edim \times \edim}$,
  $\frac 1 {\sqrt \dn} \norm{XR - \tilde X} 
  \leq \frac{\norm H}{\mygap(\myL) - \norm H} 
       + \norm{\frac 1 \dn X^T \tilde X - R}$. 
\end{lem}
\begin{proof}
  Applying \cref{lem:pert-sin-theta}, we obtain that
  $\norm{P_{\NN(X)} P_{\RR(\tilde X)}} \leq \frac{\norm H}{\mygap(\myL) - \norm H}$.
  Since $\frac 1 {\sqrt \dn} \tilde X^T$ treated as a map from $\RR(\tilde X)$ to $\R^\edim$ is an isometry, we obtain that
  \begin{align*}
    \norm{P_{\NN(X)} P_{\RR(\tilde X)}}
    &= \norm{(\Id - \frac 1 \dn XX^T) \frac 1 \dn \tilde X \tilde X^T} \\
    &= \norm{(\Id - \frac 1 \dn XX^T) \frac 1 {\sqrt \dn} \tilde X}
    = \frac 1 {\sqrt \dn} \norm{\tilde X - \frac 1 \dn XX^T\tilde X} \ .
  \end{align*}
  We fix a rotation matrix $R$ and expand $\frac 1 \dn X^T \tilde X = \frac 1 \dn X^T \tilde X - R + R$ to obtain:
  \begin{align}
    \norm{P_{\NN(X)} P_{\RR(\tilde X)}}
    &= \frac 1 {\sqrt \dn} \norm{\tilde X - XR + X(R - \frac 1 \dn X^T\tilde X)} \nonumber \\
    &\geq \frac 1 {\sqrt \dn}( \norm{\tilde X - XR} - \norm{X(R - \frac 1 \dn X^T \tilde X}) \ . \label{eq:pert-sin-theta-1}
  \end{align}
  Treating $\frac 1 {\sqrt \dn} X$ as a linear map from $\RR(X)$ to
  $\R^\edim$ defined by the left multiplication 
  $\vec u \mapsto \frac 1 {\sqrt \dn} \vec u^T X$, 
  then $\frac 1 {\sqrt \dn} X$ is an isometry.
  As such, $\norm{\frac 1 {\sqrt \dn} X(R - \frac 1 \dn X^T \tilde X)} = \norm{R - \frac 1 \dn X^T \tilde X}$.
  Rearranging terms in \cref{eq:pert-sin-theta-1} and then applying \cref{lem:pert-sin-theta}, we obtain:
  \begin{align*}
    \frac 1 {\sqrt \dn} \norm{\tilde X - X R} 
    &\leq \norm{P_{\NN(X)}P_{\RR(\tilde X)}} + \norm{R - \frac 1 \dn X^T \tilde X} \\
    &\leq \frac{\norm H}{\mygap(\myL) - \norm H} + \norm{R - \frac 1 \dn X^T \tilde X} \ . \qedhere
  \end{align*}
  % where the final inequality uses \cref{lem:pert-sin-theta}.
\end{proof}
\begin{lem}\label{lem:pert-rotation-existence}
  Under the assumptions of \cref{lem:pert-arb-rotation},
  there exists a rotation matrix $R \in \R^{\edim \times \edim}$ such that $\norm{R - \frac 1 \dn X^T \tilde X} \leq \norm{P_{\NN(X)}P_{\RR(\tilde X)}} \leq \frac{\norm H}{\mygap(\myL) - \norm H}$.
\end{lem}
\begin{proof}
  Letting $U \Sigma V^T$ be a singular value decomposition of $\frac 1 \dn X^T \tilde X$, we consider the rotation $R = UV^T$.
  For this choice of $R$, $\norm{R - \frac 1 \dn X^T \tilde X} = \norm{U(\Id-\Sigma)V^T} = \norm{\Id - \Sigma}$.
  To see that $\norm{R - \frac 1 \dn X^T \tilde X} \leq \norm{P_{\NN(X)} P_{\RR(\tilde X)}}$, 
  it suffices to show that all of the singular values of $\frac 1 \dn X^T \tilde X$ are contained in the interval $[1 - \norm{P_{\NN(X)}P_{\RR(\tilde X)}}, 1]$.
  
  We denote the singular values of $\frac 1 \dn X^T \tilde X$ by the decreasing sequence $\sigma_1(\frac 1 \dn X^T \tilde X) \geq \cdots \geq \sigma_\edim(\frac 1 \dn X^T \tilde X)$.
  An upper bound is given by 
  \begin{displaymath}
    \sigma_1( \frac 1 \dn X^T \tilde X) = \norm{\frac 1 \dn X^T \tilde X} \leq \frac 1 \dn \norm{X^T} \norm{\tilde X} \leq 1 \ .
  \end{displaymath}
  
  We now find a lower bound on the singular values.
  Construct the matrix $Y \in \R^{\dn \times (\dn-\edim)}$ such that the columns of $[X\ Y]$ forms a scaled orthogonal basis of $\R^\dn$ with each column having $\sqrt \dn$ norm.
  By construction, $\sigma_1(\frac 1 \dn [X\ Y]^T \tilde X) = \cdots = \sigma_\edim(\frac 1 \dn  [X\ Y]^T \tilde X) = 1$. 
  % and $\sigma_{\edim + 1}(\frac 1 \dn  [X\ Y]^T \tilde X) = \cdots = \sigma_\dn(\frac 1 \dn  [X\ Y]^T \tilde X) = 0$.
  Expanding $\frac 1 \dn [X\ Y]^T \tilde X = \frac 1 \dn X^T \tilde X + \frac 1 \dn Y^T \tilde Y$, we obtain from a Weyl's inequality like bound for singular values \citep[Theorem 3.3.16]{horn37topics} that $\sigma_\edim(\frac 1 \dn [X\ Y]^T \tilde X) \leq \sigma_\edim(\frac 1 \dn X^T \tilde X) + \sigma_1(\frac 1 \dn Y^T \tilde X)$.
  Hence, $\sigma_\edim(\frac 1 \dn  X^T \tilde X) \geq \sigma_\edim(\frac 1 \dn [X\ Y]^T \tilde X) - \sigma_1(\frac 1 \dn  Y^T \tilde X) = 1 - \norm{\frac 1 \dn  Y^T \tilde X}$.
  Noting that the maps $\frac 1 {\sqrt \dn} Y : \RR(Y) \rightarrow \R^\edim$ defined by $\vec u \mapsto \frac 1 {\sqrt \dn} \vec u^T Y$ and $\frac 1 {\sqrt \dn} \tilde X^T : \RR( \tilde X ) \rightarrow \R^\edim$ defined by $\vec u \mapsto \frac 1 {\sqrt \dn} \tilde X^T \vec u$ are isometries, it follows that $\norm {\frac 1 \dn Y^T \tilde X} = \norm{ \frac 1 {\dn^2} YY^T \tilde X \tilde X^T } = \norm{P_{\NN(X)} P_{\RR(\tilde X)}}$.
  In particular, $\sigma_\edim(\frac 1 \dn X^T \tilde X) \geq 1 - \norm{P_{\NN(X)} P_{\RR(\tilde X)}}$ as desired.

  We have demonstrated that $\norm{R - \frac 1 \dn X^T \tilde X} \leq \norm{P_{\NN(X)} P_{\RR(\tilde X)}}$.
  To see the final inequality $\norm{P_{\NN(X)} P_{\RR(\tilde X)}} \leq \frac{\norm H}{\mygap(L) - \norm H}$, we apply \cref{lem:pert-sin-theta}.
\end{proof}

\Cref{lem:pert-arb-rotation,lem:pert-rotation-existence} combine to provide the following bound on the embedding error.

\begin{prop} \label{prop:pert-simplex-embedding-rotation}
  Suppose that $\norm H < \mygap(L)$,
  that $X = (x_{\vecdot 1}, \dotsc, x_{\vecdot \edim})$ contains a scaled orthogonal
  basis of $\NN(\myL)$ such that each $\norm{x_{\vecdot i}} = \frac 1 {\sqrt \dn}$,
  and that $\tilde X = (\tilde x_{\vecdot 1}, \dotsc, \tilde x_{\vecdot \edim})$
  contains the lowest $\edim$ eigenvectors of $\tilde \myL$ scaled such that
  each $\norm{\tilde x_{\vecdot i}} = \frac 1 {\sqrt \dn}$.
  There exists an orthogonal matrix $R \in \R^{\edim \times \edim}$ such that $\frac 1 {\sqrt \dn}\norm{X R - \tilde X} \leq \frac{2 \norm H}{\mygap(\myL) - \norm H}$.
\end{prop}

\Cref{thm:pert-simplex-embedding} follows by setting $X$ in \cref{thm:pert-simplex-embedding} to be $XR$ from \cref{prop:pert-simplex-embedding-rotation}.

\subsection{Perturbation Analysis of Cluster Recovery}
\label{sec:pert-analys-clust}
We now complete the perturbation analysis of spectral clustering.
We let $\fg : \R^{\edim} \rightarrow \R$ be as in
\cref{constr:spectral-Fg-L} (for a ``clean'' graph consisting of $\edim$ connected components).
We will first demonstrate that when $g$ is a robust contrast function
satisfying the \crefrange{assumpt:first}{assumpt:last}, then $F_g$
a robust \sef\@.
With this observation, we may construct $\tilde F_g$ an estimate of $F_g$ from the perturbed graph $G$ and then use our error analysis of the gradient
iteration\index{gradient iteration!error analysis} algorithm to provide a perturbation analysis for our spectral clustering method.
In particular, we will propagate the perturbation analysis of the
spectral embedding\index{spectral embedding!perturbation}
(\cref{sec:spectral-laplacian-pert}) to provide bounds on our
estimate of $\nabla F_g$.
Then, by applying the error analysis of the gradient iteration algorithm, we will bound the allowable perturbation size for perfect cluster recovery.

We now proceed with demonstrating that $F_g$ is a robust \sef\@.
% However, as we are interested in using the error analysis of the gradient iteration for spectral clustering, we will discuss the conditions are which $F_g$ is $(\alpha, \beta, \gamma, \delta)$-robust.
% Since $F_g$ for spectral clustering is built from a single contrast $g$, we will make use of the following definition for robustness of a single contrast function to for a bridge between individual contrast functions being robust and \ansef\@ being robust.

% \begin{defn}\label{def:contrast-robust}
%   Let $D \subset \R$.
%   A contrast function $g : D \rightarrow \R$ is said to be $(\alpha, \beta, \gamma, \delta)$-robust on its domain $D$ if the constants $\alpha, \beta, \gamma$, and $\delta$ are strictly positive and if for all $x \in D$, $\beta x^{\gamma - 1} \leq \Abs{\frac{d^2}{d t^2}[g(\sqrt t)]\big|_{t = x}} \leq \alpha x^{\delta - 1}$.
% \end{defn}
% In particular, comparing with \cref{defn:BEF-robust}, we see that \ansef\@ $F(\vec u) = \sum_{i=1}^\ldim g_i(\ipCanonical{\vec u}{\hbev_i})$ is $(\alpha, \beta, \gamma, \delta)$-robust precisely if each of its contrasts $g_i$ are $(\alpha, \beta, \gamma, \delta)$-robust on the domain $(0, 1]$.
% Using this connection, we may rewrite the function $F_g$ arising in spectral clustering as \ansef\@, and observe the relationship between robustness of $g$ and robustness of $F_g$.
\begin{lem}\label{lem:fg-spectral-robust}
  % \vnote{Add assumptions about $g$?}
  Suppose $F_g$ and all related variables are as in
  \cref{constr:spectral-Fg-L}.
  Suppose that $g$ satisfies
  \crefrange{assumpt:first}{assumpt:last} on the domain
  $[-\frac 1 {\sqrt{w_{\min}}},\ \frac 1 {\sqrt{w_{\min}}}]$.
  Suppose we define $g_i : \R \rightarrow \R$ by $g_i(t) := w_i g(\frac 1 {\sqrt {w_i}} \abs t)$ for all $i \in [\edim]$.
  Then,
  \begin{enumerate}
  \item\label{lem:fg-spectral-robust:constr}
    $F_g(\vec u) = \sum_{i=1}^\edim g_i(\ipCanonical{\vec u}{\myZv_i})$ 
    is \ansef\@ (satisfying
    \crefrange{assumpt:first}{assumpt:last}) with hidden
    basis $\myZv_1, \dotsc, \myZv_\edim$.
  \item\label{lem:fg-spectral-robust:robustness}
    If $g$ is $(\alpha,$ $\beta,$ $\gamma,$ $\delta)$-robust on the domain
    $(0, \frac 1 {\sqrt{w_{\min}}}]$, then the \sef\@ $F_g$ is 
    $(\frac \alpha {w_{\min}^\gamma},$ $\frac{\beta}{w_{\max}^\delta},$ $\gamma,$
    $\delta)$-robust.
  \end{enumerate}
\end{lem}
\begin{proof}
  We first prove part~\ref{lem:fg-spectral-robust:constr}.
  To see this, we expand each $g_i$ according to its definition to see:
  \begin{align*}
    \sum_{i=1}^\edim g_i(\ipCanonical {\vec u}{\myZv_i})
    = \sum_{i = 1}^\edim w_i g(\frac 1 {\sqrt {w_i}} \abs{\ipCanonical{\vec u}{\myZv_i}})
    = F_g(\vec u) \ ,
  \end{align*}
  by using \cref{eq:f_weighted_form}.
  Further, since the weights $w_1, \dotsc, w_\edim$ are non-zero and
  $g$ satisfies \crefrange{assumpt:first}{assumpt:last},
  it follows that each $g_i$ satisfies
  \crefrange{assumpt:first}{assumpt:last}.
  In particular, $F_g$ is \ansef\@.
  
  We now consider part~\ref{lem:fg-spectral-robust:robustness}.
  We note that on $(0, 1]$, $g_i(t) = w_i g(\frac 1 {\sqrt {w_i}} t)$ by construction.
  We may thus define the functions $h_i(t) := g_i(\sqrt t)$ and $h(t) := g(\sqrt t)$.
  We see that $h_i(t) = g_i(\sqrt t) = w_i g(\frac 1 {\sqrt{w_i}} \sqrt t) = w_i h( \frac t {w_i} )$.
  Taking derivatives, we obtain (for any $t \in (0, 1]$):
  \begin{equation}\label{eq:spectral-fg-gi-expansion}
    \frac{d^2}{d x^2}[g_i(\sqrt x)]\big|_{x=t}
    = h_i''(t) 
    = \frac 1 {w_i} h''( \frac t {w_i} )
    = \frac 1 {w_i} \cdot \frac{d^2}{d x^2}[g(\sqrt x)]\big|_{x={t/{w_i}}} \ .
  \end{equation}
  Since $g$ is $(\alpha, \beta, \gamma, \delta)$-robust, we see from \cref{eq:spectral-fg-gi-expansion} that for all $t \in (0, 1]$ and all $i \in [\edim]$,
  \begin{align*}
    \Abs{\frac{d^2}{d x^2}[g_i(\sqrt x)]\big|_{x=t}}
    &\in [\frac \beta {w_i} (t/{w_i})^{\delta - 1},\ \frac \alpha {w_i} (t/w_i)^{\gamma - 1}] \\
    &= [\frac \beta {w_i^\delta} t^\delta, \ \frac \alpha {w_i^\gamma} t^\gamma]
    \subset [\frac \beta {w_{\max}^\delta} t^\delta, \ \frac \alpha {w_{\min}^\gamma} t^\gamma] \ .
  \end{align*}
  Hence, $F_g$ is $(\frac \alpha {w_{\min}^\gamma}, \frac \beta {w_{\max}^\delta}, \gamma, \delta)$-robust.
\end{proof}
  % Suppose $F_g$ and all related variables are as in
  % \cref{constr:spectral-Fg-L}.
  
We will now combine the results from
\cref{sec:spectral-laplacian-pert} on the error analysis of the
spectral embedding with \cref{lem:fg-spectral-robust} to provide
an error analysis of the entire spectral clustering framework.
For this purpose, we will first define in
\cref{constr:BEF-spectral-pert-exact-Fg} below what is
meant by the exact \sef\@ $F_g$ given access to the approximate $\tilde
F_g$ constructed from $\tilde L$.
Then, in \cref{lem:spectral-bef-pert}, we bound the estimation
error for $\nabla \tilde F_g$.
Finally in \cref{thm:BEF-spectral-pert-full}, we use the error
analysis of the gradient iteration algorithm
(\cref{cor:robust-all-recovery-error-version}) to provide an
error analysis of BEF-based spectral clustering.

\begin{construction}[Perturbed and Exact BEFs for Spectral Clustering]\label{constr:BEF-spectral-pert-exact-Fg}
  We use the notation of \cref{sec:spectral-laplacian-pert}.
  In particular, $G$ is an $\dn$-vertex graph consisting
  of $\edim$-connected components with vertices in the index sets
  $\SS_1, \dotsc, \SS_\edim$ respectively; $L = D - A$ is the
  graph Laplacian constructed from $G$; $\tilde L = L +
  H$ is the graph Laplacian of a graph $\tilde G$ with identical
  vertices to $G$, but with similarity matrix $\tilde A$ considered to
  be a perturbation of $A$; and the eigengap $\mygap(L) = \lambda_{\edim + 1}(L) -
  \lambda_\edim(L)$ is such that $\norm H < \mygap(L)$.

  Let $\tilde X \in \R^{\dn \times \edim}$ be such that its columns
  are the lowest $\edim$ eigenvectors of $\tilde L$, scaled such that
  each column satisfies $\norm{\tilde x_{\vecdot i}} = \sqrt \dn$.
  Let $X$ be as in \cref{thm:pert-simplex-embedding}.
  The function $F_g$ and its approximation $\tilde F_g$ are
  defined as $F_g(\vec u) := \frac 1 \dn \sum_{i = 1}^\dn
  g(\abs{\ipCanonical{\vec u}{x_{i\vecdot}}})$ and $\tilde F_g(\vec u)
  := \frac 1 \dn \sum_{i = 1}^\dn g(\abs{\ipCanonical{\vec u}{\tilde
      x_{i\vecdot}}})$ respectively.
\end{construction}
  
\begin{lem}\label{lem:spectral-bef-pert}
  Under \cref{constr:BEF-spectral-pert-exact-Fg}, we let
  $E \geq 0$ be a fixed constant, we suppose that $\norm H \leq
  \mygap(L) \min(\frac 1 2, \frac E {\sqrt \dn})$,
  and we suppose that $g$ is $(\alpha, \beta, \delta, \gamma)$-robust.
  Then, there exists a universal constant $C > 0$ such that for all
  $\vec u \in \overline{\ball(0, 1)}$,
  \begin{displaymath}
    \norm{\nabla \tilde F_g(\vec u) - \nabla F_g(\vec u)}
    \leq C \alpha (1 + \frac 1 \gamma) \sqrt \edim [\frac 1 {\sqrt{\wmin}} + 4E]^{1 + 2\gamma} \frac {\norm H}{\mygap(L)} \ . \qedhere
  \end{displaymath}
  % \begin{displaymath}
  %   \norm{\nabla \tilde F(\vec u) - \nabla F(\vec u)}
  %   \leq C \alpha (1 + \frac 1 \gamma) \frac {E \sqrt \edim}{\sqrt \dn}[\frac 1 {\sqrt {\wmin}} + 4E]^{1 + 2\gamma} \ .
  % \end{displaymath}
\end{lem}
\begin{proof}
  We expand the formula $\norm{\nabla \tilde F_g(\vec u) - \nabla F_g(\vec u)}$ to obtain:
  \begin{align} \label{eq:spectral-gradf-error-expansion}
    &\norm{\nabla \tilde F_g(\vec u) - \nabla F_g(\vec u)}
    = \frac 1 \dn \biggr\lVert \sum_{i = 1}^\dn \left[g'(\ipCanonical{\tilde x_{i \vecdot}}{\vec u}) \tilde x_{i \vecdot} - g'(\ipCanonical{x_{i \vecdot}}{\vec u}) x_{i \vecdot}  \right] \biggr\rVert \nonumber \\
    &\qquad= \frac 1 \dn \biggr\lVert \sum_{i = 1}^\dn \Big[
      g'(\ipCanonical{\tilde x_{i \vecdot}}{\vec u})[\tilde x_{i \vecdot} - x_{i \vecdot}] 
      + [g'(\ipCanonical{\tilde x_{i \vecdot}}{\vec u}) - g'(\ipCanonical{x_{i \vecdot}}{\vec u})] x_{i \vecdot}
      \Big] \biggr\rVert \nonumber \\
    &\qquad\leq \frac 1 \dn \sum_{i=1}^\dn \abs{g'(\ipCanonical{\tilde x_{i \vecdot}}{\vec u})} \cdot \norm{\tilde x_{i \vecdot} - x_{i \vecdot}}
      + \frac 1 \dn \sum_{i=1}^\dn \frac 1 {\sqrt {w_{\min}}} \abs{g'( \ipCanonical{\tilde x_{i \vecdot}}{\vec u}) - g'(\ipCanonical{x_{i\vecdot}}{\vec u})} \ ,
  \end{align}
  by using that for any $i \in \SS_j$, $\norm{x_{i \vecdot}} = \frac 1
  {\sqrt{w_j}} \leq \frac 1 {\sqrt {w_{\min}}}$ (see
  \cref{prop:discrete-simplex}). 
  % and \cref{constr:spectral-Fg-L}).
  We now bound the individual terms in
  \cref{eq:spectral-gradf-error-expansion}.
  We first bound $\frac 1 \dn \sum_{i = 1}^\dn \norm{\tilde x_{i \vecdot} -
    x_{i \vecdot}}$ and the closely related $\frac 1 \dn \sum_{i = 1}^\dn
  \abs{\ipCanonical{(\tilde x_{i \vecdot} - x_{i \vecdot})}{\vec u}}$.
  By Jensen's inequality, 
  \begin{equation}\label{eq:X-pert-Jensen-bound}
    (\frac 1 \dn \sum_{i = 1}^\dn \abs{\ipCanonical{(\tilde x_{i \vecdot} - x_{i \vecdot})}{\vec u}})^2
    \leq \frac 1 \dn \sum_{i=1}^\dn \ipCanonicalp{(\tilde x_{i \vecdot} - x_{i \vecdot})}{\vec u}^2 \ .
  \end{equation}
  % \begin{displaymath}
  %   (\frac 1 \dn \sum_{i = 1}^\dn \norm{\tilde x_{i \vecdot} - x_{i \vecdot}})^2
  %   \leq \frac 1 \dn \sum_{i=1}^\dn \norm{\tilde x_{i \vecdot} - x_{i \vecdot}}^2
  %   = \frac 1 \dn \norm[F]{\tilde X - X}^2
  %   \leq \frac 1 \dn \norm{\tilde X - X}^2 \edim \ .
  % \end{displaymath}
  In order to compress notation, we define $\epsilon := \frac{2 \norm H}{\mygap(L) - \norm H}$.
  Applying \cref{rmk:pert-simplex-embedding} to \cref{eq:X-pert-Jensen-bound}, we obtain
  \begin{equation}\label{eq:spectral-bef-pert:1}
    \frac 1 \dn \sum_{i = 1}^\dn \abs{\ipCanonical{(\tilde x_{i \vecdot} - x_{i \vecdot})}{\vec u}}
    \leq \epsilon \ .
    % \qquad\qquad \text{and} \\
    % \frac 1 \dn \sum_{i = 1}^\dn \norm{\tilde x_{i \vecdot} - x_{i \vecdot}}
    % & %\leq \frac{ \sqrt \edim} {\sqrt \dn} \norm{\tilde X - X}
    % \leq \frac 1 \dn \Big(\sum_{i = 1}^\dn \sum_{j=1}^\edim \ipCanonicalp{(\tilde x_{i\vecdot} - x_{i \vecdot})}{\vec e_j}^2\Big)^{1/2}
    % \leq \frac{\sqrt \edim}{\sqrt \dn} \epsilon \ .
  \end{equation}
  By similar reasoning, we see that $(\frac 1 \dn \sum_{i = 1}^\dn
  \norm{\tilde x_{i \vecdot} - x_{i \vecdot}})^2 \leq \frac 1 \dn
  \sum_{i=1}^\dn \norm{\tilde x_{i \vecdot} - x_{i \vecdot}}^2 \leq
  \epsilon^2 \edim$, and hence
  \begin{equation}\label{eq:spectral-bef-pert:2}
    \frac 1 \dn \sum_{i = 1}^\dn \norm{\tilde x_{i \vecdot} - x_{i \vecdot}}
    \leq \epsilon\sqrt \edim \ .
  \end{equation}

  We now bound the second summand in \cref{eq:spectral-gradf-error-expansion}.
  By the mean value theorem, for all $i \in [\dn]$ there exists $c_i$ between $\ipCanonical{\tilde x_{i \vecdot}}{\vec u}$ and $\ipCanonical{x_{i \vecdot}}{\vec u}$ such that
  \begin{align*}
    \frac 1 \dn \sum_{i=1}^\dn \frac 1 {\sqrt {w_{\min}}} \abs{g'( \ipCanonical{\tilde x_{i \vecdot}}{\vec u}) - g'(\ipCanonical{x_{i\vecdot}}{\vec u})}
    &= \frac 1 {\dn} \sum_{i = 1}^\dn \frac 1 {\sqrt {\wmin}} \abs{g''(c_i)\ipCanonicalp{(\tilde x_{i\vecdot} - x_{i \vecdot})}{\vec u}} \ .
  \end{align*}
  By \cref{eq:spectral-bef-pert:1}, it follows that 
  \begin{displaymath}
    \frac 1 \dn \sum_{i=1}^\dn \frac 1 {\sqrt {w_{\min}}} \abs{g'( \ipCanonical{\tilde x_{i \vecdot}}{\vec u}) - g'(\ipCanonical{x_{i\vecdot}}{\vec u})}
    \leq \frac \epsilon  {\sqrt {\wmin}} \max_{i \in [\dn]} \abs{g''(c_i)} \ .
  \end{displaymath}
  By \cref{thm:pert-simplex-embedding}, we obtain
  \begin{math}
    \norm{\tilde x_{i \vecdot}} 
    \leq \norm{x_{i \vecdot}} + \norm{\tilde x_{i \vecdot} - x_{i \vecdot}}
    \leq \frac 1 {\sqrt {\wmin}} + \epsilon \sqrt \dn .
  \end{math}
  As such, for all $i \in [\dn]$, $\abs{c_i} \leq \frac 1 {\sqrt{\wmin}} + \epsilon\sqrt \dn$.
  Applying \cref{lem:F-robust-implications}, we see that
  \begin{math}
    \abs{g''(c_i)}
    \leq 2(2+\frac 1 \gamma)\alpha (\frac 1 {\sqrt {\wmin}} + \epsilon\sqrt \dn)^{2\gamma} .
  \end{math}
  The second summand of \cref{eq:spectral-gradf-error-expansion} can be bounded as
  \begin{equation}\label{eq:spectral-bef-pert:summand2}
    \frac 1 \dn \sum_{i=1}^\dn \frac 1 {\sqrt {w_{\min}}} \abs{g'( \ipCanonical{\tilde x_{i \vecdot}}{\vec u}) - g'(\ipCanonical{x_{i\vecdot}}{\vec u})}
    \leq 2(2+\frac 1 \gamma)\alpha (\frac 1 {\sqrt {\wmin}} + \epsilon\sqrt \dn)^{2\gamma} \frac{\epsilon}{\sqrt{\wmin}} \ .
  \end{equation}

  We now bound the first summand of \cref{eq:spectral-gradf-error-expansion}.
  We note that each
  \begin{math}
    \abs{\ipCanonical{\tilde x_{i \vecdot}}{\vec u}}
    \leq \norm{\tilde x_{i\vecdot}}
    \leq \frac 1 {\sqrt {\wmin}} + \epsilon \sqrt \dn .
  \end{math}
  Using \cref{lem:F-robust-implications}, we thus obtain that
  \begin{displaymath} 
    \abs{g'(\ipCanonical{\tilde x_{i \vecdot}}{\vec u})}
    \leq 2 \frac \alpha \gamma (\frac 1 {\sqrt{w_{\min}}} + \epsilon \sqrt \dn)^{1 + 2\gamma}
  \end{displaymath}
  for all $i \in [\dn]$.
  % Further, using \cref{eq:spectral-bef-pert:1}, we see that
  % \begin{displaymath}
  %   \frac 1 \dn \sum_{i=1}^\dn \norm{\tilde x_{i \vecdot} - x_{i \vecdot}}
  %   = \Big(\frac 1 \dn \sum_{i = 1}^\dn \sum_{j=1}^\edim \abs{\ipCanonical{(\tilde x_{i \vecdot} - x_{i \vecdot})}{\vec u}} \Big)^{1/2}
  %   \leq \frac {\sqrt \edim}{\sqrt \dn} \epsilon .
  % \end{displaymath}
  Combining this with \cref{eq:spectral-bef-pert:2}, we see
  that the first summand of
  \cref{eq:spectral-gradf-error-expansion} is bounded as
  \begin{equation}
    \label{eq:spectral-gradf-error-expansoin:1-1}
    \frac 1 \dn \sum_{i=1}^\dn \abs{g'(\ipCanonical{\tilde x_{i \vecdot}}{\vec u})} \cdot \norm{\tilde x_{i \vecdot} - x_{i \vecdot}}
    \leq 2\frac \alpha \gamma [\frac 1 {\sqrt {\wmin}} + \epsilon \sqrt \dn]^{1+2\gamma}  \epsilon \sqrt \edim
  \end{equation}
  From \cref{eq:spectral-gradf-error-expansion,eq:spectral-bef-pert:summand2,eq:spectral-gradf-error-expansoin:1-1}, we obtain a full error bound:
  \begin{align*}
    &\norm {\nabla \tilde F_g(\vec u) - \nabla F_g(\vec u)} \\
    &\qquad\leq 2 \frac \alpha \gamma [\frac 1 {\sqrt {\wmin}} + \epsilon \sqrt \dn]^{1+2\gamma} \epsilon \sqrt \edim
      + 2 (2+\frac 1 \gamma)\alpha (\frac 1 {\sqrt {\wmin}} + \epsilon\sqrt \dn)^{2\gamma} \frac \epsilon {\sqrt{\wmin}} \ .
  \end{align*}

  Expanding $\epsilon$ and using the assumed bound on $\norm H$, we see that
  \begin{displaymath}
    \epsilon 
    = \frac{2 \norm H}{\mygap(L) - \norm H}
    \leq \frac {4 \norm H}{\delta (L)}
    \leq \frac {4E}{\sqrt \dn} \ .
  \end{displaymath}
  It follows that for some universal constant $C > 0$,
  \begin{displaymath}
    \norm{\nabla \tilde F_g(\vec u) - \nabla F_g(\vec u)}
    \leq C \alpha (1 + \frac 1 \gamma) \sqrt \edim [\frac 1 {\sqrt{\wmin}} + 4E]^{1 + 2\gamma} \frac {\norm H}{\mygap(L)} \ . \qedhere
  \end{displaymath}
  % \begin{displaymath}
  %   \norm{\nabla \tilde F_g(\vec u) - \nabla F_g(\vec u)}
  %   \leq C \alpha (1 + \frac 1 \gamma) \frac {E \sqrt \edim}{\sqrt \dn}[\frac 1 {\sqrt{\wmin}} + 4E]^{1 + 2\gamma} \ . \qedhere
  % \end{displaymath}
\end{proof}

\begin{algorithm}[tbh]
  \caption[Robust spectral clustering algorithm]{
    A robust algorithm for spectral clustering.
  }\label{alg:spectral-robust}
  \begin{algorithmic}[1]
    \Function{RobustSpectralClustering}{$\tilde A$, $g'$, $k$, $\sigma$, $N_1$, $N_2$, $I$}
      \State Construct the graph Laplacian $\tilde L$ from $\tilde A$.
      \State Construct $\tilde X = (\tilde x_{\vecdot 1}, \dotsc, \tilde x_{\vecdot \edim})$ such that each $\tilde x_{\vecdot i}$ is the $i$\textsuperscript{th} lowest eigenvector \newline \phantom{.} $\qquad$ of $\tilde L$ scaled such that $\norm{\tilde x_{\vecdot \edim}} = \sqrt \dn$.
      \State Define the function pointer $dF_g(\vec u) := \frac 1 \dn \sum_{i=1}^\dn g'(\ipCanonical{\vec u}{\tilde x_{i \vecdot}}) x_{i \vecdot}^T$.
      \State\label{alg:robust-spectral:step:robust-gi}
      $\tilde \myZv_1, \dotsc, \tilde \myZv_\edim \leftarrow \textsc{RobustGI-Recovery}$($k$, $\sigma$, $dF_g$, $N_1$, $N_2$, $I$).
      \State
      \State // Initialize the clusters
      \For {$j \leftarrow 1$ to $\edim$}
        \State $\tilde \SS_j \leftarrow \emptyset$
      \EndFor
      \State
      \State // Assign cluster labels to graph vertices.
      \For {$i \leftarrow 1$ to $\dn$}
        \State $j \leftarrow \argmax_\ell \abs{\ipCanonical {\tilde \myZv_\ell}{x_{i \vecdot}}}$.
        \State $\tilde \SS_j \leftarrow \tilde \SS_j \cup \{i\}$
      \EndFor
      \State \Return $\tilde \SS_1, \dotsc, \tilde \SS_\edim$.
    \EndFunction
  \end{algorithmic}
\end{algorithm}


For simplicity, we proceed in analyzing spectral clustering using the families of contrasts $g_{p,{\tabs}}(t) := \frac{1}{p(p+1)} \abs{t}^{2(p+1)}$ and  $g_{p,{\sign}}(t) := \frac{\sign(t)}{p(p+1)} \abs{t}^{2(p+1)}$ for all real $p > 0$.
It can be verified that these contrast functions are $(1, 1, p, p)$ robust.
For clarity, we will denote by $C_0, C_1, C_2, \dotsc$ positive universal constants in the main theorem statements.
These can represent different constant values in different theorem statements.
\begin{thm}[Full spectral perturbation analysis]\label{thm:BEF-spectral-pert-full}
  In \cref{constr:BEF-spectral-pert-exact-Fg}, we suppose that $g$ is a $(1, 1, p, p)$-robust function on the domain $[- \frac 1 {\sqrt {\wmin}}, \frac 1 {\sqrt {\wmin}} ]$.
  We suppose that $\sigma \leq C_0 \cdot  16^{-\frac 1 p}(1+p)^{-\frac 1 2} \cdot \frac \wmin \wmax \edim^{-\frac 3 2}$ and that
  \begin{displaymath}
    \norm H
    \leq \min\Big( \frac 1 2,\ C_1(\dn \wmax)^{-\frac 1 2},\
    C_2 \frac{\sigma \sqrt{\wmin}(\frac \wmin \wmax)^{3p + \frac 7 2}}{2^{\frac 8 p + 2p}(p+1)\edim^{2p + \frac 7 2}}\Big) \mygap(L)\ .
  \end{displaymath}
  Fix any $\delta \in (0, 1)$.
  Suppose that $I \geq C_3 \edim\lceil \log(\edim / \delta)\rceil$,
  $N_1 \geq C_4
  \Big\lceil \log_{1+2p}\big[(\frac 8 p + 2p + 4)(1+\log_2(\frac {k \wmax}{\sigma \wmin})) \big]\Big\rceil$, 
  and $N_2 \geq C_5
  \Big\lceil 16^{\frac 1 p} \sigma^{-1} ( \frac{\wmax}{\wmin} )^{p + 2}
  \edim^{\frac 5 2} \big[ \log( \frac {\wmax}{\wmin} ) + \log(k)
  \big]\Big\rceil + N_1$.
  Then with probability at least $1-\delta$,
  \textsc{RobustSpectralClustering}($\tilde A, g', k, \sigma, N_1,
  N_2, I$) partitions $\tilde G$ according to the components of $G$ in
  $(N_1 + IN_2)\poly(\edim, \dn)$ time.
\end{thm}

The proof of \cref{thm:BEF-spectral-pert-full} relies on the
perturbation analysis of the gradient iteration algorithm from
\cref{cor:robust-all-recovery-error-version}.
For easier reference, we rewrite this corollary using the notation of
spectral clustering.
\begin{lem}[\Cref{cor:robust-all-recovery-error-version} restated for spectral clustering]\label{lem:cor-gi-robust-spectral-version} 
  In \cref{constr:BEF-spectral-pert-exact-Fg}, we suppose
  that $F_g$ is $(\frac 1 {\wmin^p}, \frac 1
  {\wmax^p}, p, p)$-robust.
  Suppose also that
  \begin{itemize}
  \item $\sigma \leq C_0\Big(16^{-\frac 1 p}(1+p)^{-\frac 1 2} \cdot \frac \wmin \wmax \edim^{-3/2}\Big)$,
  \item $\eta \leq C_1\Big(2^{-\frac 8 p}(\frac{\wmin}{\wmax})^{2p+\frac 7 2} \edim^{-2p-4} \sigma \Big)$,
  \item $N_1 \geq C_2 \Big\lceil \log_{1+2p}\log_2(\frac 1 \eta) \Big\rceil$, and
  \item $N_2 \geq C_3 \Big\lceil
    16^{\frac 1 p} \sigma^{-1} ( \frac{\wmax}{\wmin} )^{p + 2} \edim^{\frac 5 2} 
    \big[ \log( \frac {\wmax}{\wmin} ) + \log(k) \big]\Big\rceil
    + C_2\Big\lceil \log_{1+2p}\log_2(\frac 1 \eta) \Big\rceil$.
  \end{itemize}
  Let $\delta \in (0, 1)$, and suppose $I \geq C_4\edim \lceil\log (\edim/\delta)\rceil$.
  If $\nabla \tilde F_g$ is a $C_5 \frac \eta {p \wmax^{p}}$-approximation to $\nabla F_g$ and if we execute
  $\tilde \myZv_1, \dotsc, \tilde \myZv_\edim \leftarrow \textsc{RobustGI-Recovery}(\edim, \sigma, \nabla \tilde F_g, N_1, N_2, I)$,
  then with probability at least $1-\delta$, $\tilde \myZv_1, \dotsc, \tilde \myZv_\edim$ is an $\eta$-recovery of $\myZv_1, \dotsc, \myZv_\edim$.
\end{lem}

% \begin{thm}[\cref{cor:robust-all-recovery-error-version} restated for spectral clustering]\label{thm:cor-gi-robust-spectral-version}
%   In \cref{constr:BEF-spectral-pert-exact-Fg}, we suppose
%   that $F_g$ is $(\frac \alpha {\wmin^\gamma}, \frac \beta
%   {\wmax^\delta}, \gamma, \delta)$-robust.
%   Treating $\gamma$ and $\delta$ as fixed constants, we suppose that
%   $\sigma \leq \poly^{-1}(\edim, \frac {\wmax^\delta}{\wmin^\gamma}, \frac \alpha \beta)$, 
%   $\eta \leq \poly^{-1}(\edim, \frac {\wmax^\delta}{\wmin^\gamma}, \frac \alpha \beta)\sigma$,
%   $N_1 \geq O\big( \log \log(\frac 1 \eta) \big)$, 
%   and $N_2 \geq \poly(\frac \alpha \beta, \frac {\wmax^\delta}{\wmin^\gamma}, \edim)\sigma^{-1} + O\big( \log\log(\frac 1 \eta) \big)$.
%   Let $p \in (0, 1)$, and suppose that $I \geq O(\edim \log (k/p))$.
%   If $\nabla \tilde F_g$ is a $O(\frac \beta {\wmax^\delta}
%   \eta)$-approximation to $\nabla F_g$ and if we execute
%   $\tilde \myZv_1, \dotsc, \tilde \myZv_\edim \leftarrow \textsc{RobustGI-Recovery}(\edim, \sigma, \nabla \tilde F_g)$
%   (implemented with these choices of $N_1$, $N_2$, and $I$), then with
%   probability at least $1-p$ there exists $\pi$ a permutation of
%   $[\edim]$ and signs $s_1, \dotsc, s_\edim$ such that $\norm{\myZv_i
%     - s_i \tilde \myZv_{\pi(i)}} \leq \eta$ for all $i \in [\edim]$.
% \end{thm}

\begin{proof}[\proofword of \cref{thm:BEF-spectral-pert-full}]
  We will require that $C_1 \leq \frac 1 4$ so that $\norm{H} \leq \frac 1 4
  (\dn \wmax)^{- \frac 1 2}$.
  Then, we apply \cref{lem:spectral-bef-pert} (with the constant $E=\frac
  1 {4\sqrt {\wmax}}$ in that Lemma) to obtain that for all $\vec u \in \overline {B(0, 1)}$,
  \begin{align*}
    \norm{\nabla \tilde F(\vec u) - \nabla F(\vec u)}
    &\leq 
    O\left( (1+1 / p) (\frac 1 {\sqrt {\wmin}} + \frac 1 {\sqrt{\wmax}})^{1+2p}  \edim^{- \frac 1 2 } \frac {\norm H}{\mygap(L)} \right) \\
    &\leq O\left( 2^{2p}\Big(\frac{p+1} p\Big) \wmin^{-\frac 1 2 - p}  \edim^{- \frac 1 2 } \frac {\norm H}{\mygap(L)} \right)\ ,
  \end{align*}
  using that $\frac 1 {\sqrt {\wmax}} \leq \frac 1 {\sqrt {\wmin}}$ in the
  final inequality.
  Further, by the given bound on $\norm H$, $\nabla \tilde F_g$ is an
  \begin{equation}\label{eq:4}
    O\left(2^{-\frac 8 p} p^{-1} \wmin^{-p} \Big(\frac \wmin \wmax\Big)^{3p + \frac 7 2} \edim^{-2p-4} \sigma \right)
  \end{equation}
  approximation to $\nabla F_g$.
  We set $\eta$ to be $p \wmax^p$ times \cref{eq:4} to obtain that
  $\nabla \tilde F_g$ is an $O(\frac{\eta}{p \wmax^p})$-approximation to
  $\nabla F_g$.
  Further,
  \begin{equation}\label{eq:5}
\eta \leq O(2^{-\frac 8 p} \big(\frac \wmin \wmax\big)^{2p + \frac
    7 2} \edim^{-2p - 4}\sigma) \ .
  \end{equation}

  By \cref{lem:fg-spectral-robust}, $\nabla \tilde F_g$ is a $(\frac 1
  {\wmin^p}, \frac 1 {\wmax^p}, p, p)$-approximation to $\nabla F_g$.
  Further, it can be verified that $N_1 \geq \log_{1+2p}(\log_2(1/\eta))$.
  Combining these facts, we may apply
  \cref{lem:cor-gi-robust-spectral-version} to see that at the end of the
  execution of line~\ref{alg:robust-spectral:step:robust-gi} of
  \textsc{RobustSpectralClustering}, then with probability at least $1-\delta$
  $\tilde \myZv_1, \dotsc, \tilde \myZv_\edim$ is an $\eta$-recovery of $\myZv_1, \dotsc, \myZv_\edim$.
  
  We assume without loss of generality\footnote{%
    We may do this since the ordering and sign associated with the $\pm
    \myZv_i$ hidden basis directions are a matter of convention.}
  that $\norm{\tilde \myZv_i - \myZv_i} \leq
  \eta$ for all $i \in [\edim]$.
  To complete the proof, we will need the following claim.
  \begin{claim}\label{claim:correct-clustering-criterion}
    If $\frac{2\norm H \sqrt \dn}{\mygap(L) - \norm H} + \frac 1 {\sqrt {\wmin}} \max_j
    \norm{\tilde \myZv_j - \myZv_j} < \frac 1 {2 \sqrt{\wmax}}$, then
    \textsc{RobustSpectralClustering} clusters the vertices of $\tilde
    G$ according to the connected components of $G$.
  \end{claim}
  \begin{subproof}
    In order to simplify notation, we define $\epsilon_0 := \frac{2\norm
      H}{\mygap(L) - \norm H}$ to be the constant from
    \cref{thm:pert-simplex-embedding}.
    % We note that this may be bounded as $\epsilon_0 = O(\frac{\norm
    %   H}{\mygap(L)})$ by the assumption that $\norm H \leq \frac 1 2
    % \mygap(L)$.

    For all $i \in [\dn]$ and all $j \in [\edim]$, it follows (using the notation from \cref{constr:BEF-spectral-pert-exact-Fg}) that
    \begin{align}\label{eq:spectralError-1}
      \abs{\ipCanonical{\tilde x_{i \vecdot}}{\tilde \myZv_j} - \ipCanonical{x_{i \vecdot}}{\myZv_j}}
        &= \abs{
          \ipCanonical{(\tilde x_{i \vecdot} - x_{i \vecdot})}{\tilde \myZv_j} +
          \ipCanonical{x_{i \vecdot}}{(\tilde \myZv_j - \myZv_j)}
        }  \nonumber \\
        &\leq \abs{\ipCanonical{(\tilde x_{i \vecdot} - x_{i \vecdot})}{\tilde \myZv_j}} +
        \norm{x_{i\vecdot}} \cdot \norm{\tilde \myZv_j - \myZv_j} \nonumber \\
        &\leq \epsilon_0 \sqrt \dn + \frac 1 {\sqrt{\wmin}} \cdot \norm{\tilde \myZv_j - \myZv_j} \ ,
    \end{align}
    where the first term in the final inequality is bounded using
    \cref{thm:pert-simplex-embedding}, and the second term is
    bounded using \cref{prop:discrete-simplex}.
    Also by \cref{prop:discrete-simplex},
    $\ipCanonical{x_{i\vecdot}}{\myZv_j} = \indicator{i \in
      \SS_j}\frac 1 {\sqrt{w_j}}$.
    We proceed from \cref{eq:spectralError-1} in two cases.
    In the case where $i \in \SS_j$,
    \begin{displaymath}
      \abs{\ipCanonical{\tilde x_{i \vecdot}}{\tilde \myZv_j} - \frac 1 {\sqrt{w_j}}}
      \leq \epsilon_0 \sqrt \dn + \frac 1 {\sqrt{\wmin}} \cdot \norm{\tilde \myZv_j - \myZv_j} \notag      
    \end{displaymath}
  and hence,
    \begin{align}\label{eq:spectralError-2}
      \abs{\ipCanonical{\tilde x_{i \vecdot}}{\tilde \myZv_j}}
      &\geq \frac 1 {\sqrt{w_j}} - \epsilon_0 \sqrt \dn - \frac 1 {\sqrt{\wmin}} \cdot \norm{\tilde \myZv_j - \myZv_j} \nonumber \\
      &\geq \frac 1 {\sqrt{\wmax}} - \epsilon_0 \sqrt \dn - \frac 1 {\sqrt{\wmin}} \cdot \norm{\tilde \myZv_j - \myZv_j} \ .
    \end{align}

    In the case where $i \not \in \SS_j$, we obtain
    \begin{equation}
      \label{eq:spectralError-3}
      \abs{\ipCanonical{\tilde x_{i \vecdot}}{\tilde \myZv_j}}
      \leq \epsilon_0 \sqrt \dn + \frac 1 {\sqrt{\wmin}} \cdot \norm{\tilde \myZv_j - \myZv_j} \ .
    \end{equation}

    The $i$\textsuperscript{th} vertex is correctly clustered if for
    that choice of $i$, the right hand side (r.h.s.\@) of
    \cref{eq:spectralError-2} with $i \in \SS_j$ exceeds the
    r.h.s.\@ of \cref{eq:spectralError-3} for all
    other choices of $j$.
    It suffices that the smallest obtainable value for the r.h.s.\@ of \cref{eq:spectralError-2} exceeds the largest obtainable value for the r.h.s.\@ of \cref{eq:spectralError-3}, i.e.\@ $\frac 1 {\sqrt {\wmax}} - \epsilon_0 \sqrt
    \dn - \frac 1 {\sqrt{\wmin}} \max_{j \in [\edim]}\norm{\tilde \myZv_j - \myZv_j}
    > \epsilon_0 \sqrt \dn + \frac 1 {\sqrt{\wmin}} \max_{j \in [\edim]} \norm{\tilde \myZv_\ell - \myZv_\ell}$.
    In particular, it suffices that $\epsilon_0 \sqrt \dn + \frac
    1 {\sqrt{\wmin}} \cdot \max_{j} \norm{\tilde \myZv_j - \myZv_j} <
    \frac 1 {2 \sqrt {\wmax}}$.
  \end{subproof}
  To complete the proof, we bound the terms in the inequality from \cref{claim:correct-clustering-criterion}.
  First, we note that
  \begin{displaymath}
    \frac{2\norm H \sqrt \dn}{\mygap(L) - \norm H}
    \leq O(\frac{\norm H}{\mygap(L)} \sqrt \dn)
    \leq O(\frac 1 {\sqrt{\wmax}}) \ ,
  \end{displaymath}
  where the first inequality uses the given bound $\norm H \leq \frac 1 2 \mygap(L)$ to see that the denominator is at least $\frac 1 2 \mygap(L)$, and the second inequality uses the given bound $\norm H \leq O(n \wmax)^{-\frac 1 2} \mygap(L)$.
  We also note that
  \begin{align*}
    \frac 1 {\sqrt {\wmin}} \max_j \norm{\tilde \myZv_j - \myZv_j}
    &\leq \frac \eta {\sqrt {\wmin}}
    \leq \frac 1 {\sqrt{\wmin}}O\left(2^{-\frac 8 p}\bigr(\frac \wmin \wmax\bigr)^{2p+\frac 7 2}\edim^{-2p-4}\sigma\right) \\
    &\leq \frac 1 {\sqrt{\wmin}}O\left(2^{-\frac {12} p}(1+p)^{-\frac 1 2} \bigr(\frac \wmin \wmax \bigr)^{2p+\frac 9 2} \edim^{-2p - \frac{11}{2}}\right)  \\
    &\leq O\left(\frac 1 {\sqrt{\wmax}}\right) \ .
  \end{align*}
  As such, applying \cref{claim:correct-clustering-criterion} completes the proof.
\end{proof}
\def\dn{\dnold}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> spectral-error-analysis.tex <==
\def\myL{L}
\def\mygap{\delta_\edim}
\def\edim{\ensuremath{k}}
\def\AppendixLabel{Appendix}
\def\wmin{\ensuremath{w_{\mathrm{min}}}}
\def\wmax{\ensuremath{w_{\mathrm{max}}}}
\def\tabs{\mathrm{abs}}
\def\dnold{\dn}
\def\dn{n}
\section{Perturbation Analysis of Spectral Clustering}
\label{sec:spectral-pert-analysis}

We now revisit the spectral clustering method introduced in \cref{sec:example-befs} for performing multi-way clustering of vertices within a graph.
First, in \cref{sec:Laplacian-structure} we briefly describe the structure of the spectral embedding, and note that it leads to a basis recovery problem when working with graphs consisting of $\edim$ connected components.
Then, in \cref{sec:spectral-laplacian-pert,sec:pert-analys-clust}, we show that under a perturbation from the setting of $\edim$ connected components, we are able to recover the underlying clusters using our {\sef} framework.

\subsection{\Sef\@ Structure of the Spectral Embedding}
\label{sec:Laplacian-structure}

We consider an undirected graph $G$ with non-negative edge weights.
The goal in graph clustering is to partition the vertices of $G$ into sets which are internally well connected.
Spectral clustering is commonly used for performing such a clustering.

Spectral clustering proceeds in two steps.
When looking for $\edim$ clusters, the vertices of $G$ are first
embedded into $\R^\edim$ using a process called the \emph{Laplacian
embedding}.
Then, the resulting embedded vertices are clustered within $\R^\edim$ typically using a clustering algorithm defined in Euclidean space such as $k$-means.
Interestingly, when $G$ consists of $\edim$ connected components, the Laplacian embedding induces an orthogonality structure upon the embedded vertices that allows us to construct \ansef\@ with which to perform the clustering. 

To define the Lablacian embedding, we must first introduce some notations.
We denote by $A$ the adjacency matrix of our graph $G$, i.e.\@ $A_{ij}$ is the
weight of the edge connecting vertices $i$ and $j$ if an edge is present and 0
if no edge is present.
We denote by $D$ the diagonal matrix with its $i$\textsuperscript{th} diagonal
entry being the degree of the $i$\textsuperscript{th} vertex, i.e., $D_{ii} :=
\sum_{j} A_{ij}$.
The graph Laplacian is defined by $L := D - A$.

Throughout this section, we will make use of several properties of the graph Laplacian (see \cite{von2007tutorial} for an overview).
A perhaps more intuitive alternate definition of the graph Laplacian  is that for all $\vec x \in \R^\dn$, $\vec x^T L \vec x = \frac 1 2 \sum_{i, j} A_{ij}(x_i - x_j)^2$.
From this characterization, it can be demonstrated that $L$ is positive semi-definite, and that the multiplicity of its $0$ eigenvalue is the same as the number of connected components in $G$.
When $G$ consists of $\edim$ connected components, the Laplacian embedding into $\R^\edim$ is actually formed using the null space of the Laplacian.

In general, the Laplacian embedding is constructed as follows: We let
$X \in \R^{\dn \times \edim}$ be a matrix such that its columns $X =
[\vec x_{\vecdot 1}, \dotsc, \vec x_{\vecdot \edim}]$ are the lowest
$\edim$ eigenvectors of $L$ scaled such that $\norm{\vec x_{\vecdot
    i}} = \sqrt \dn$.
Then, the rows $\vec x_{1 \vecdot}, \dotsc, \vec x_{\dn \vecdot}$ of
$X$ are the embeddings of the $\dn$ vertices of $G$.

% As such, we have by definition that $A_{ij} = 0$ if $i \in S_k$, $j \in S_\ell$, and $k \neq \ell$.

% The degree matrix $D$ is a diagonal matrix with entries $D_{ii} = \sum_{j=1}^\dn A_{ij}$.

% The goal in graph clustering problem is to partition the vertices into sets which are internally well connected.
% One popular set of ideas for graph clustering is spectral clustering.
% Spectral clustering proceeds in two steps:
% \begin{enumerate}
% \item \emph{Laplacian Embedding.}
%   The graph Laplacian is defined by $L := D - A$.
%   Let $X$ be a matrix such that its columns are the bottom $\edim$ eigenvectors of $L$ scaled such that each column has $\sqrt \dn$-norm.
%   If we denote the rows of $X$ by $X = [\vec x_1^T, \dotsc, \vec x_\dn^T]^T$, then the $\vec x_1, \dotsc, \vec x_\dn$ form the embeddings for the vertices of the graph $G$.
% \item \emph{Clustering Step.}
%   Using the properties of the Laplacian embedding, it is assumed that the desired clusters within the graph are mapped to nice point clouds (natural clusters) in the embedded space $\R^\edim$.
%   A clustering algorithm is employed in the embedded space to recover the desired clusters.
% \end{enumerate}

% There are multiple ways of interpreting what spectral clustering accomplishes.
% Here, we start by noting that for a graph consisting of $\edim$ connected components, the spectral embedding takes on a very simple form in which each of the embedded points $\vec x_i$ from the same component are mapped to a single point forming very natural clusters.
% In the upcoming sections, we view the case of a fully connected graph $G$ (as seen in practice) as being a perturbation from the setting of $k$ connected components, and we show that we can recover the desired underlying clusters---i.e., the clusters corresponding to the $\edim$ connected components in the unperturbed graph---assuming that the perturbation is sufficiently small.
% We note that more generally, spectral clustering can also be viewed as a generalization of the NP hard multi-way ratio cut problem \citep[section 5]{von2007tutorial}.
%In particular, when $G$ consists of $\edim$ connected components, the Laplacian embedding takes on a very simple form.
%Further, a fully connected graph (i.e., one which arises in practice) can be viewed as a perturbation from 
%
%When the graph $G$ is fully connected, there are multiple ways of interpreting what this clustering process accomplishes.
%One intuitive goal of graph clustering is minimize certain normalized cuts induced by partitioning the graph into $\edim$ clusters.
%In particular, spectral clustering using the unnormalized graph Laplacian described can be viewed as a relaxation of the NP-hard problem of min ratio cut for a $\edim$-partitioning of the graph $G$ into clusters \citep[section 5]{von2007tutorial}.

The orthogonality structure of the Laplacian embedding is described by the following Lemma (adapted from \citep{BelkinRV14}).
\begin{lem}\label{prop:discrete-simplex}
  Suppose that the graph $G$ consists of $\edim$ connected components with corresponding index sets $S_1, \dotsc, S_\edim$.
  Suppose that $\vec x_1, \dotsc, \vec x_\dn \in \R^\edim$ are the embeddings the of vertices of $G$ under the Laplacian embedding.
  Then, there exists orthogonal unit vectors $\myZv_1, \dotsc, \myZv_\edim$ in $\R^\edim$ such that $\vec x_i = \sqrt{\dn/\abs{S_j}}\myZv_j$ for all $i \in S_j$.
\end{lem}

Using that the embedded vertices for each component of $G$ are orthogonal to each other, we are able to construct \ansef\@ from the embedded data as follows.
\begin{construction}\label{constr:spectral-Fg-L}
  We proceed under the assumptions and notation of \cref{prop:discrete-simplex}.
  Let $g : \R^\edim \rightarrow \R$ be a twice continuously differtiable function satisfying \crefrange{assumpt:first}{assumpt:last}.
  We define the function $F : \R^\edim \rightarrow \R$ by
  \begin{displaymath}
    F(\vec u) := \frac 1 \dn \sum_{i = 1}^\dn g(\ipCanonical{\vec u}{\vec x_i}) \ .
  \end{displaymath}
  By \cref{prop:discrete-simplex}, we see that for all $j \in [\edim]$, there $\abs{S_j}$ copies of the point $\sqrt{\dn / \abs{S_j}} \myZv_j$ among the embedded vertices.
  Defining $w_j := \abs{S_j} / {\dn}$, we may thus equivalently write:
  \begin{equation}\label{eq:f_weighted_form}
    F(\vec u) := \sum_{i = 1}^\edim w_j g(w_j^{-\frac 1 2} \ipCanonical{\vec u}{\myZv_i}) \ .
  \end{equation}
  We define coordinate functions $g_i : \R \rightarrow \R$ by $g_i(t) := w_j g(w_j^{- \frac 1 2} t)$.
  Then, we may write that $F(\vec u) = \sum_{i = 1}^\edim g_i(\ipCanonical{\vec u}{\myZv_i})$.
  As it may be verified that the coordinate functions also satisfy \crefrange{assumpt:first}{assumpt:last}, we obtain that $F$ is \ansef\@.
\end{construction}

When the graph $G$ consists of $\edim$ connected compoenents, the spectral embedding gives rise to \ansef\@.
As such, the gradient iteration algorithm (\cref{alg:gi-generic}) can be used to recover the underlying directions $\myZv_i$ up to sign.
If $\hat \myZv_i$ denote the recovered basis directions, then we may cluster the vertices of $G$ by assigning the $i$\textsuperscript{th} vertex to the cluster $\argmax_{j \in [\edim]} \abs{\ipCanonical{\vec x_i}{\hat \myZv_i}}$.

\subsection{Perturbation of the Spectral Embedding}\index{spectral embedding!perturbation}\label{sec:spectral-laplacian-pert}
We have now seen that when $G$ consists of $\edim$ connected components, the components can be recovered by making use of the \sef\@ structure of the Laplacian embedding described in \cref{prop:discrete-simplex,constr:spectral-Fg-L}.
However when performing spectral clustering, one typically observes a graph which is fully connected and tries to discover natural clusters in such a graph.
We now wish to demonstrate that when an observed graph has an adjacency matrix which is close to that of a ``clean'' graph consisting of $\edim$ connected components, then the clusters corresponding to the connected components in the clean graph can be recovered from the observed graph using spectral clustering.

Our analysis proceeds in two steps.
In this subsection, we analyze the Laplacian embedding induced by a perturbation from the setting of $\edim$ connected components.
This demonstrates that when we are close to the setting of $\edim$ connected components, the orthogonality structure of the Laplacian embedding from \cref{prop:discrete-simplex} is approximately preserved.
Then, in \cref{sec:pert-analys-clust} we apply our gradient iteration error analysis to demonstrate that \textsc{RobustGI-Recovery} (\cref{alg:FullRecovery}) can be employed to robustly recover the desired vertex clusters.

For the remainder of \cref{sec:spectral-pert-analysis}, we assume that $\myL
:= D - A$ is the graph Laplacian constructed from a graph $G$ consisting of
$\dn$ vertices arranged in $\edim$ connected components.
Let $\lambda_1(\myL) \leq \lambda_2(\myL) \leq \cdots \leq \lambda_\dn(\myL)$
denote the eigenvalues of $\myL$.
Under our assumptions, $0 = \lambda_1(\myL) = \lambda_2(\myL) =
\cdots = \lambda_\edim(\myL) < \lambda_{\edim + 1}(\myL)$ \citep[Proposition 2]{von2007tutorial}.
Throughout this section, we denote by $\mygap(\myL) = \lambda_{\edim+1}(\myL)
- \lambda_{\edim}(\myL)$ the eigengap between the null space of $\myL$
(denoted by $\NN(\myL)$) and the range of $\myL$ (denoted as $\RR(\myL)$).
We further assume that $\tilde G$ is a pertubed version of $G$ such that the
graph Laplacian $\tilde L$ constructed from $\tilde G$ satisfies $\tilde \myL
= \myL + H$ for some perturbation $H$.
By the construction, $\tilde L$, $L$, and $H$ are symmetric.
We obtain the following perturbation result for the spectral embedding.

\begin{thm} \label{thm:pert-simplex-embedding}
  Suppose that $\norm H < \mygap(L)$ and that
  $\tilde X = (\tilde x_{\vecdot 1}, \dotsc, \tilde x_{\vecdot \edim})$ contains the lowest $\edim$ eigenvectors of $\tilde \myL$ as its columns, scaled such that $\norm{\tilde x_{\vecdot i}} = \frac 1 {\sqrt \dn}$ for all $i \in [\edim]$.
  Then there exists $X = (x_{\vecdot 1}, \dotsc, x_{\vecdot \edim})$ with columns forming a scaled orthogonal basis of $\NN(\myL)$ such that each $\norm{x_{\vecdot i}} = \frac 1 {\sqrt \dn}$ and $\frac 1 {\sqrt \dn} \norm{X - \tilde X} \leq \frac{2 \norm H}{\mygap(\myL) - \norm H}$.
\end{thm}

\begin{rmk}\label{rmk:pert-simplex-embedding}
    In \cref{thm:pert-simplex-embedding}, the bound on $\frac 1 {\sqrt \dn}\norm{X - \tilde X}$ also implies:
  \begin{compactenum}
    \item If $\vec v \in \R^\edim$ is a unit vector, then $\frac 1 \dn \sum_{i=1}^\dn (\ipCanonicalp{\tilde x_{i \vecdot}}{\vec v} - \ipCanonicalp{ x_{i \vecdot}}{\vec v})^2 \leq \frac{4 \norm H^2}{(\mygap(\myL) - \norm H)^2}$.
    \item $\frac 1 \dn \sum_{i=1}^\dn \norm{\tilde x_{i \vecdot} - x_{i \vecdot}}^2 \leq \frac{4 \norm H^2 \edim}{(\mygap(\myL) - \norm{H})^2}$.
  \end{compactenum}
\end{rmk}

\Cref{thm:pert-simplex-embedding} implies that the
orthogonal basis structure from \cref{prop:discrete-simplex} 
is approximately preserved under a perturbation.
To see the sorts of assumptions under which $\norm H$ is small relative to the eigengap $\mygap(L)$, we refer the reader to the work of \mycitet{Ng et al.}{ng2002spectral}.
In their work, they analyze the spectral embedding quality of the symmetric normalized Laplacian $D^{-1/2}LD^{-1/2}$ under a similar perturbation.

We now proceed with the proof of \cref{thm:pert-simplex-embedding}.
The following Lemma is a direct implication of the $\sin \Theta$ theorem\index{sin $\Theta$ theorem} of  \mycitet{Davis and Kahan}{davis1970rotation}, which is reproduced in \cref{sec:error-bounds-eigenv} as \cref{thm:sin-theta-thm}.
\begin{lem}\label{lem:pert-sin-theta}
  Suppose that $\norm H < \mygap(L)$,
  that $X = (x_{\vecdot 1}, \dotsc, x_{\vecdot \edim})$ is an orthogonal basis of $\NN(\myL)$,
  and that $\tilde X = (x_{\vecdot 1}, \dotsc, x_{\vecdot \edim})$ are the bottom $\edim$ eigenvectors of $\tilde \myL$.
  Then, $\norm{P_{\NN(X)} P_{\RR(\tilde X)}} \leq \frac{\norm H}{\mygap(\myL) - \norm H}$.
\end{lem}

We now decompose the bound from \cref{lem:pert-sin-theta} in order to
write a bound in terms of the actual entries of $X$ and $\tilde X$.
This is complicated by the fact that $X$ is only meaningfully defined up to a
rotation of its columns within the subspace $\NN(\myL)$.
In \cref{lem:pert-sin-theta}, this is reflected by the fact that we are
bounding the change in the projection operators onto the subspaces spanned by
$X$ and $\tilde X$ rather than directly bounding the change in the
eigenvectors themselves.
Indeed, if $X$ and $Y$ contained two different bases of $\NN(\myL)$ in their
columns (with the columns of $X$ and $Y$ scaled to have $\sqrt \dn$-norm),
then $R = \frac 1 \dn X^T Y$ would be the rotation%
\footnote{For our purposes, a rotation matrix is an element of the general
  orthogonal group $O(k)$.
  In particular, we allow orthogonal matrices $R$ with
  determinant satisfying either $\det(R) = +1$ or $\det(R) = -1$.
}
matrix providing a transition between the coordinate systems of these two bases of $\NN(L)$.
If $X$ and $\tilde X$ are constructed from the $\edim$ lowest eigenvectors of
$\myL$ and its perturbation $\tilde \myL$ respectively, then we may view
$\frac 1 n X^T \tilde X$ as being an approximate rotation matrix.
In the following two Lemmas, we deal directly with the issues arising from
this missing rotation in \cref{lem:pert-sin-theta}.
% The following Lemmas provide the key steps in proving \cref{thm:pert-simplex-embedding} by directly taking into account this missing rotation.
\begin{lem}\label{lem:pert-arb-rotation}
  Suppose that $\norm H < \delta (L)$, that $X = (x_{\vecdot 1},
  \dotsc, x_{\vecdot \edim})$ contains an orthogonal basis of
  $\NN( \myL )$ scaled such that each $\norm{x_{\vecdot i}} = \sqrt
  \dn$, and that $\tilde X = (\tilde x_{\vecdot 1}, \dotsc, \tilde
  x_{\vecdot \edim})$ contains the lowest $\edim$ eigenvectors
  of $\tilde \myL$ scaled such that each $\norm{\tilde x_{\vecdot i}}
  = \sqrt \dn$.
  Then, for any rotation matrix $R \in \R^{\edim \times \edim}$,
  $\frac 1 {\sqrt \dn} \norm{XR - \tilde X} 
  \leq \frac{\norm H}{\mygap(\myL) - \norm H} 
       + \norm{\frac 1 \dn X^T \tilde X - R}$. 
\end{lem}
\begin{proof}
  Applying \cref{lem:pert-sin-theta}, we obtain that
  $\norm{P_{\NN(X)} P_{\RR(\tilde X)}} \leq \frac{\norm H}{\mygap(\myL) - \norm H}$.
  Since $\frac 1 {\sqrt \dn} \tilde X^T$ treated as a map from $\RR(\tilde X)$ to $\R^\edim$ is an isometry, we obtain that
  \begin{align*}
    \norm{P_{\NN(X)} P_{\RR(\tilde X)}}
    &= \norm{(\Id - \frac 1 \dn XX^T) \frac 1 \dn \tilde X \tilde X^T} \\
    &= \norm{(\Id - \frac 1 \dn XX^T) \frac 1 {\sqrt \dn} \tilde X}
    = \frac 1 {\sqrt \dn} \norm{\tilde X - \frac 1 \dn XX^T\tilde X} \ .
  \end{align*}
  We fix a rotation matrix $R$ and expand $\frac 1 \dn X^T \tilde X = \frac 1 \dn X^T \tilde X - R + R$ to obtain:
  \begin{align}
    \norm{P_{\NN(X)} P_{\RR(\tilde X)}}
    &= \frac 1 {\sqrt \dn} \norm{\tilde X - XR + X(R - \frac 1 \dn X^T\tilde X)} \nonumber \\
    &\geq \frac 1 {\sqrt \dn}( \norm{\tilde X - XR} - \norm{X(R - \frac 1 \dn X^T \tilde X}) \ . \label{eq:pert-sin-theta-1}
  \end{align}
  Treating $\frac 1 {\sqrt \dn} X$ as a linear map from $\RR(X)$ to
  $\R^\edim$ defined by the left multiplication 
  $\vec u \mapsto \frac 1 {\sqrt \dn} \vec u^T X$, 
  then $\frac 1 {\sqrt \dn} X$ is an isometry.
  As such, $\norm{\frac 1 {\sqrt \dn} X(R - \frac 1 \dn X^T \tilde X)} = \norm{R - \frac 1 \dn X^T \tilde X}$.
  Rearranging terms in \cref{eq:pert-sin-theta-1} and then applying \cref{lem:pert-sin-theta}, we obtain:
  \begin{align*}
    \frac 1 {\sqrt \dn} \norm{\tilde X - X R} 
    &\leq \norm{P_{\NN(X)}P_{\RR(\tilde X)}} + \norm{R - \frac 1 \dn X^T \tilde X} \\
    &\leq \frac{\norm H}{\mygap(\myL) - \norm H} + \norm{R - \frac 1 \dn X^T \tilde X} \ . \qedhere
  \end{align*}
  % where the final inequality uses \cref{lem:pert-sin-theta}.
\end{proof}
\begin{lem}\label{lem:pert-rotation-existence}
  Under the assumptions of \cref{lem:pert-arb-rotation},
  there exists a rotation matrix $R \in \R^{\edim \times \edim}$ such that $\norm{R - \frac 1 \dn X^T \tilde X} \leq \norm{P_{\NN(X)}P_{\RR(\tilde X)}} \leq \frac{\norm H}{\mygap(\myL) - \norm H}$.
\end{lem}
\begin{proof}
  Letting $U \Sigma V^T$ be a singular value decomposition of $\frac 1 \dn X^T \tilde X$, we consider the rotation $R = UV^T$.
  For this choice of $R$, $\norm{R - \frac 1 \dn X^T \tilde X} = \norm{U(\Id-\Sigma)V^T} = \norm{\Id - \Sigma}$.
  To see that $\norm{R - \frac 1 \dn X^T \tilde X} \leq \norm{P_{\NN(X)} P_{\RR(\tilde X)}}$, 
  it suffices to show that all of the singular values of $\frac 1 \dn X^T \tilde X$ are contained in the interval $[1 - \norm{P_{\NN(X)}P_{\RR(\tilde X)}}, 1]$.
  
  We denote the singular values of $\frac 1 \dn X^T \tilde X$ by the decreasing sequence $\sigma_1(\frac 1 \dn X^T \tilde X) \geq \cdots \geq \sigma_\edim(\frac 1 \dn X^T \tilde X)$.
  An upper bound is given by 
  \begin{displaymath}
    \sigma_1( \frac 1 \dn X^T \tilde X) = \norm{\frac 1 \dn X^T \tilde X} \leq \frac 1 \dn \norm{X^T} \norm{\tilde X} \leq 1 \ .
  \end{displaymath}
  
  We now find a lower bound on the singular values.
  Construct the matrix $Y \in \R^{\dn \times (\dn-\edim)}$ such that the columns of $[X\ Y]$ forms a scaled orthogonal basis of $\R^\dn$ with each column having $\sqrt \dn$ norm.
  By construction, $\sigma_1(\frac 1 \dn [X\ Y]^T \tilde X) = \cdots = \sigma_\edim(\frac 1 \dn  [X\ Y]^T \tilde X) = 1$. 
  % and $\sigma_{\edim + 1}(\frac 1 \dn  [X\ Y]^T \tilde X) = \cdots = \sigma_\dn(\frac 1 \dn  [X\ Y]^T \tilde X) = 0$.
  Expanding $\frac 1 \dn [X\ Y]^T \tilde X = \frac 1 \dn X^T \tilde X + \frac 1 \dn Y^T \tilde Y$, we obtain from a Weyl's inequality like bound for singular values \citep[Theorem 3.3.16]{horn37topics} that $\sigma_\edim(\frac 1 \dn [X\ Y]^T \tilde X) \leq \sigma_\edim(\frac 1 \dn X^T \tilde X) + \sigma_1(\frac 1 \dn Y^T \tilde X)$.
  Hence, $\sigma_\edim(\frac 1 \dn  X^T \tilde X) \geq \sigma_\edim(\frac 1 \dn [X\ Y]^T \tilde X) - \sigma_1(\frac 1 \dn  Y^T \tilde X) = 1 - \norm{\frac 1 \dn  Y^T \tilde X}$.
  Noting that the maps $\frac 1 {\sqrt \dn} Y : \RR(Y) \rightarrow \R^\edim$ defined by $\vec u \mapsto \frac 1 {\sqrt \dn} \vec u^T Y$ and $\frac 1 {\sqrt \dn} \tilde X^T : \RR( \tilde X ) \rightarrow \R^\edim$ defined by $\vec u \mapsto \frac 1 {\sqrt \dn} \tilde X^T \vec u$ are isometries, it follows that $\norm {\frac 1 \dn Y^T \tilde X} = \norm{ \frac 1 {\dn^2} YY^T \tilde X \tilde X^T } = \norm{P_{\NN(X)} P_{\RR(\tilde X)}}$.
  In particular, $\sigma_\edim(\frac 1 \dn X^T \tilde X) \geq 1 - \norm{P_{\NN(X)} P_{\RR(\tilde X)}}$ as desired.

  We have demonstrated that $\norm{R - \frac 1 \dn X^T \tilde X} \leq \norm{P_{\NN(X)} P_{\RR(\tilde X)}}$.
  To see the final inequality $\norm{P_{\NN(X)} P_{\RR(\tilde X)}} \leq \frac{\norm H}{\mygap(L) - \norm H}$, we apply \cref{lem:pert-sin-theta}.
\end{proof}

\Cref{lem:pert-arb-rotation,lem:pert-rotation-existence} combine to provide the following bound on the embedding error.

\begin{prop} \label{prop:pert-simplex-embedding-rotation}
  Suppose that $\norm H < \mygap(L)$,
  that $X = (x_{\vecdot 1}, \dotsc, x_{\vecdot \edim})$ contains a scaled orthogonal
  basis of $\NN(\myL)$ such that each $\norm{x_{\vecdot i}} = \frac 1 {\sqrt \dn}$,
  and that $\tilde X = (\tilde x_{\vecdot 1}, \dotsc, \tilde x_{\vecdot \edim})$
  contains the lowest $\edim$ eigenvectors of $\tilde \myL$ scaled such that
  each $\norm{\tilde x_{\vecdot i}} = \frac 1 {\sqrt \dn}$.
  There exists an orthogonal matrix $R \in \R^{\edim \times \edim}$ such that $\frac 1 {\sqrt \dn}\norm{X R - \tilde X} \leq \frac{2 \norm H}{\mygap(\myL) - \norm H}$.
\end{prop}

\Cref{thm:pert-simplex-embedding} follows by setting $X$ in \cref{thm:pert-simplex-embedding} to be $XR$ from \cref{prop:pert-simplex-embedding-rotation}.

\subsection{Perturbation Analysis of Cluster Recovery}
\label{sec:pert-analys-clust}
We now complete the perturbation analysis of spectral clustering.
We let $\fg : \R^{\edim} \rightarrow \R$ be as in
\cref{constr:spectral-Fg-L} (for a ``clean'' graph consisting of $\edim$ connected components).
We will first demonstrate that when $g$ is a robust contrast function
satisfying the \crefrange{assumpt:first}{assumpt:last}, then $F_g$
a robust \sef\@.
With this observation, we may construct $\tilde F_g$ an estimate of $F_g$ from the perturbed graph $G$ and then use our error analysis of the gradient
iteration\index{gradient iteration!error analysis} algorithm to provide a perturbation analysis for our spectral clustering method.
In particular, we will propagate the perturbation analysis of the
spectral embedding\index{spectral embedding!perturbation}
(\cref{sec:spectral-laplacian-pert}) to provide bounds on our
estimate of $\nabla F_g$.
Then, by applying the error analysis of the gradient iteration algorithm, we will bound the allowable perturbation size for perfect cluster recovery.

We now proceed with demonstrating that $F_g$ is a robust \sef\@.
% However, as we are interested in using the error analysis of the gradient iteration for spectral clustering, we will discuss the conditions are which $F_g$ is $(\alpha, \beta, \gamma, \delta)$-robust.
% Since $F_g$ for spectral clustering is built from a single contrast $g$, we will make use of the following definition for robustness of a single contrast function to for a bridge between individual contrast functions being robust and \ansef\@ being robust.

% \begin{defn}\label{def:contrast-robust}
%   Let $D \subset \R$.
%   A contrast function $g : D \rightarrow \R$ is said to be $(\alpha, \beta, \gamma, \delta)$-robust on its domain $D$ if the constants $\alpha, \beta, \gamma$, and $\delta$ are strictly positive and if for all $x \in D$, $\beta x^{\gamma - 1} \leq \Abs{\frac{d^2}{d t^2}[g(\sqrt t)]\big|_{t = x}} \leq \alpha x^{\delta - 1}$.
% \end{defn}
% In particular, comparing with \cref{defn:BEF-robust}, we see that \ansef\@ $F(\vec u) = \sum_{i=1}^\ldim g_i(\ipCanonical{\vec u}{\hbev_i})$ is $(\alpha, \beta, \gamma, \delta)$-robust precisely if each of its contrasts $g_i$ are $(\alpha, \beta, \gamma, \delta)$-robust on the domain $(0, 1]$.
% Using this connection, we may rewrite the function $F_g$ arising in spectral clustering as \ansef\@, and observe the relationship between robustness of $g$ and robustness of $F_g$.
\begin{lem}\label{lem:fg-spectral-robust}
  % \vnote{Add assumptions about $g$?}
  Suppose $F_g$ and all related variables are as in
  \cref{constr:spectral-Fg-L}.
  Suppose that $g$ satisfies
  \crefrange{assumpt:first}{assumpt:last} on the domain
  $[-\frac 1 {\sqrt{w_{\min}}},\ \frac 1 {\sqrt{w_{\min}}}]$.
  Suppose we define $g_i : \R \rightarrow \R$ by $g_i(t) := w_i g(\frac 1 {\sqrt {w_i}} \abs t)$ for all $i \in [\edim]$.
  Then,
  \begin{enumerate}
  \item\label{lem:fg-spectral-robust:constr}
    $F_g(\vec u) = \sum_{i=1}^\edim g_i(\ipCanonical{\vec u}{\myZv_i})$ 
    is \ansef\@ (satisfying
    \crefrange{assumpt:first}{assumpt:last}) with hidden
    basis $\myZv_1, \dotsc, \myZv_\edim$.
  \item\label{lem:fg-spectral-robust:robustness}
    If $g$ is $(\alpha,$ $\beta,$ $\gamma,$ $\delta)$-robust on the domain
    $(0, \frac 1 {\sqrt{w_{\min}}}]$, then the \sef\@ $F_g$ is 
    $(\frac \alpha {w_{\min}^\gamma},$ $\frac{\beta}{w_{\max}^\delta},$ $\gamma,$
    $\delta)$-robust.
  \end{enumerate}
\end{lem}
\begin{proof}
  We first prove part~\ref{lem:fg-spectral-robust:constr}.
  To see this, we expand each $g_i$ according to its definition to see:
  \begin{align*}
    \sum_{i=1}^\edim g_i(\ipCanonical {\vec u}{\myZv_i})
    = \sum_{i = 1}^\edim w_i g(\frac 1 {\sqrt {w_i}} \abs{\ipCanonical{\vec u}{\myZv_i}})
    = F_g(\vec u) \ ,
  \end{align*}
  by using \cref{eq:f_weighted_form}.
  Further, since the weights $w_1, \dotsc, w_\edim$ are non-zero and
  $g$ satisfies \crefrange{assumpt:first}{assumpt:last},
  it follows that each $g_i$ satisfies
  \crefrange{assumpt:first}{assumpt:last}.
  In particular, $F_g$ is \ansef\@.
  
  We now consider part~\ref{lem:fg-spectral-robust:robustness}.
  We note that on $(0, 1]$, $g_i(t) = w_i g(\frac 1 {\sqrt {w_i}} t)$ by construction.
  We may thus define the functions $h_i(t) := g_i(\sqrt t)$ and $h(t) := g(\sqrt t)$.
  We see that $h_i(t) = g_i(\sqrt t) = w_i g(\frac 1 {\sqrt{w_i}} \sqrt t) = w_i h( \frac t {w_i} )$.
  Taking derivatives, we obtain (for any $t \in (0, 1]$):
  \begin{equation}\label{eq:spectral-fg-gi-expansion}
    \frac{d^2}{d x^2}[g_i(\sqrt x)]\big|_{x=t}
    = h_i''(t) 
    = \frac 1 {w_i} h''( \frac t {w_i} )
    = \frac 1 {w_i} \cdot \frac{d^2}{d x^2}[g(\sqrt x)]\big|_{x={t/{w_i}}} \ .
  \end{equation}
  Since $g$ is $(\alpha, \beta, \gamma, \delta)$-robust, we see from \cref{eq:spectral-fg-gi-expansion} that for all $t \in (0, 1]$ and all $i \in [\edim]$,
  \begin{align*}
    \Abs{\frac{d^2}{d x^2}[g_i(\sqrt x)]\big|_{x=t}}
    &\in [\frac \beta {w_i} (t/{w_i})^{\delta - 1},\ \frac \alpha {w_i} (t/w_i)^{\gamma - 1}] \\
    &= [\frac \beta {w_i^\delta} t^\delta, \ \frac \alpha {w_i^\gamma} t^\gamma]
    \subset [\frac \beta {w_{\max}^\delta} t^\delta, \ \frac \alpha {w_{\min}^\gamma} t^\gamma] \ .
  \end{align*}
  Hence, $F_g$ is $(\frac \alpha {w_{\min}^\gamma}, \frac \beta {w_{\max}^\delta}, \gamma, \delta)$-robust.
\end{proof}
  % Suppose $F_g$ and all related variables are as in
  % \cref{constr:spectral-Fg-L}.
  
We will now combine the results from
\cref{sec:spectral-laplacian-pert} on the error analysis of the
spectral embedding with \cref{lem:fg-spectral-robust} to provide
an error analysis of the entire spectral clustering framework.
For this purpose, we will first define in
\cref{constr:BEF-spectral-pert-exact-Fg} below what is
meant by the exact \sef\@ $F_g$ given access to the approximate $\tilde
F_g$ constructed from $\tilde L$.
Then, in \cref{lem:spectral-bef-pert}, we bound the estimation
error for $\nabla \tilde F_g$.
Finally in \cref{thm:BEF-spectral-pert-full}, we use the error
analysis of the gradient iteration algorithm
(\cref{cor:robust-all-recovery-error-version}) to provide an
error analysis of BEF-based spectral clustering.

\begin{construction}[Perturbed and Exact BEFs for Spectral Clustering]\label{constr:BEF-spectral-pert-exact-Fg}
  We use the notation of \cref{sec:spectral-laplacian-pert}.
  In particular, $G$ is an $\dn$-vertex graph consisting
  of $\edim$-connected components with vertices in the index sets
  $\SS_1, \dotsc, \SS_\edim$ respectively; $L = D - A$ is the
  graph Laplacian constructed from $G$; $\tilde L = L +
  H$ is the graph Laplacian of a graph $\tilde G$ with identical
  vertices to $G$, but with similarity matrix $\tilde A$ considered to
  be a perturbation of $A$; and the eigengap $\mygap(L) = \lambda_{\edim + 1}(L) -
  \lambda_\edim(L)$ is such that $\norm H < \mygap(L)$.

  Let $\tilde X \in \R^{\dn \times \edim}$ be such that its columns
  are the lowest $\edim$ eigenvectors of $\tilde L$, scaled such that
  each column satisfies $\norm{\tilde x_{\vecdot i}} = \sqrt \dn$.
  Let $X$ be as in \cref{thm:pert-simplex-embedding}.
  The function $F_g$ and its approximation $\tilde F_g$ are
  defined as $F_g(\vec u) := \frac 1 \dn \sum_{i = 1}^\dn
  g(\abs{\ipCanonical{\vec u}{x_{i\vecdot}}})$ and $\tilde F_g(\vec u)
  := \frac 1 \dn \sum_{i = 1}^\dn g(\abs{\ipCanonical{\vec u}{\tilde
      x_{i\vecdot}}})$ respectively.
\end{construction}
  
\begin{lem}\label{lem:spectral-bef-pert}
  Under \cref{constr:BEF-spectral-pert-exact-Fg}, we let
  $E \geq 0$ be a fixed constant, we suppose that $\norm H \leq
  \mygap(L) \min(\frac 1 2, \frac E {\sqrt \dn})$,
  and we suppose that $g$ is $(\alpha, \beta, \delta, \gamma)$-robust.
  Then, there exists a universal constant $C > 0$ such that for all
  $\vec u \in \overline{\ball(0, 1)}$,
  \begin{displaymath}
    \norm{\nabla \tilde F_g(\vec u) - \nabla F_g(\vec u)}
    \leq C \alpha (1 + \frac 1 \gamma) \sqrt \edim [\frac 1 {\sqrt{\wmin}} + 4E]^{1 + 2\gamma} \frac {\norm H}{\mygap(L)} \ . \qedhere
  \end{displaymath}
  % \begin{displaymath}
  %   \norm{\nabla \tilde F(\vec u) - \nabla F(\vec u)}
  %   \leq C \alpha (1 + \frac 1 \gamma) \frac {E \sqrt \edim}{\sqrt \dn}[\frac 1 {\sqrt {\wmin}} + 4E]^{1 + 2\gamma} \ .
  % \end{displaymath}
\end{lem}
\begin{proof}
  We expand the formula $\norm{\nabla \tilde F_g(\vec u) - \nabla F_g(\vec u)}$ to obtain:
  \begin{align} \label{eq:spectral-gradf-error-expansion}
    &\norm{\nabla \tilde F_g(\vec u) - \nabla F_g(\vec u)}
    = \frac 1 \dn \biggr\lVert \sum_{i = 1}^\dn \left[g'(\ipCanonical{\tilde x_{i \vecdot}}{\vec u}) \tilde x_{i \vecdot} - g'(\ipCanonical{x_{i \vecdot}}{\vec u}) x_{i \vecdot}  \right] \biggr\rVert \nonumber \\
    &\qquad= \frac 1 \dn \biggr\lVert \sum_{i = 1}^\dn \Big[
      g'(\ipCanonical{\tilde x_{i \vecdot}}{\vec u})[\tilde x_{i \vecdot} - x_{i \vecdot}] 
      + [g'(\ipCanonical{\tilde x_{i \vecdot}}{\vec u}) - g'(\ipCanonical{x_{i \vecdot}}{\vec u})] x_{i \vecdot}
      \Big] \biggr\rVert \nonumber \\
    &\qquad\leq \frac 1 \dn \sum_{i=1}^\dn \abs{g'(\ipCanonical{\tilde x_{i \vecdot}}{\vec u})} \cdot \norm{\tilde x_{i \vecdot} - x_{i \vecdot}}
      + \frac 1 \dn \sum_{i=1}^\dn \frac 1 {\sqrt {w_{\min}}} \abs{g'( \ipCanonical{\tilde x_{i \vecdot}}{\vec u}) - g'(\ipCanonical{x_{i\vecdot}}{\vec u})} \ ,
  \end{align}
  by using that for any $i \in \SS_j$, $\norm{x_{i \vecdot}} = \frac 1
  {\sqrt{w_j}} \leq \frac 1 {\sqrt {w_{\min}}}$ (see
  \cref{prop:discrete-simplex}). 
  % and \cref{constr:spectral-Fg-L}).
  We now bound the individual terms in
  \cref{eq:spectral-gradf-error-expansion}.
  We first bound $\frac 1 \dn \sum_{i = 1}^\dn \norm{\tilde x_{i \vecdot} -
    x_{i \vecdot}}$ and the closely related $\frac 1 \dn \sum_{i = 1}^\dn
  \abs{\ipCanonical{(\tilde x_{i \vecdot} - x_{i \vecdot})}{\vec u}}$.
  By Jensen's inequality, 
  \begin{equation}\label{eq:X-pert-Jensen-bound}
    (\frac 1 \dn \sum_{i = 1}^\dn \abs{\ipCanonical{(\tilde x_{i \vecdot} - x_{i \vecdot})}{\vec u}})^2
    \leq \frac 1 \dn \sum_{i=1}^\dn \ipCanonicalp{(\tilde x_{i \vecdot} - x_{i \vecdot})}{\vec u}^2 \ .
  \end{equation}
  % \begin{displaymath}
  %   (\frac 1 \dn \sum_{i = 1}^\dn \norm{\tilde x_{i \vecdot} - x_{i \vecdot}})^2
  %   \leq \frac 1 \dn \sum_{i=1}^\dn \norm{\tilde x_{i \vecdot} - x_{i \vecdot}}^2
  %   = \frac 1 \dn \norm[F]{\tilde X - X}^2
  %   \leq \frac 1 \dn \norm{\tilde X - X}^2 \edim \ .
  % \end{displaymath}
  In order to compress notation, we define $\epsilon := \frac{2 \norm H}{\mygap(L) - \norm H}$.
  Applying \cref{rmk:pert-simplex-embedding} to \cref{eq:X-pert-Jensen-bound}, we obtain
  \begin{equation}\label{eq:spectral-bef-pert:1}
    \frac 1 \dn \sum_{i = 1}^\dn \abs{\ipCanonical{(\tilde x_{i \vecdot} - x_{i \vecdot})}{\vec u}}
    \leq \epsilon \ .
    % \qquad\qquad \text{and} \\
    % \frac 1 \dn \sum_{i = 1}^\dn \norm{\tilde x_{i \vecdot} - x_{i \vecdot}}
    % & %\leq \frac{ \sqrt \edim} {\sqrt \dn} \norm{\tilde X - X}
    % \leq \frac 1 \dn \Big(\sum_{i = 1}^\dn \sum_{j=1}^\edim \ipCanonicalp{(\tilde x_{i\vecdot} - x_{i \vecdot})}{\vec e_j}^2\Big)^{1/2}
    % \leq \frac{\sqrt \edim}{\sqrt \dn} \epsilon \ .
  \end{equation}
  By similar reasoning, we see that $(\frac 1 \dn \sum_{i = 1}^\dn
  \norm{\tilde x_{i \vecdot} - x_{i \vecdot}})^2 \leq \frac 1 \dn
  \sum_{i=1}^\dn \norm{\tilde x_{i \vecdot} - x_{i \vecdot}}^2 \leq
  \epsilon^2 \edim$, and hence
  \begin{equation}\label{eq:spectral-bef-pert:2}
    \frac 1 \dn \sum_{i = 1}^\dn \norm{\tilde x_{i \vecdot} - x_{i \vecdot}}
    \leq \epsilon\sqrt \edim \ .
  \end{equation}

  We now bound the second summand in \cref{eq:spectral-gradf-error-expansion}.
  By the mean value theorem, for all $i \in [\dn]$ there exists $c_i$ between $\ipCanonical{\tilde x_{i \vecdot}}{\vec u}$ and $\ipCanonical{x_{i \vecdot}}{\vec u}$ such that
  \begin{align*}
    \frac 1 \dn \sum_{i=1}^\dn \frac 1 {\sqrt {w_{\min}}} \abs{g'( \ipCanonical{\tilde x_{i \vecdot}}{\vec u}) - g'(\ipCanonical{x_{i\vecdot}}{\vec u})}
    &= \frac 1 {\dn} \sum_{i = 1}^\dn \frac 1 {\sqrt {\wmin}} \abs{g''(c_i)\ipCanonicalp{(\tilde x_{i\vecdot} - x_{i \vecdot})}{\vec u}} \ .
  \end{align*}
  By \cref{eq:spectral-bef-pert:1}, it follows that 
  \begin{displaymath}
    \frac 1 \dn \sum_{i=1}^\dn \frac 1 {\sqrt {w_{\min}}} \abs{g'( \ipCanonical{\tilde x_{i \vecdot}}{\vec u}) - g'(\ipCanonical{x_{i\vecdot}}{\vec u})}
    \leq \frac \epsilon  {\sqrt {\wmin}} \max_{i \in [\dn]} \abs{g''(c_i)} \ .
  \end{displaymath}
  By \cref{thm:pert-simplex-embedding}, we obtain
  \begin{math}
    \norm{\tilde x_{i \vecdot}} 
    \leq \norm{x_{i \vecdot}} + \norm{\tilde x_{i \vecdot} - x_{i \vecdot}}
    \leq \frac 1 {\sqrt {\wmin}} + \epsilon \sqrt \dn .
  \end{math}
  As such, for all $i \in [\dn]$, $\abs{c_i} \leq \frac 1 {\sqrt{\wmin}} + \epsilon\sqrt \dn$.
  Applying \cref{lem:F-robust-implications}, we see that
  \begin{math}
    \abs{g''(c_i)}
    \leq 2(2+\frac 1 \gamma)\alpha (\frac 1 {\sqrt {\wmin}} + \epsilon\sqrt \dn)^{2\gamma} .
  \end{math}
  The second summand of \cref{eq:spectral-gradf-error-expansion} can be bounded as
  \begin{equation}\label{eq:spectral-bef-pert:summand2}
    \frac 1 \dn \sum_{i=1}^\dn \frac 1 {\sqrt {w_{\min}}} \abs{g'( \ipCanonical{\tilde x_{i \vecdot}}{\vec u}) - g'(\ipCanonical{x_{i\vecdot}}{\vec u})}
    \leq 2(2+\frac 1 \gamma)\alpha (\frac 1 {\sqrt {\wmin}} + \epsilon\sqrt \dn)^{2\gamma} \frac{\epsilon}{\sqrt{\wmin}} \ .
  \end{equation}

  We now bound the first summand of \cref{eq:spectral-gradf-error-expansion}.
  We note that each
  \begin{math}
    \abs{\ipCanonical{\tilde x_{i \vecdot}}{\vec u}}
    \leq \norm{\tilde x_{i\vecdot}}
    \leq \frac 1 {\sqrt {\wmin}} + \epsilon \sqrt \dn .
  \end{math}
  Using \cref{lem:F-robust-implications}, we thus obtain that
  \begin{displaymath} 
    \abs{g'(\ipCanonical{\tilde x_{i \vecdot}}{\vec u})}
    \leq 2 \frac \alpha \gamma (\frac 1 {\sqrt{w_{\min}}} + \epsilon \sqrt \dn)^{1 + 2\gamma}
  \end{displaymath}
  for all $i \in [\dn]$.
  % Further, using \cref{eq:spectral-bef-pert:1}, we see that
  % \begin{displaymath}
  %   \frac 1 \dn \sum_{i=1}^\dn \norm{\tilde x_{i \vecdot} - x_{i \vecdot}}
  %   = \Big(\frac 1 \dn \sum_{i = 1}^\dn \sum_{j=1}^\edim \abs{\ipCanonical{(\tilde x_{i \vecdot} - x_{i \vecdot})}{\vec u}} \Big)^{1/2}
  %   \leq \frac {\sqrt \edim}{\sqrt \dn} \epsilon .
  % \end{displaymath}
  Combining this with \cref{eq:spectral-bef-pert:2}, we see
  that the first summand of
  \cref{eq:spectral-gradf-error-expansion} is bounded as
  \begin{equation}
    \label{eq:spectral-gradf-error-expansoin:1-1}
    \frac 1 \dn \sum_{i=1}^\dn \abs{g'(\ipCanonical{\tilde x_{i \vecdot}}{\vec u})} \cdot \norm{\tilde x_{i \vecdot} - x_{i \vecdot}}
    \leq 2\frac \alpha \gamma [\frac 1 {\sqrt {\wmin}} + \epsilon \sqrt \dn]^{1+2\gamma}  \epsilon \sqrt \edim
  \end{equation}
  From \cref{eq:spectral-gradf-error-expansion,eq:spectral-bef-pert:summand2,eq:spectral-gradf-error-expansoin:1-1}, we obtain a full error bound:
  \begin{align*}
    &\norm {\nabla \tilde F_g(\vec u) - \nabla F_g(\vec u)} \\
    &\qquad\leq 2 \frac \alpha \gamma [\frac 1 {\sqrt {\wmin}} + \epsilon \sqrt \dn]^{1+2\gamma} \epsilon \sqrt \edim
      + 2 (2+\frac 1 \gamma)\alpha (\frac 1 {\sqrt {\wmin}} + \epsilon\sqrt \dn)^{2\gamma} \frac \epsilon {\sqrt{\wmin}} \ .
  \end{align*}

  Expanding $\epsilon$ and using the assumed bound on $\norm H$, we see that
  \begin{displaymath}
    \epsilon 
    = \frac{2 \norm H}{\mygap(L) - \norm H}
    \leq \frac {4 \norm H}{\delta (L)}
    \leq \frac {4E}{\sqrt \dn} \ .
  \end{displaymath}
  It follows that for some universal constant $C > 0$,
  \begin{displaymath}
    \norm{\nabla \tilde F_g(\vec u) - \nabla F_g(\vec u)}
    \leq C \alpha (1 + \frac 1 \gamma) \sqrt \edim [\frac 1 {\sqrt{\wmin}} + 4E]^{1 + 2\gamma} \frac {\norm H}{\mygap(L)} \ . \qedhere
  \end{displaymath}
  % \begin{displaymath}
  %   \norm{\nabla \tilde F_g(\vec u) - \nabla F_g(\vec u)}
  %   \leq C \alpha (1 + \frac 1 \gamma) \frac {E \sqrt \edim}{\sqrt \dn}[\frac 1 {\sqrt{\wmin}} + 4E]^{1 + 2\gamma} \ . \qedhere
  % \end{displaymath}
\end{proof}

\begin{algorithm}[tbh]
  \caption[Robust spectral clustering algorithm]{
    A robust algorithm for spectral clustering.
  }\label{alg:spectral-robust}
  \begin{algorithmic}[1]
    \Function{RobustSpectralClustering}{$\tilde A$, $g'$, $k$, $\sigma$, $N_1$, $N_2$, $I$}
      \State Construct the graph Laplacian $\tilde L$ from $\tilde A$.
      \State Construct $\tilde X = (\tilde x_{\vecdot 1}, \dotsc, \tilde x_{\vecdot \edim})$ such that each $\tilde x_{\vecdot i}$ is the $i$\textsuperscript{th} lowest eigenvector \newline \phantom{.} $\qquad$ of $\tilde L$ scaled such that $\norm{\tilde x_{\vecdot \edim}} = \sqrt \dn$.
      \State Define the function pointer $dF_g(\vec u) := \frac 1 \dn \sum_{i=1}^\dn g'(\ipCanonical{\vec u}{\tilde x_{i \vecdot}}) x_{i \vecdot}^T$.
      \State\label{alg:robust-spectral:step:robust-gi}
      $\tilde \myZv_1, \dotsc, \tilde \myZv_\edim \leftarrow \textsc{RobustGI-Recovery}$($k$, $\sigma$, $dF_g$, $N_1$, $N_2$, $I$).
      \State
      \State // Initialize the clusters
      \For {$j \leftarrow 1$ to $\edim$}
        \State $\tilde \SS_j \leftarrow \emptyset$
      \EndFor
      \State
      \State // Assign cluster labels to graph vertices.
      \For {$i \leftarrow 1$ to $\dn$}
        \State $j \leftarrow \argmax_\ell \abs{\ipCanonical {\tilde \myZv_\ell}{x_{i \vecdot}}}$.
        \State $\tilde \SS_j \leftarrow \tilde \SS_j \cup \{i\}$
      \EndFor
      \State \Return $\tilde \SS_1, \dotsc, \tilde \SS_\edim$.
    \EndFunction
  \end{algorithmic}
\end{algorithm}


For simplicity, we proceed in analyzing spectral clustering using the families of contrasts $g_{p,{\tabs}}(t) := \frac{1}{p(p+1)} \abs{t}^{2(p+1)}$ and  $g_{p,{\sign}}(t) := \frac{\sign(t)}{p(p+1)} \abs{t}^{2(p+1)}$ for all real $p > 0$.
It can be verified that these contrast functions are $(1, 1, p, p)$ robust.
For clarity, we will denote by $C_0, C_1, C_2, \dotsc$ positive universal constants in the main theorem statements.
These can represent different constant values in different theorem statements.
\begin{thm}[Full spectral perturbation analysis]\label{thm:BEF-spectral-pert-full}
  In \cref{constr:BEF-spectral-pert-exact-Fg}, we suppose that $g$ is a $(1, 1, p, p)$-robust function on the domain $[- \frac 1 {\sqrt {\wmin}}, \frac 1 {\sqrt {\wmin}} ]$.
  We suppose that $\sigma \leq C_0 \cdot  16^{-\frac 1 p}(1+p)^{-\frac 1 2} \cdot \frac \wmin \wmax \edim^{-\frac 3 2}$ and that
  \begin{displaymath}
    \norm H
    \leq \min\Big( \frac 1 2,\ C_1(\dn \wmax)^{-\frac 1 2},\
    C_2 \frac{\sigma \sqrt{\wmin}(\frac \wmin \wmax)^{3p + \frac 7 2}}{2^{\frac 8 p + 2p}(p+1)\edim^{2p + \frac 7 2}}\Big) \mygap(L)\ .
  \end{displaymath}
  Fix any $\delta \in (0, 1)$.
  Suppose that $I \geq C_3 \edim\lceil \log(\edim / \delta)\rceil$,
  $N_1 \geq C_4
  \Big\lceil \log_{1+2p}\big[(\frac 8 p + 2p + 4)(1+\log_2(\frac {k \wmax}{\sigma \wmin})) \big]\Big\rceil$, 
  and $N_2 \geq C_5
  \Big\lceil 16^{\frac 1 p} \sigma^{-1} ( \frac{\wmax}{\wmin} )^{p + 2}
  \edim^{\frac 5 2} \big[ \log( \frac {\wmax}{\wmin} ) + \log(k)
  \big]\Big\rceil + N_1$.
  Then with probability at least $1-\delta$,
  \textsc{RobustSpectralClustering}($\tilde A, g', k, \sigma, N_1,
  N_2, I$) partitions $\tilde G$ according to the components of $G$ in
  $(N_1 + IN_2)\poly(\edim, \dn)$ time.
\end{thm}

The proof of \cref{thm:BEF-spectral-pert-full} relies on the
perturbation analysis of the gradient iteration algorithm from
\cref{cor:robust-all-recovery-error-version}.
For easier reference, we rewrite this corollary using the notation of
spectral clustering.
\begin{lem}[\Cref{cor:robust-all-recovery-error-version} restated for spectral clustering]\label{lem:cor-gi-robust-spectral-version} 
  In \cref{constr:BEF-spectral-pert-exact-Fg}, we suppose
  that $F_g$ is $(\frac 1 {\wmin^p}, \frac 1
  {\wmax^p}, p, p)$-robust.
  Suppose also that
  \begin{itemize}
  \item $\sigma \leq C_0\Big(16^{-\frac 1 p}(1+p)^{-\frac 1 2} \cdot \frac \wmin \wmax \edim^{-3/2}\Big)$,
  \item $\eta \leq C_1\Big(2^{-\frac 8 p}(\frac{\wmin}{\wmax})^{2p+\frac 7 2} \edim^{-2p-4} \sigma \Big)$,
  \item $N_1 \geq C_2 \Big\lceil \log_{1+2p}\log_2(\frac 1 \eta) \Big\rceil$, and
  \item $N_2 \geq C_3 \Big\lceil
    16^{\frac 1 p} \sigma^{-1} ( \frac{\wmax}{\wmin} )^{p + 2} \edim^{\frac 5 2} 
    \big[ \log( \frac {\wmax}{\wmin} ) + \log(k) \big]\Big\rceil
    + C_2\Big\lceil \log_{1+2p}\log_2(\frac 1 \eta) \Big\rceil$.
  \end{itemize}
  Let $\delta \in (0, 1)$, and suppose $I \geq C_4\edim \lceil\log (\edim/\delta)\rceil$.
  If $\nabla \tilde F_g$ is a $C_5 \frac \eta {p \wmax^{p}}$-approximation to $\nabla F_g$ and if we execute
  $\tilde \myZv_1, \dotsc, \tilde \myZv_\edim \leftarrow \textsc{RobustGI-Recovery}(\edim, \sigma, \nabla \tilde F_g, N_1, N_2, I)$,
  then with probability at least $1-\delta$, $\tilde \myZv_1, \dotsc, \tilde \myZv_\edim$ is an $\eta$-recovery of $\myZv_1, \dotsc, \myZv_\edim$.
\end{lem}

% \begin{thm}[\cref{cor:robust-all-recovery-error-version} restated for spectral clustering]\label{thm:cor-gi-robust-spectral-version}
%   In \cref{constr:BEF-spectral-pert-exact-Fg}, we suppose
%   that $F_g$ is $(\frac \alpha {\wmin^\gamma}, \frac \beta
%   {\wmax^\delta}, \gamma, \delta)$-robust.
%   Treating $\gamma$ and $\delta$ as fixed constants, we suppose that
%   $\sigma \leq \poly^{-1}(\edim, \frac {\wmax^\delta}{\wmin^\gamma}, \frac \alpha \beta)$, 
%   $\eta \leq \poly^{-1}(\edim, \frac {\wmax^\delta}{\wmin^\gamma}, \frac \alpha \beta)\sigma$,
%   $N_1 \geq O\big( \log \log(\frac 1 \eta) \big)$, 
%   and $N_2 \geq \poly(\frac \alpha \beta, \frac {\wmax^\delta}{\wmin^\gamma}, \edim)\sigma^{-1} + O\big( \log\log(\frac 1 \eta) \big)$.
%   Let $p \in (0, 1)$, and suppose that $I \geq O(\edim \log (k/p))$.
%   If $\nabla \tilde F_g$ is a $O(\frac \beta {\wmax^\delta}
%   \eta)$-approximation to $\nabla F_g$ and if we execute
%   $\tilde \myZv_1, \dotsc, \tilde \myZv_\edim \leftarrow \textsc{RobustGI-Recovery}(\edim, \sigma, \nabla \tilde F_g)$
%   (implemented with these choices of $N_1$, $N_2$, and $I$), then with
%   probability at least $1-p$ there exists $\pi$ a permutation of
%   $[\edim]$ and signs $s_1, \dotsc, s_\edim$ such that $\norm{\myZv_i
%     - s_i \tilde \myZv_{\pi(i)}} \leq \eta$ for all $i \in [\edim]$.
% \end{thm}

\begin{proof}[\proofword of \cref{thm:BEF-spectral-pert-full}]
  We will require that $C_1 \leq \frac 1 4$ so that $\norm{H} \leq \frac 1 4
  (\dn \wmax)^{- \frac 1 2}$.
  Then, we apply \cref{lem:spectral-bef-pert} (with the constant $E=\frac
  1 {4\sqrt {\wmax}}$ in that Lemma) to obtain that for all $\vec u \in \overline {B(0, 1)}$,
  \begin{align*}
    \norm{\nabla \tilde F(\vec u) - \nabla F(\vec u)}
    &\leq 
    O\left( (1+1 / p) (\frac 1 {\sqrt {\wmin}} + \frac 1 {\sqrt{\wmax}})^{1+2p}  \edim^{- \frac 1 2 } \frac {\norm H}{\mygap(L)} \right) \\
    &\leq O\left( 2^{2p}\Big(\frac{p+1} p\Big) \wmin^{-\frac 1 2 - p}  \edim^{- \frac 1 2 } \frac {\norm H}{\mygap(L)} \right)\ ,
  \end{align*}
  using that $\frac 1 {\sqrt {\wmax}} \leq \frac 1 {\sqrt {\wmin}}$ in the
  final inequality.
  Further, by the given bound on $\norm H$, $\nabla \tilde F_g$ is an
  \begin{equation}\label{eq:4}
    O\left(2^{-\frac 8 p} p^{-1} \wmin^{-p} \Big(\frac \wmin \wmax\Big)^{3p + \frac 7 2} \edim^{-2p-4} \sigma \right)
  \end{equation}
  approximation to $\nabla F_g$.
  We set $\eta$ to be $p \wmax^p$ times \cref{eq:4} to obtain that
  $\nabla \tilde F_g$ is an $O(\frac{\eta}{p \wmax^p})$-approximation to
  $\nabla F_g$.
  Further,
  \begin{equation}\label{eq:5}
\eta \leq O(2^{-\frac 8 p} \big(\frac \wmin \wmax\big)^{2p + \frac
    7 2} \edim^{-2p - 4}\sigma) \ .
  \end{equation}

  By \cref{lem:fg-spectral-robust}, $\nabla \tilde F_g$ is a $(\frac 1
  {\wmin^p}, \frac 1 {\wmax^p}, p, p)$-approximation to $\nabla F_g$.
  Further, it can be verified that $N_1 \geq \log_{1+2p}(\log_2(1/\eta))$.
  Combining these facts, we may apply
  \cref{lem:cor-gi-robust-spectral-version} to see that at the end of the
  execution of line~\ref{alg:robust-spectral:step:robust-gi} of
  \textsc{RobustSpectralClustering}, then with probability at least $1-\delta$
  $\tilde \myZv_1, \dotsc, \tilde \myZv_\edim$ is an $\eta$-recovery of $\myZv_1, \dotsc, \myZv_\edim$.
  
  We assume without loss of generality\footnote{%
    We may do this since the ordering and sign associated with the $\pm
    \myZv_i$ hidden basis directions are a matter of convention.}
  that $\norm{\tilde \myZv_i - \myZv_i} \leq
  \eta$ for all $i \in [\edim]$.
  To complete the proof, we will need the following claim.
  \begin{claim}\label{claim:correct-clustering-criterion}
    If $\frac{2\norm H \sqrt \dn}{\mygap(L) - \norm H} + \frac 1 {\sqrt {\wmin}} \max_j
    \norm{\tilde \myZv_j - \myZv_j} < \frac 1 {2 \sqrt{\wmax}}$, then
    \textsc{RobustSpectralClustering} clusters the vertices of $\tilde
    G$ according to the connected components of $G$.
  \end{claim}
  \begin{subproof}
    In order to simplify notation, we define $\epsilon_0 := \frac{2\norm
      H}{\mygap(L) - \norm H}$ to be the constant from
    \cref{thm:pert-simplex-embedding}.
    % We note that this may be bounded as $\epsilon_0 = O(\frac{\norm
    %   H}{\mygap(L)})$ by the assumption that $\norm H \leq \frac 1 2
    % \mygap(L)$.

    For all $i \in [\dn]$ and all $j \in [\edim]$, it follows (using the notation from \cref{constr:BEF-spectral-pert-exact-Fg}) that
    \begin{align}\label{eq:spectralError-1}
      \abs{\ipCanonical{\tilde x_{i \vecdot}}{\tilde \myZv_j} - \ipCanonical{x_{i \vecdot}}{\myZv_j}}
        &= \abs{
          \ipCanonical{(\tilde x_{i \vecdot} - x_{i \vecdot})}{\tilde \myZv_j} +
          \ipCanonical{x_{i \vecdot}}{(\tilde \myZv_j - \myZv_j)}
        }  \nonumber \\
        &\leq \abs{\ipCanonical{(\tilde x_{i \vecdot} - x_{i \vecdot})}{\tilde \myZv_j}} +
        \norm{x_{i\vecdot}} \cdot \norm{\tilde \myZv_j - \myZv_j} \nonumber \\
        &\leq \epsilon_0 \sqrt \dn + \frac 1 {\sqrt{\wmin}} \cdot \norm{\tilde \myZv_j - \myZv_j} \ ,
    \end{align}
    where the first term in the final inequality is bounded using
    \cref{thm:pert-simplex-embedding}, and the second term is
    bounded using \cref{prop:discrete-simplex}.
    Also by \cref{prop:discrete-simplex},
    $\ipCanonical{x_{i\vecdot}}{\myZv_j} = \indicator{i \in
      \SS_j}\frac 1 {\sqrt{w_j}}$.
    We proceed from \cref{eq:spectralError-1} in two cases.
    In the case where $i \in \SS_j$,
    \begin{displaymath}
      \abs{\ipCanonical{\tilde x_{i \vecdot}}{\tilde \myZv_j} - \frac 1 {\sqrt{w_j}}}
      \leq \epsilon_0 \sqrt \dn + \frac 1 {\sqrt{\wmin}} \cdot \norm{\tilde \myZv_j - \myZv_j} \notag      
    \end{displaymath}
  and hence,
    \begin{align}\label{eq:spectralError-2}
      \abs{\ipCanonical{\tilde x_{i \vecdot}}{\tilde \myZv_j}}
      &\geq \frac 1 {\sqrt{w_j}} - \epsilon_0 \sqrt \dn - \frac 1 {\sqrt{\wmin}} \cdot \norm{\tilde \myZv_j - \myZv_j} \nonumber \\
      &\geq \frac 1 {\sqrt{\wmax}} - \epsilon_0 \sqrt \dn - \frac 1 {\sqrt{\wmin}} \cdot \norm{\tilde \myZv_j - \myZv_j} \ .
    \end{align}

    In the case where $i \not \in \SS_j$, we obtain
    \begin{equation}
      \label{eq:spectralError-3}
      \abs{\ipCanonical{\tilde x_{i \vecdot}}{\tilde \myZv_j}}
      \leq \epsilon_0 \sqrt \dn + \frac 1 {\sqrt{\wmin}} \cdot \norm{\tilde \myZv_j - \myZv_j} \ .
    \end{equation}

    The $i$\textsuperscript{th} vertex is correctly clustered if for
    that choice of $i$, the right hand side (r.h.s.\@) of
    \cref{eq:spectralError-2} with $i \in \SS_j$ exceeds the
    r.h.s.\@ of \cref{eq:spectralError-3} for all
    other choices of $j$.
    It suffices that the smallest obtainable value for the r.h.s.\@ of \cref{eq:spectralError-2} exceeds the largest obtainable value for the r.h.s.\@ of \cref{eq:spectralError-3}, i.e.\@ $\frac 1 {\sqrt {\wmax}} - \epsilon_0 \sqrt
    \dn - \frac 1 {\sqrt{\wmin}} \max_{j \in [\edim]}\norm{\tilde \myZv_j - \myZv_j}
    > \epsilon_0 \sqrt \dn + \frac 1 {\sqrt{\wmin}} \max_{j \in [\edim]} \norm{\tilde \myZv_\ell - \myZv_\ell}$.
    In particular, it suffices that $\epsilon_0 \sqrt \dn + \frac
    1 {\sqrt{\wmin}} \cdot \max_{j} \norm{\tilde \myZv_j - \myZv_j} <
    \frac 1 {2 \sqrt {\wmax}}$.
  \end{subproof}
  To complete the proof, we bound the terms in the inequality from \cref{claim:correct-clustering-criterion}.
  First, we note that
  \begin{displaymath}
    \frac{2\norm H \sqrt \dn}{\mygap(L) - \norm H}
    \leq O(\frac{\norm H}{\mygap(L)} \sqrt \dn)
    \leq O(\frac 1 {\sqrt{\wmax}}) \ ,
  \end{displaymath}
  where the first inequality uses the given bound $\norm H \leq \frac 1 2 \mygap(L)$ to see that the denominator is at least $\frac 1 2 \mygap(L)$, and the second inequality uses the given bound $\norm H \leq O(n \wmax)^{-\frac 1 2} \mygap(L)$.
  We also note that
  \begin{align*}
    \frac 1 {\sqrt {\wmin}} \max_j \norm{\tilde \myZv_j - \myZv_j}
    &\leq \frac \eta {\sqrt {\wmin}}
    \leq \frac 1 {\sqrt{\wmin}}O\left(2^{-\frac 8 p}\bigr(\frac \wmin \wmax\bigr)^{2p+\frac 7 2}\edim^{-2p-4}\sigma\right) \\
    &\leq \frac 1 {\sqrt{\wmin}}O\left(2^{-\frac {12} p}(1+p)^{-\frac 1 2} \bigr(\frac \wmin \wmax \bigr)^{2p+\frac 9 2} \edim^{-2p - \frac{11}{2}}\right)  \\
    &\leq O\left(\frac 1 {\sqrt{\wmax}}\right) \ .
  \end{align*}
  As such, applying \cref{claim:correct-clustering-criterion} completes the proof.
\end{proof}
\def\dn{\dnold}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 

